Fact Probability Vector Based Goal Recognition

We present a new approach to goal recognition that involves comparing observed facts with their expected probabilities. These probabilities depend on a specified goal g and initial state s0. Our method maps these probabilities and observed facts into a real vector space to compute heuristic values for potential goals. These values estimate the likelihood of a given goal being the true objective of the observed agent. As obtaining exact expected probabilities for observed facts in an observation sequence is often practically infeasible, we propose and empirically validate a method for approximating these probabilities. Our empirical results show that the proposed approach offers improved goal recognition precision compared to state-of-the-art techniques while reducing computational complexity.

==> algorithms/calculate_fact_probability.tex <==
\begin{algorithm}[t!]
\caption{Derive Fact Probability Algorithm.}
\label{alg:factProbability}
\begin{algorithmic}[1]
\Function{Derive Fact Probabilities}{$P_A$}
\State $P_F \leftarrow \{\}$
\State $max \leftarrow 0$
\ForAll{$a \in P_A.keys$}
    \ForAll{$e \in add(a)$}
        \State $P_F[e] \leftarrow P_F[e] + P_A[a]$
        \If{$P_F[e] > max$}
            \State $max \leftarrow P_F[e]$
        \EndIf
    \EndFor
\EndFor
\ForAll{$e \in P_F.keys$}
    \State $P_F[e] \leftarrow P_F[e]/max$
\EndFor
\State \Return $P_F$
\EndFunction
\end{algorithmic}
\end{algorithm}

==> tables/VSAPN_2.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MastersSardina, Landmarks-EX-wInitial, RG09, LPBased, VSAPN) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{5}{*}{\rotatebox[origin=c]{90}{grid-world}}
 & A & .14 & .17 & .2 & .25 & .31 & .36 & .4 & .5 & .59 & .6 & 5.5\\
 & B & .09 & .09 & .09 & .08 & .13 & .13 & .22 & .35 & .66 & .83 & 13.0\\
 & C & .14 & .17 & .2 & .25 & .31 & .36 & .4 & .5 & .59 & .6 & 5.5\\
 & D & .1 & .11 & .13 & .16 & .2 & .22 & .25 & .32 & .37 & .37 & 7.6\\
 & E & \textbf{.21} & \textbf{.22} & \textbf{.27} & \textbf{.33} & \textbf{.46} & \textbf{.5} & \textbf{.64} & \textbf{.78} & \textbf{.96} & \textbf{.97} & \textbf{1.2} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{intrusion-detection}}
 & A & \textbf{.26} & \textbf{.45} & .59 & \textbf{.8} & \textbf{.83} & \textbf{.83} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.8\\
 & B & .22 & .4 & \textbf{.65} & .77 & .81 & .81 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.1} \\
 & C & \textbf{.26} & \textbf{.45} & .59 & \textbf{.8} & \textbf{.83} & \textbf{.83} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.8\\
 & D & .18 & .24 & .35 & .38 & .66 & .67 & .72 & .78 & .94 & .96 & 2.9\\
 & E & \textbf{.26} & \textbf{.45} & .59 & \textbf{.8} & \textbf{.83} & \textbf{.83} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.8\\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{kitchen}}
 & A & \textbf{.7} & .77 & .87 & \textbf{.87} & .67 & .67 & .8 & .9 & \textbf{.9} & \textbf{.9} & \textbf{1.2} \\
 & B & .58 & \textbf{.8} & \textbf{.9} & .8 & .8 & .83 & .73 & .8 & .8 & .8 & 1.3\\
 & C & .66 & .73 & .77 & .83 & .83 & .83 & .83 & \textbf{.93} & .8 & .8 & 1.4\\
 & E & \textbf{.7} & .77 & .87 & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & .87 & .77 & .77 & \textbf{1.2} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{logistics}}
 & A & .35 & .41 & .47 & .6 & .7 & .73 & .76 & \textbf{.89} & \textbf{.97} & \textbf{1.0} & \textbf{1.5} \\
 & B & .27 & .32 & .4 & .56 & .62 & .66 & .72 & .8 & .88 & .91 & 2.4\\
 & C & .34 & \textbf{.47} & \textbf{.58} & \textbf{.69} & \textbf{.72} & \textbf{.77} & \textbf{.8} & .82 & .93 & \textbf{1.0} & 1.9\\
 & D & .16 & .35 & .41 & .48 & .5 & .53 & .68 & .68 & .69 & .74 & 3.7\\
 & E & \textbf{.4} & \textbf{.47} & .56 & .64 & .66 & .73 & .76 & .88 & .95 & \textbf{1.0} & 1.6\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & .41 & .65 & .73 & \textbf{.84} & .88 & .86 & .89 & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.3\\
 & B & \textbf{.61} & \textbf{.77} & \textbf{.8} & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & C & .32 & .49 & .59 & .74 & .82 & .87 & .9 & .95 & \textbf{1.0} & \textbf{1.0} & 1.7\\
 & D & .24 & .43 & .58 & .57 & .76 & .8 & .82 & .86 & .95 & .93 & 2.0\\
 & E & .51 & .72 & .76 & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.4\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & .46 & .6 & .69 & .89 & .89 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & B & .46 & \textbf{.64} & \textbf{.8} & .88 & .88 & .91 & .95 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & C & .43 & .6 & .74 & \textbf{.91} & \textbf{.92} & .93 & .93 & .96 & .98 & .98 & 1.5\\
 & D & .31 & .48 & .64 & .67 & .7 & .74 & .81 & .84 & .91 & .93 & 2.0\\
 & E & \textbf{.51} & \textbf{.64} & .78 & .89 & .88 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.3\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{satellite}}
 & A & .35 & .31 & .36 & .43 & .59 & .66 & .74 & .81 & .81 & .81 & 2.4\\
 & B & .4 & .4 & .54 & .72 & \textbf{.8} & \textbf{.8} & \textbf{.89} & \textbf{.95} & .95 & \textbf{.96} & \textbf{1.6} \\
 & C & .35 & .35 & .42 & .54 & .64 & .62 & .67 & .71 & .74 & .77 & 2.7\\
 & D & .26 & .29 & .38 & .52 & .52 & .62 & .72 & .71 & .72 & .75 & 2.9\\
 & E & \textbf{.51} & \textbf{.47} & \textbf{.6} & \textbf{.73} & .79 & .78 & .85 & .93 & \textbf{.96} & \textbf{.96} & \textbf{1.6} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & \textbf{.28} & \textbf{.3} & .16 & .14 & .27 & .3 & .34 & .25 & .29 & .3 & \textbf{1.2} \\
 & B & .19 & .21 & .24 & .37 & .57 & .61 & .63 & .65 & .69 & \textbf{1.0} & 2.4\\
 & C & .15 & .22 & .32 & .45 & \textbf{.58} & .6 & .61 & \textbf{.68} & .73 & .8 & 2.7\\
 & D & .16 & .25 & \textbf{.36} & \textbf{.5} & .57 & \textbf{.63} & \textbf{.68} & .64 & \textbf{.83} & .87 & 1.9\\
 & E & .05 & .25 & \textbf{.36} & .46 & .5 & .57 & .61 & .5 & .71 & .82 & \textbf{1.2} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & .32 & .36 & \textbf{.57} & \textbf{.68} & .82 & \textbf{.95} & \textbf{.96} & \textbf{.98} & \textbf{1.0} & \textbf{1.0} & 1.2\\
 & B & .2 & .34 & .46 & .62 & \textbf{.83} & .93 & .95 & .96 & \textbf{1.0} & \textbf{1.0} & 1.6\\
 & C & .28 & .29 & .38 & .48 & .59 & .73 & .83 & .89 & .93 & .96 & 1.8\\
 & D & .22 & .3 & .42 & .52 & .6 & .65 & .85 & .92 & .95 & \textbf{1.0} & 2.4\\
 & E & \textbf{.33} & \textbf{.41} & .52 & .52 & .68 & .93 & \textbf{.96} & .96 & \textbf{1.0} & \textbf{1.0} & \textbf{1.1} \\
\hline
\end{tabular}
}
\end{table}

==> tables/adjusted_goals/longest_goals.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (PLR, VSAPN) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{2}{*}{\rotatebox[origin=c]{90}{average}}
 & A & .15 & .17 & .24 & .26 & .34 & .39 & .49 & .61 & .74 & .87 & 1.3\\
 & B & \textbf{.4} & \textbf{.55} & \textbf{.64} & \textbf{.7} & \textbf{.77} & \textbf{.82} & \textbf{.86} & \textbf{.88} & \textbf{.92} & \textbf{.95} & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{blocks-world}}
 & A & \textbf{.06} & .05 & .05 & .05 & .15 & .15 & .17 & .19 & .28 & .42 & 1.9\\
 & B & \textbf{.06} & \textbf{.19} & \textbf{.24} & \textbf{.31} & \textbf{.51} & \textbf{.58} & \textbf{.68} & \textbf{.81} & \textbf{.91} & \textbf{.91} & \textbf{1.5} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{campus}}
 & A & \textbf{.93} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & B & .7 & .97 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.1\\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{depots}}
 & A & .04 & .04 & .04 & .04 & .04 & .04 & .25 & .36 & .42 & .69 & 1.5\\
 & B & \textbf{.21} & \textbf{.29} & \textbf{.29} & \textbf{.39} & \textbf{.46} & \textbf{.68} & \textbf{.86} & \textbf{.86} & \textbf{.86} & \textbf{.89} & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & A & .05 & .05 & .08 & .08 & .08 & .19 & .26 & .46 & .6 & .71 & 1.3\\
 & B & \textbf{.5} & \textbf{.46} & \textbf{.54} & \textbf{.54} & \textbf{.55} & \textbf{.63} & \textbf{.64} & \textbf{.71} & \textbf{.89} & \textbf{.89} & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{dwr}}
 & A & .0 & .0 & .04 & .11 & .21 & .21 & .29 & .32 & .63 & \textbf{.87} & \textbf{1.0} \\
 & B & \textbf{.32} & \textbf{.36} & \textbf{.46} & \textbf{.57} & \textbf{.61} & \textbf{.61} & \textbf{.64} & \textbf{.64} & \textbf{.64} & .79 & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & .09 & .09 & .14 & .15 & .26 & .32 & .42 & .49 & .68 & \textbf{1.0} & 1.7\\
 & B & \textbf{.35} & \textbf{.37} & \textbf{.48} & \textbf{.51} & \textbf{.62} & \textbf{.67} & \textbf{.75} & \textbf{.76} & \textbf{.88} & .94 & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{ferry}}
 & A & .0 & .0 & .0 & .04 & .11 & .14 & .36 & .57 & .82 & .98 & 1.1\\
 & B & \textbf{.39} & \textbf{.82} & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{intrusion-detection}}
 & A & .29 & .37 & .68 & .7 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & B & \textbf{.79} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{logistics}}
 & A & .18 & .21 & .48 & .47 & .51 & .61 & .69 & .74 & .95 & .99 & 1.1\\
 & B & \textbf{.48} & \textbf{.84} & \textbf{.94} & \textbf{.94} & \textbf{.97} & \textbf{.99} & \textbf{.99} & \textbf{.99} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & .23 & .38 & .55 & .59 & .55 & .61 & .8 & .89 & \textbf{1.0} & .98 & \textbf{1.0} \\
 & B & \textbf{.59} & \textbf{.77} & \textbf{.88} & \textbf{.91} & \textbf{.95} & \textbf{.95} & \textbf{.95} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & .11 & .14 & .14 & .2 & .46 & .55 & .64 & .77 & .82 & .82 & \textbf{0.9} \\
 & B & \textbf{.54} & \textbf{.5} & \textbf{.71} & \textbf{.79} & \textbf{.96} & \textbf{.96} & \textbf{.96} & \textbf{.96} & \textbf{.96} & \textbf{.96} & 1.0\\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{satellite}}
 & A & .0 & .0 & .03 & .04 & .07 & .14 & .25 & .61 & .9 & .93 & 1.1\\
 & B & \textbf{.29} & \textbf{.36} & \textbf{.45} & \textbf{.64} & \textbf{.75} & \textbf{.86} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & .03 & .03 & .1 & .15 & .24 & .33 & .4 & .45 & .37 & .87 & 1.9\\
 & B & \textbf{.04} & \textbf{.23} & \textbf{.45} & \textbf{.49} & \textbf{.58} & \textbf{.65} & \textbf{.7} & \textbf{.68} & \textbf{.75} & \textbf{.89} & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & .04 & .04 & .04 & .04 & .14 & .18 & .32 & .68 & .82 & .89 & \textbf{1.0} \\
 & B & \textbf{.36} & \textbf{.59} & \textbf{.66} & \textbf{.75} & \textbf{.86} & \textbf{.89} & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{.96} & \textbf{1.0} \\
\hline
\end{tabular}
}
\end{table}

==> tables/adjusted_goals/original_goals.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (PLR, VSAPN) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{2}{*}{\rotatebox[origin=c]{90}{average}}
 & A & .31 & .33 & .39 & .42 & .5 & .55 & .65 & .72 & .8 & \textbf{.91} & 1.2\\
 & B & \textbf{.48} & \textbf{.55} & \textbf{.6} & \textbf{.65} & \textbf{.7} & \textbf{.74} & \textbf{.78} & \textbf{.83} & \textbf{.85} & .87 & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{blocks-world}}
 & A & .13 & .13 & .15 & .15 & .28 & .3 & .35 & .39 & .58 & .65 & \textbf{1.5} \\
 & B & \textbf{.15} & \textbf{.28} & \textbf{.27} & \textbf{.34} & \textbf{.53} & \textbf{.57} & \textbf{.61} & \textbf{.76} & \textbf{.79} & \textbf{.79} & 1.6\\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{campus}}
 & A & .93 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & B & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{depots}}
 & A & .16 & .19 & \textbf{.19} & .22 & .22 & .25 & .5 & .57 & .67 & \textbf{.84} & 1.4\\
 & B & \textbf{.21} & \textbf{.25} & .18 & \textbf{.32} & \textbf{.36} & \textbf{.43} & \textbf{.64} & \textbf{.71} & \textbf{.75} & .82 & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & A & .16 & .15 & .19 & .19 & .24 & .35 & .39 & .55 & .64 & .74 & 1.3\\
 & B & \textbf{.52} & \textbf{.46} & \textbf{.54} & \textbf{.61} & \textbf{.59} & \textbf{.68} & \textbf{.68} & \textbf{.84} & \textbf{.93} & \textbf{.93} & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{dwr}}
 & A & .39 & \textbf{.29} & .29 & \textbf{.36} & \textbf{.36} & .39 & \textbf{.43} & \textbf{.5} & \textbf{.61} & \textbf{.86} & \textbf{1.0} \\
 & B & \textbf{.43} & .25 & \textbf{.39} & \textbf{.36} & \textbf{.36} & \textbf{.43} & \textbf{.43} & .39 & .36 & .36 & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & .09 & .09 & .14 & .15 & .26 & .32 & .42 & .49 & .68 & \textbf{1.0} & 1.7\\
 & B & \textbf{.32} & \textbf{.37} & \textbf{.48} & \textbf{.51} & \textbf{.62} & \textbf{.67} & \textbf{.75} & \textbf{.78} & \textbf{.88} & .94 & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{ferry}}
 & A & .35 & .45 & .45 & .55 & .71 & .71 & .82 & .89 & .95 & .96 & \textbf{1.0} \\
 & B & \textbf{.75} & \textbf{.93} & \textbf{.93} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{intrusion-detection}}
 & A & .33 & .37 & .65 & .69 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & B & \textbf{.75} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{logistics}}
 & A & .21 & .31 & .49 & .55 & .56 & .62 & .78 & .78 & .94 & .99 & 1.1\\
 & B & \textbf{.5} & \textbf{.76} & \textbf{.88} & \textbf{.87} & \textbf{.87} & \textbf{.92} & \textbf{.94} & \textbf{.97} & \textbf{.98} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & .63 & .64 & .79 & .82 & .82 & .82 & .98 & \textbf{1.0} & \textbf{1.0} & .98 & \textbf{1.0} \\
 & B & \textbf{.82} & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & .21 & .25 & .29 & .36 & .48 & .55 & .79 & .84 & .86 & .86 & \textbf{0.9} \\
 & B & \textbf{.46} & \textbf{.63} & \textbf{.71} & \textbf{.92} & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{.96} & \textbf{.96} & \textbf{.96} & 1.0\\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{satellite}}
 & A & \textbf{.29} & \textbf{.29} & \textbf{.32} & .3 & .3 & .45 & .59 & .77 & \textbf{.92} & \textbf{.96} & 1.1\\
 & B & \textbf{.29} & \textbf{.29} & \textbf{.32} & \textbf{.41} & \textbf{.59} & \textbf{.68} & \textbf{.73} & \textbf{.86} & .89 & .89 & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & \textbf{.2} & \textbf{.2} & .24 & .28 & .36 & .41 & .45 & .53 & .46 & \textbf{.91} & 2.2\\
 & B & .14 & .18 & \textbf{.29} & \textbf{.29} & \textbf{.39} & \textbf{.54} & \textbf{.57} & \textbf{.54} & \textbf{.57} & .68 & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & .25 & .25 & .25 & .29 & .36 & .46 & .54 & \textbf{.82} & \textbf{.91} & \textbf{.93} & \textbf{1.0} \\
 & B & \textbf{.36} & \textbf{.43} & \textbf{.5} & \textbf{.5} & \textbf{.5} & \textbf{.54} & \textbf{.64} & .75 & .82 & .82 & \textbf{1.0} \\
\hline
\end{tabular}
}
\end{table}

==> tables/adjusted_goals/shortest_goals.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (PLR, VSAPN) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{2}{*}{\rotatebox[origin=c]{90}{average}}
 & A & .34 & .38 & .43 & .46 & .54 & .61 & .67 & .75 & \textbf{.82} & \textbf{.92} & 1.2\\
 & B & \textbf{.49} & \textbf{.56} & \textbf{.6} & \textbf{.64} & \textbf{.65} & \textbf{.68} & \textbf{.72} & \textbf{.78} & .82 & .85 & \textbf{1.1} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{blocks-world}}
 & A & .15 & .15 & .17 & .17 & .3 & .38 & .4 & .53 & \textbf{.72} & \textbf{.74} & \textbf{1.4} \\
 & B & \textbf{.18} & \textbf{.2} & \textbf{.22} & \textbf{.23} & \textbf{.4} & \textbf{.4} & \textbf{.43} & \textbf{.55} & .62 & .62 & 1.7\\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{campus}}
 & A & \textbf{.93} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & B & .7 & .97 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.1\\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{depots}}
 & A & .2 & .23 & \textbf{.23} & .27 & \textbf{.3} & \textbf{.36} & \textbf{.57} & \textbf{.61} & \textbf{.63} & \textbf{.86} & 1.3\\
 & B & \textbf{.25} & \textbf{.32} & .21 & \textbf{.32} & .29 & .32 & .5 & .5 & .61 & .68 & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & A & .17 & .19 & .27 & .37 & .48 & .59 & \textbf{.59} & .6 & .74 & .76 & 1.3\\
 & B & \textbf{.55} & \textbf{.5} & \textbf{.59} & \textbf{.63} & \textbf{.6} & \textbf{.6} & .5 & \textbf{.68} & \textbf{.8} & \textbf{.83} & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{dwr}}
 & A & .43 & \textbf{.39} & \textbf{.43} & \textbf{.43} & \textbf{.43} & \textbf{.46} & \textbf{.43} & \textbf{.5} & \textbf{.63} & \textbf{.84} & \textbf{1.0} \\
 & B & \textbf{.46} & .36 & .39 & .32 & .32 & .36 & .36 & .36 & .39 & .46 & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & .09 & .09 & .14 & .15 & .26 & .32 & .42 & .49 & .68 & \textbf{1.0} & 1.7\\
 & B & \textbf{.32} & \textbf{.37} & \textbf{.48} & \textbf{.51} & \textbf{.6} & \textbf{.65} & \textbf{.72} & \textbf{.76} & \textbf{.86} & .94 & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{ferry}}
 & A & .38 & .52 & .52 & .59 & .71 & .75 & .79 & .96 & .95 & .96 & \textbf{1.0} \\
 & B & \textbf{.75} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{intrusion-detection}}
 & A & .33 & .37 & .63 & .66 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & B & \textbf{.76} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{logistics}}
 & A & .3 & .47 & .54 & .59 & .62 & .67 & .77 & .86 & .98 & .99 & 1.1\\
 & B & \textbf{.57} & \textbf{.76} & \textbf{.86} & \textbf{.88} & \textbf{.76} & \textbf{.83} & \textbf{.91} & \textbf{.93} & \textbf{.99} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & .7 & .73 & .88 & .86 & .84 & .89 & .91 & .96 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & B & \textbf{.95} & \textbf{.95} & \textbf{.95} & \textbf{.95} & \textbf{.98} & \textbf{.98} & \textbf{.98} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & .29 & .32 & .36 & .45 & .48 & .55 & .71 & .82 & .86 & .86 & \textbf{0.9} \\
 & B & \textbf{.5} & \textbf{.58} & \textbf{.75} & \textbf{.88} & \textbf{.92} & \textbf{.96} & \textbf{1.0} & \textbf{.96} & \textbf{.96} & \textbf{.96} & 1.0\\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{satellite}}
 & A & .25 & .25 & .28 & .27 & .3 & \textbf{.57} & \textbf{.75} & .89 & \textbf{.96} & \textbf{.96} & 1.1\\
 & B & \textbf{.39} & \textbf{.32} & \textbf{.38} & \textbf{.45} & \textbf{.48} & \textbf{.57} & .64 & \textbf{.93} & .93 & .93 & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & \textbf{.25} & \textbf{.25} & .26 & .26 & .35 & .35 & .38 & \textbf{.47} & .48 & \textbf{.93} & 2.2\\
 & B & .21 & .18 & \textbf{.32} & \textbf{.36} & \textbf{.36} & \textbf{.46} & \textbf{.46} & .46 & \textbf{.54} & .68 & \textbf{1.0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & \textbf{.32} & .32 & \textbf{.36} & \textbf{.39} & \textbf{.46} & \textbf{.63} & \textbf{.66} & \textbf{.84} & \textbf{.91} & \textbf{.92} & \textbf{1.0} \\
 & B & \textbf{.32} & \textbf{.36} & \textbf{.36} & \textbf{.39} & .36 & .46 & .57 & .75 & .82 & .82 & \textbf{1.0} \\
\hline
\end{tabular}
}
\end{table}

==> tables/computationTimeTable.tex <==
\begin{table}
\caption{Comparison among average required computation time \emph{per possible goal} in seconds for different approaches and different values of $t$ when applied to the \emph {CMU dataset}.}
\label{tab:computationTimes}
\begin{tabular}{c||ccccc}
                 & MS    & PLR   & VSG   & VSM   & VSA   \\ \hline \hline
$t = 0$            & 25.3  & 169.5 & \textbf{0.786} & 63.3  & 68.8  \\
$t > 0$ & 21.95 & 0.008  & \textbf{0.001} & \textbf{0.001} & \textbf{0.001}
\end{tabular}
\end{table}

==> tables/evaluationTable.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MS(A), PLR(B), RG09(C), VSG(D), VSA(E), VSM(F)) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{T} reports the average computation time in seconds per goal per observation step for $t=0(t_1)$ and $t>0(t_2)$. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}
\label{tab:benchmarkEvaluation}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|ll|l}
\multicolumn{1}{c}{}                 & \multicolumn{1}{c|}{} & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}                          & \multicolumn{2}{c|}{\textbf{T}} & \textbf{S} \\
                                     &                                   & .1 & .2 & .3 & .4 & .5 & .6 & .7 & .8 & .9 & 1      & $t_1$   & $t_2$              &  \\ \hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{block-worlds}} & A                    &.65             &.63            &.61            &.62            &.69        &.71   &.73   &.74   &.78   &.79      & 6.8         & 9.3              & 7.17   \\
                                                        & B                   &.2           &.27                &.23            &.37            &.55        &.68   &.75   &.8   &.97   &\textbf{1.0}         & .05         & \textbf{0}              & \textbf{1.62}    \\
                                                        & C                  &\textbf{.86}   &\textbf{.73}   &\textbf{.65}   &\textbf{.68}   &\textbf{.71}   &\textbf{.86}   &\textbf{.9}   &\textbf{.9}   &.97   &\textbf{1.0}          & \textbf{0}         & .36              & 4.63    \\
                                                        & D                   &\textbf{.86}   &\textbf{.73}   &\textbf{.65}   &\textbf{.68}   &\textbf{.71}   &.84   &.88   &.88   &\textbf{1.0}   &\textbf{1.0}       & \textbf{0}         & \textbf{0}              & 4.61    \\
                                                        & E                   &\textbf{.86}   &\textbf{.73}   &\textbf{.65}   &\textbf{.68}   &\textbf{.71}   &.84   &.88   &.88   &\textbf{1.0}   &\textbf{1.0}       & .03         & \textbf{0}              & 4.61    \\
                                                        & F                   &\textbf{.86}   &\textbf{.73}   &\textbf{.65}   &\textbf{.68}   &\textbf{.71}   &.84   &.88   &.88   &\textbf{1.0}   &\textbf{1.0}       & .03         & \textbf{0}              & 4.61    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{depots}}       & A                    &.36   &.25   &.25   &.32   &.46   &.54   &.5   &.57   &.61   &.61       & 4.8         & 4.6              & 1.88    \\
                                                        & B                   &.14   &.21   &.21   &.29   &.46   &.75   &.86   &.96   &\textbf{1.0 }  &\textbf{1.0}       & .13         & \textbf{0}              & \textbf{1.37}    \\
                                                        & C                  &\textbf{.82}   &\textbf{.79}   &.57   &.68   &.79   &.86   &.79   &.82   &.75   &.93        & \textbf{0}         & .53              & 2.87   \\
                                                        & D                   &.64   &.5   &.54   &.43   &.57   &.64   &.75   &.79   &.89   &.93        & .01         & \textbf{0}              & 2.63    \\
                                                        & E                   &.71   &.75   &\textbf{.79}   &\textbf{.71}   &\textbf{.89}   &\textbf{.96}   &\textbf{.96}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}       & .03         & \textbf{0}              & 3.09    \\
                                                        & F                   &.68   &.61   &.68   &.68   &.75   &.82   &.86   &.89   &.93   &.93       & .03         & \textbf{0}              & 2.86    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{driverlog}}    & A                    &.46   &.54   &.64   &.79   &.86   &.93   &\textbf{.96}   &.93   &.93   &\textbf{1.0}      & .1         & .14              & \textbf{1.48}    \\
                                                        & B                   &.82   &.75   &.82   &.86   &.89   &.86   &.93   &\textbf{.96}   &\textbf{.96}   &\textbf{1.0}       & .51         & \textbf{0}              & 2.52    \\
                                                        & C                  &\textbf{1.0}   &\textbf{.96}   &\textbf{.96}   &\textbf{.96}   &\textbf{.92}   &\textbf{.96}   &\textbf{.96}   &\textbf{.96}   &\textbf{.96}   &.96        & \textbf{0}         & .27              & 3.04    \\
                                                        & D                   &.82   &.79   &.86   &.79   &.79   &.82   &.89   &.89   &.93   &.93       & .01         & \textbf{0}              & 2.76    \\
                                                        & E                   &.86   &.75   &.75   &.71   &.75   &.75   &.82   &.86   &.89   &.93       & .04         & \textbf{0}              & 2.72    \\
                                                        & F                   &.86   &.71   &.71   &.71   &.79   &.82   &.86   &.86   &.86   &.89       & .04         & \textbf{0}              & 2.57    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{dwr}}          & A                    &.36   &.39   &.39   &.57   &.57   &.64   &.64   &.71   &.75   &.79      & 3.9         & 3.4              & 2.08    \\
                                                        & B                   &.5   &.61   &.61   &.57   &.61   &.61   &.68   &\textbf{.79}   &\textbf{.89}   &\textbf{1.0}        & .14         & \textbf{0}              & \textbf{1.22}    \\
                                                        & C                  &.88   &\textbf{.82}   &.78   &.63   &.5   &.55   &.6   &.57   &.57   &.63          & \textbf{0}         & 1.6              & 2.81    \\
                                                        & D                   &.82   &\textbf{.82}   &\textbf{.79}   &.54   &.61   &.61   &.57   &.64   &.68   &.82       & .01         & \textbf{0}              & 2.57    \\
                                                        & E                   &.79   &.75   &.75   &\textbf{.64}  &\textbf{.71}   &\textbf{.68}   &\textbf{.68}   &.75   &\textbf{.89}   &.89       & .05         & \textbf{0}              & 2.21    \\
                                                        & F                   &\textbf{.89}   &.79   &.71   &.57   &.5   &.64   &.57   &.68   &.86   &.93        & .05         & \textbf{0}              & 2.57    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}} & A                    &.7   &.85   &.89   &.96   &.9   &.92   &.94   &.94   &.94   &.94       & .01         & .01              & 2.61    \\
                                                         & B                   &.39   &.4   &.42   &.46   &.43   &.5   &.56   &.61   &.7   &\textbf{1.0}         & .54         & \textbf{0}              & \textbf{1.76}    \\
                                                         & C                  &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}       & \textbf{0}         & .54              & 3.16    \\
                                                         & D                   &.95   &.92   &.93   &.91   &.89   &.89   &.89   &.89   &.9   &.93       & .04         & \textbf{0}              & 3.06    \\
                                                         & E                   &.87   &.84   &.86   &.84   &.84   &.86   &.89   &.89   &.9   &.93       & .07         & \textbf{0}              & 2.85    \\
                                                         & F                   &.89   &.85   &.87   &.85   &.85   &.85   &.88   &.88   &.9   &.93       & .06         & \textbf{0}              & 2.82    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{ferry}}    & A                    &.71   &.89   &.89   &.89   &.93   &.96   &.93   &\textbf{.96}   &\textbf{.96}   &\textbf{.96}          & .02         & .01              & 1.28    \\
                                                    & B                   &.64   &.79   &.86   &.93   &.93   &.96   &.96   &\textbf{.96}   &\textbf{.96}   &\textbf{.96}           & .09         & \textbf{0}              & \textbf{1.23}    \\
                                                    & C                  &\textbf{1.0}   &\textbf{1.0}   &\textbf{.96}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{.96}   &\textbf{.96}   &\textbf{.96}            & \textbf{0}         & .33              & 1.77    \\
                                                    & D                   &\textbf{1.0}   &\textbf{1.0}   &\textbf{.96}   &.96   &.96   &.96   &.96   &\textbf{.96}   &\textbf{.96}   &\textbf{.96}           & .01         & \textbf{0}              & 1.71    \\
                                                    & E                   &\textbf{1.0}   &\textbf{1.0}   &\textbf{.96}   &.96   &.96   &.96   &.96   &\textbf{.96}   &\textbf{.96}   &\textbf{.96}           & .02         & \textbf{0}              & 1.71    \\
                                                    & F                   &\textbf{1.0}   &\textbf{1.0}   &\textbf{.96}   &.96   &.96   &.96   &.96   &\textbf{.96}   &\textbf{.96}   &\textbf{.96}           & .02         & \textbf{0}              & 1.71    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{\scriptsize{intrusion-detection}}} & A                    &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}      & .01         & .01              & 1.95    \\
                                                                            & B                   &.24   &.42   &.76   &.88   &.91   &.91   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}      & .03         & \textbf{0}              & \textbf{1.12}    \\
                                                                            & C                  &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}     & \textbf{0}         & .11              & 1.95    \\
                                                                            & D                   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}      & \textbf{0}         & \textbf{0}              & 1.95    \\
                                                                            & E                   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}      & .01         & \textbf{0}              & 1.95    \\
                                                                            & F                   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}      & .01         & \textbf{0}              & 1.95    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{logistics}}    & A                    &.73   &.72   &.72   &.75   &.82   &.85   &.85   &.94   &\textbf{1.0}   &\textbf{1.0}      & .02           & .01              & \textbf{1.55}    \\
                                                        & B                   &.45   &.47   &.53   &.63   &.6   &.7   &.8   &.95   &\textbf{1.0}   &\textbf{1.0}          & .15           & \textbf{0}              & 1.73    \\
                                                        & C                  &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}        & \textbf{0}             & .57              & 2.09    \\
                                                        & D                   &.95   &.95   &.95   &.92   &.94   &.94   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}       & .01           & \textbf{0}              & 2.04    \\
                                                        & E                   &.9   &.93   &.95   &.92   &.92   &.92   &.97   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}        & .06           & \textbf{0}              & 1.95    \\
                                                        & F                   &.88   &.85   &.82   &.84   &.84   &.84   &.92   &.97   &\textbf{1.0}   &\textbf{1.0}       & .06           & \textbf{0}              & 1.92    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{miconic}}      & A                    &.86   &.89   &.93   &.96   &.93   &.93   &.96   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}      & .02           & .02              & 1.39    \\
                                                        & B                   &.75   &.93   &.93   &.93   &.96   &.96   &.96   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}       & 1.64          & \textbf{0}              & \textbf{1.18}    \\
                                                        & C                  &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}        & \textbf{0}             & .53              & 1.81    \\
                                                        & D                   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}       & .02           & \textbf{0}              & 1.52    \\
                                                        & E                   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}       & .07           & \textbf{0}              & 1.52    \\
                                                        & F                   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}       & .08           & \textbf{0}              & 1.52    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{rovers}}       & A                    &.71   &.82   &.86   &.96   &.96   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}      & .02         & .02              & \textbf{1.29}    \\
                                                        & B                   &.86   &.86   &.89   &.93   &.93   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}       & 1.03         & \textbf{0}              & 1.4    \\
                                                        & C                  &.96   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}        & \textbf{0}         & .26              & 1.62    \\
                                                        & D                   &\textbf{1.0}   &.93   &.96   &.96   &.96   &.96   &.96   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}       & .01         & \textbf{0}              & 1.63    \\
                                                        & E                   &.96   &.93   &.93   &.96   &.93   &.96   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}       & .11         & \textbf{0}              & 1.52    \\
                                                        & F                   &.96   &.86   &.89   &.93   &.93   &.96   &.93   &.93   &.93   &.93       & .11         & \textbf{0}              & 1.61    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{satellite}}    & A                    &.75   &.71   &.75   &.79   &.86   &.89   &\textbf{.96}   &\textbf{.96}   &\textbf{.96}   &\textbf{.96}      & .02         & .01              & 2.46    \\
                                                        & B                   &\textbf{.96}   &\textbf{.96}   &\textbf{.96}   &.93   &.93   &.93   &.89   &.93   &.93   &.93       & .26         & \textbf{0}              & 2.09    \\
                                                        & C                  &\textbf{.96}   &.93   &.93   &.96   &\textbf{.96}   &.93   &.93   &.93   &.93   &.93        & \textbf{0}         & .22              & 2.74    \\
                                                        & D                   &\textbf{.96}   &.92   &\textbf{.96}   &\textbf{.96}   &\textbf{.96}   &\textbf{.96}   &\textbf{.96}   &\textbf{.96}   &\textbf{.96}   &\textbf{.96}       & .01         & \textbf{0}              & 2.05    \\
                                                        & E                   &.75   &.64   &.64   &.64   &.61   &.75   &.68   &.75   &.75   &.79       & \textbf{0}              & \textbf{0}        & 1.8    \\
                                                        & F                   &.75   &.68   &.57   &.61   &.64   &.68   &.79   &.82   &.82   &.86       & \textbf{0}              & \textbf{0}       & \textbf{1.71}    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{sokoban}}      & A                    &.46   &.32   &.18   &.14   &.29   &.32   &.36   &.25   &.29   &.36      & .05         & .04              & \textbf{1.26}    \\
                                                        & B                   &.68   &.61   &.46   &.54   &.61   &.68   &.79   &.79   &\textbf{.86}   &\textbf{1.0}       & 1.27        & \textbf{0}              & 2.14    \\
                                                        & C                  &\textbf{1.0}   &\textbf{.86}   &\textbf{.79}   &\textbf{.86}   &\textbf{.89}   &\textbf{.86}   &\textbf{.86}   &\textbf{.86}   &\textbf{.86}   &.89        & \textbf{0}         & 1.02              & 2.9    \\
                                                        & D                   &.5   &.54   &.63   &.58   &.63   &.67   &.58   &.63   &.58   &.67        & .03         & \textbf{0}              & 2.21    \\
                                                        & E                   &.5   &.32   &.5   &.5   &.5   &.54   &.54   &.57   &.61   &.64           & \textbf{0}              & \textbf{0}           & 1.81    \\
                                                        & F                   &.64   &.39   &.54   &.5   &.46   &.5   &.5   &.57   &.64   &.71          & \textbf{0}              & \textbf{0}          & 1.92    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{zeno-travel}}  & A                    &.46   &.43   &.68   &.75   &.89   &\textbf{.96}   &\textbf{.96}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}      & .02         & .02              & \textbf{1.26}    \\
                                                        & B                   &\textbf{.89}   &\textbf{.93}   &\textbf{.96}   &.93   &.96   &.96   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}       & 2.8         & \textbf{0}              & 2.24    \\
                                                        & C                  &.86   &.64   &.64   &.71   &.79   &.89   &.93   &\textbf{1.0}   &\textbf{1.0}   &\textbf{1.0}        & \textbf{0}         & .39              & 1.98    \\
                                                        & D                   &.68   &.75   &.82   &.79   &.86   &.86   &.89   &.86   &.93   &.96       & .01         & \textbf{0}              & 1.79    \\
                                                        & E                   &.57   &.36   &.57   &.57   &.68   &.75   &.75   &.68   &.75   &.82       & .05         & \textbf{0}              & 1.63    \\
                                                        & F                   &.54   &.46   &.54   &.54   &.61   &.68   &.71   &.68   &.71   &.86       & .06         & \textbf{0}              & 1.66   
\end{tabular}
}
\end{table}

==> tables/evaluationTable_EX_landmarks.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MastersSardina, Landmarks-VSX-wInitial, RG09, LPPLRased, VRL10-woVSctions) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{5}{*}{\rotatebox[origin=c]{90}{blocks-world}}
 & MS & .1 & .13 & .14 & .24 & .29 & .36 & .41 & .47 & .54 & .55 & 7.1\\
 & PLR & .09 & .23 & \textbf{.28} & \textbf{.32} & \textbf{.43} & \textbf{.56} & \textbf{.62} & \textbf{.71} & \textbf{.85} & \textbf{.92} & \textbf{1.5} \\
 & RG09 & .08 & .22 & .23 & .29 & .38 & .42 & .53 & .63 & .81 & .9 & 4.1\\
 & LP & .06 & .13 & .15 & .2 & .33 & .38 & .46 & .52 & .76 & .81 & 5.4\\
 & VS & \textbf{.12} & \textbf{.27} & .18 & .27 & .36 & .39 & .53 & .59 & .77 & .87 & 2.5\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{depots}}
 & VS & \textbf{.21} & .16 & .16 & .22 & .38 & .49 & .48 & .54 & .59 & .59 & 1.8\\
 & PLR & .13 & .17 & .24 & .27 & .33 & .42 & .75 & .83 & .91 & .93 & 1.9\\
 & RG09 & .16 & \textbf{.29} & .28 & \textbf{.32} & .45 & .62 & .59 & .6 & .61 & .78 & 2.6\\
 & LP & .09 & .16 & .17 & .27 & .34 & .44 & .57 & .69 & .75 & .89 & 2.4\\
 & VS & .19 & .18 & \textbf{.29} & .23 & \textbf{.5} & \textbf{.7} & \textbf{.86} & \textbf{.86} & \textbf{.96} & \textbf{.96} & \textbf{1.4} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & VS & \textbf{.29} & \textbf{.37} & \textbf{.5} & \textbf{.63} & \textbf{.73} & \textbf{.84} & \textbf{.92} & \textbf{.91} & \textbf{.91} & \textbf{.96} & 1.4\\
 & PLR & .19 & .33 & .42 & .54 & .64 & .71 & .75 & .84 & .88 & .92 & \textbf{1.3} \\
 & RG09 & .22 & .27 & .35 & .46 & .52 & .6 & .75 & .77 & .81 & .81 & 2.9\\
 & LP & .2 & .26 & .37 & .5 & .58 & .68 & .67 & .68 & .76 & .8 & 2.3\\
 & VS & .19 & .19 & .29 & .36 & .45 & .52 & .68 & .79 & .79 & .79 & 1.7\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{dwr}}
 & VS & .13 & .23 & .2 & .34 & .34 & .39 & .43 & .47 & .46 & .55 & 2.0\\
 & PLR & \textbf{.36} & \textbf{.38} & \textbf{.46} & \textbf{.54} & \textbf{.52} & \textbf{.5} & \textbf{.66} & \textbf{.77} & \textbf{.91} & \textbf{1.0} & \textbf{1.2} \\
 & RG09 & .25 & .33 & .32 & .26 & .2 & .22 & .3 & .27 & .31 & .41 & 2.7\\
 & LP & .19 & .18 & .24 & .29 & .28 & .33 & .51 & .51 & .65 & .81 & 2.0\\
 & VS & .22 & .24 & .3 & .26 & .26 & .32 & .39 & .43 & .46 & .57 & \textbf{1.2} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & VS & .29 & .32 & .44 & \textbf{.52} & .56 & .63 & \textbf{.71} & .76 & .83 & .94 & 2.4\\
 & PLR & .09 & .09 & .14 & .15 & .26 & .32 & .42 & .51 & .68 & \textbf{1.0} & \textbf{1.6} \\
 & RG09 & \textbf{.32} & .34 & \textbf{.45} & .48 & .57 & .63 & .69 & \textbf{.78} & \textbf{.85} & \textbf{1.0} & 3.0\\
 & LP & .13 & .24 & .28 & .35 & .39 & .47 & .5 & .57 & .7 & .78 & 3.3\\
 & VS & \textbf{.32} & \textbf{.38} & .43 & .5 & \textbf{.6} & \textbf{.64} & .69 & .76 & .84 & .93 & 2.6\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{ferry}}
 & VS & \textbf{.38} & \textbf{.7} & \textbf{.8} & .83 & .89 & .95 & .93 & .96 & .96 & .96 & \textbf{1.2} \\
 & PLR & .37 & .56 & .7 & .82 & .88 & .95 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & RG09 & .28 & .58 & .73 & .8 & .89 & .91 & .95 & .96 & .96 & .96 & 1.6\\
 & LP & .19 & .34 & .54 & .75 & .85 & .88 & .91 & .91 & .93 & .96 & 2.1\\
 & VS & .28 & .57 & .76 & \textbf{.89} & \textbf{.96} & \textbf{.96} & .98 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.5\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{logistics}}
 & VS & .35 & .41 & .47 & .6 & .7 & .73 & .76 & \textbf{.89} & \textbf{.97} & \textbf{1.0} & \textbf{1.5} \\
 & PLR & .27 & .32 & .4 & .56 & .62 & .66 & .72 & .8 & .88 & .91 & 2.4\\
 & RG09 & .34 & .47 & .58 & .69 & .72 & \textbf{.77} & \textbf{.8} & .82 & .93 & \textbf{1.0} & 1.9\\
 & LP & .16 & .35 & .41 & .48 & .5 & .53 & .68 & .68 & .69 & .74 & 3.7\\
 & VS & \textbf{.38} & \textbf{.54} & \textbf{.65} & \textbf{.71} & \textbf{.73} & .76 & .79 & .87 & .95 & \textbf{1.0} & 1.6\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{miconic}}
 & VS & .41 & .65 & .73 & \textbf{.84} & .88 & .86 & .89 & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.3\\
 & PLR & \textbf{.61} & \textbf{.77} & \textbf{.8} & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & RG09 & .32 & .49 & .59 & .74 & .82 & .87 & .9 & .95 & \textbf{1.0} & \textbf{1.0} & 1.7\\
 & LP & .24 & .43 & .58 & .57 & .76 & .8 & .82 & .86 & .95 & .93 & 2.0\\
 & VS & .51 & .72 & .76 & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.4\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{rovers}}
 & VS & .46 & .6 & .69 & .89 & .89 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & PLR & .46 & \textbf{.64} & .8 & .88 & .88 & .91 & .95 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & RG09 & .43 & .6 & .74 & \textbf{.91} & \textbf{.92} & .93 & .93 & .96 & .98 & .98 & 1.5\\
 & LP & .31 & .48 & .64 & .67 & .7 & .74 & .81 & .84 & .91 & .93 & 2.0\\
 & VS & \textbf{.51} & .62 & \textbf{.83} & .9 & .88 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{satellite}}
 & VS & .35 & .31 & .36 & .43 & .59 & .66 & .74 & .81 & .81 & .81 & 2.4\\
 & PLR & .4 & \textbf{.4} & \textbf{.54} & \textbf{.72} & \textbf{.8} & .8 & \textbf{.89} & \textbf{.95} & \textbf{.95} & \textbf{.96} & \textbf{1.6} \\
 & RG09 & .35 & .35 & .42 & .54 & .64 & .62 & .67 & .71 & .74 & .77 & 2.7\\
 & LP & .26 & .29 & .38 & .52 & .52 & .62 & .72 & .71 & .72 & .75 & 2.9\\
 & VS & \textbf{.44} & .39 & .52 & .71 & .76 & \textbf{.81} & .88 & .92 & .93 & .95 & 1.9\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & VS & \textbf{.28} & \textbf{.3} & .16 & .14 & .27 & .3 & .34 & .25 & .29 & .3 & 1.2\\
 & PLR & .19 & .21 & .24 & .37 & .57 & .61 & .63 & .65 & .69 & \textbf{1.0} & 2.4\\
 & RG09 & .15 & .22 & .32 & .45 & \textbf{.58} & .6 & .61 & \textbf{.68} & .73 & .8 & 2.7\\
 & LP & .16 & .25 & \textbf{.36} & \textbf{.5} & .57 & \textbf{.63} & \textbf{.68} & .64 & \textbf{.83} & .87 & 1.9\\
 & VS & .05 & .25 & .3 & .46 & .57 & .5 & .46 & .43 & .57 & .79 & \textbf{1.1} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & VS & .32 & .36 & .57 & .68 & .82 & .95 & .96 & .98 & \textbf{1.0} & \textbf{1.0} & 1.2\\
 & PLR & .2 & .34 & .46 & .62 & .83 & .93 & .95 & .96 & \textbf{1.0} & \textbf{1.0} & 1.6\\
 & RG09 & .28 & .29 & .38 & .48 & .59 & .73 & .83 & .89 & .93 & .96 & 1.8\\
 & LP & .22 & .3 & .42 & .52 & .6 & .65 & .85 & .92 & .95 & \textbf{1.0} & 2.4\\
 & VS & \textbf{.45} & \textbf{.68} & \textbf{.8} & \textbf{.86} & \textbf{.95} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.1} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{average}}
 & VS & .3 & .38 & .44 & .53 & .61 & .68 & .71 & .75 & .78 & .81 & 2.1\\
 & PLR & .28 & .37 & .46 & .55 & .64 & .69 & \textbf{.77} & \textbf{.83} & \textbf{.9} & \textbf{.97} & \textbf{1.6} \\
 & RG09 & .27 & .37 & .45 & .54 & .61 & .66 & .71 & .75 & .81 & .86 & 2.4\\
 & LP & .18 & .28 & .38 & .47 & .54 & .6 & .68 & .71 & .8 & .86 & 2.7\\
 & VS & \textbf{.31} & \textbf{.42} & \textbf{.51} & \textbf{.58} & \textbf{.66} & \textbf{.71} & .76 & .8 & .86 & .9 & \textbf{1.6} \\
\hline
\end{tabular}
}
\end{table}

==> tables/evaluationTable_EX_landmarks_woInitial.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MastersSardina, Landmarks-EX-woInitial, RG09, LPBased, VRL10-woActions) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{5}{*}{\rotatebox[origin=c]{90}{blocks-world}}
 & A & .1 & .13 & .14 & .24 & .29 & .36 & .41 & .47 & .54 & .55 & 7.1\\
 & B & .11 & \textbf{.29} & \textbf{.27} & \textbf{.35} & \textbf{.44} & \textbf{.56} & \textbf{.62} & \textbf{.72} & \textbf{.85} & \textbf{.92} & \textbf{1.6} \\
 & C & .08 & .22 & .23 & .29 & .38 & .42 & .53 & .63 & .81 & .9 & 4.1\\
 & D & .06 & .13 & .15 & .2 & .33 & .38 & .46 & .52 & .76 & .81 & 5.4\\
 & E & \textbf{.12} & .27 & .18 & .27 & .36 & .39 & .53 & .59 & .77 & .87 & 2.5\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{depots}}
 & A & \textbf{.21} & .16 & .16 & .22 & .38 & .49 & .48 & .54 & .59 & .59 & 1.8\\
 & B & .13 & .17 & .24 & .27 & .38 & .47 & .79 & .85 & .91 & .93 & 1.8\\
 & C & .16 & \textbf{.29} & .28 & \textbf{.32} & .45 & .62 & .59 & .6 & .61 & .78 & 2.6\\
 & D & .09 & .16 & .17 & .27 & .34 & .44 & .57 & .69 & .75 & .89 & 2.4\\
 & E & .19 & .18 & \textbf{.29} & .23 & \textbf{.5} & \textbf{.7} & \textbf{.86} & \textbf{.86} & \textbf{.96} & \textbf{.96} & \textbf{1.4} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & A & \textbf{.29} & \textbf{.37} & \textbf{.5} & \textbf{.63} & \textbf{.73} & \textbf{.84} & \textbf{.92} & \textbf{.91} & \textbf{.91} & \textbf{.96} & \textbf{1.4} \\
 & B & .21 & .35 & .44 & .59 & .67 & .74 & .78 & .81 & .89 & .92 & 2.1\\
 & C & .22 & .27 & .35 & .46 & .52 & .6 & .75 & .77 & .81 & .81 & 2.9\\
 & D & .2 & .26 & .37 & .5 & .58 & .68 & .67 & .68 & .76 & .8 & 2.3\\
 & E & .19 & .19 & .29 & .36 & .45 & .52 & .68 & .79 & .79 & .79 & 1.7\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{dwr}}
 & A & .13 & .23 & .2 & .34 & .34 & .39 & .43 & .47 & .46 & .55 & 2.0\\
 & B & \textbf{.38} & \textbf{.46} & \textbf{.5} & \textbf{.54} & \textbf{.52} & \textbf{.52} & \textbf{.63} & \textbf{.77} & \textbf{.91} & \textbf{1.0} & \textbf{1.2} \\
 & C & .25 & .33 & .32 & .26 & .2 & .22 & .3 & .27 & .31 & .41 & 2.7\\
 & D & .19 & .18 & .24 & .29 & .28 & .33 & .51 & .51 & .65 & .81 & 2.0\\
 & E & .22 & .24 & .3 & .26 & .26 & .32 & .39 & .43 & .46 & .57 & \textbf{1.2} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & .29 & .32 & .44 & \textbf{.52} & .56 & .63 & \textbf{.71} & .76 & .83 & .94 & 2.4\\
 & B & .18 & .25 & .32 & .35 & .4 & .43 & .46 & .59 & .72 & \textbf{1.0} & \textbf{1.8} \\
 & C & \textbf{.32} & .34 & \textbf{.45} & .48 & .57 & .63 & .69 & \textbf{.78} & \textbf{.85} & \textbf{1.0} & 3.0\\
 & D & .13 & .24 & .28 & .35 & .39 & .47 & .5 & .57 & .7 & .78 & 3.3\\
 & E & \textbf{.32} & \textbf{.38} & .43 & .5 & \textbf{.6} & \textbf{.64} & .69 & .76 & .84 & .93 & 2.6\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{ferry}}
 & A & .38 & \textbf{.7} & \textbf{.8} & .83 & .89 & .95 & .93 & .96 & .96 & .96 & \textbf{1.2} \\
 & B & \textbf{.42} & .62 & .7 & .82 & .91 & \textbf{.98} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & C & .28 & .58 & .73 & .8 & .89 & .91 & .95 & .96 & .96 & .96 & 1.6\\
 & D & .19 & .34 & .54 & .75 & .85 & .88 & .91 & .91 & .93 & .96 & 2.1\\
 & E & .28 & .57 & .76 & \textbf{.89} & \textbf{.96} & .96 & .98 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.5\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{logistics}}
 & A & .35 & .41 & .47 & .6 & .7 & .73 & .76 & \textbf{.89} & \textbf{.97} & \textbf{1.0} & \textbf{1.5} \\
 & B & .29 & .35 & .45 & .58 & .63 & .69 & .72 & .8 & .88 & .91 & 2.4\\
 & C & .34 & .47 & .58 & .69 & .72 & \textbf{.77} & \textbf{.8} & .82 & .93 & \textbf{1.0} & 1.9\\
 & D & .16 & .35 & .41 & .48 & .5 & .53 & .68 & .68 & .69 & .74 & 3.7\\
 & E & \textbf{.38} & \textbf{.54} & \textbf{.65} & \textbf{.71} & \textbf{.73} & .76 & .79 & .87 & .95 & \textbf{1.0} & 1.6\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & .41 & .65 & .73 & \textbf{.84} & .88 & .86 & .89 & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.3\\
 & B & \textbf{.61} & \textbf{.77} & \textbf{.8} & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & C & .32 & .49 & .59 & .74 & .82 & .87 & .9 & .95 & \textbf{1.0} & \textbf{1.0} & 1.7\\
 & D & .24 & .43 & .58 & .57 & .76 & .8 & .82 & .86 & .95 & .93 & 2.0\\
 & E & .51 & .72 & .76 & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.4\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & .46 & .6 & .69 & .89 & .89 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & B & .41 & .59 & .77 & .88 & .88 & .91 & .95 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.3\\
 & C & .43 & .6 & .74 & \textbf{.91} & \textbf{.92} & .93 & .93 & .96 & .98 & .98 & 1.5\\
 & D & .31 & .48 & .64 & .67 & .7 & .74 & .81 & .84 & .91 & .93 & 2.0\\
 & E & \textbf{.51} & \textbf{.62} & \textbf{.83} & .9 & .88 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{satellite}}
 & A & .35 & .31 & .36 & .43 & .59 & .66 & .74 & .81 & .81 & .81 & 2.4\\
 & B & .41 & \textbf{.41} & \textbf{.54} & \textbf{.72} & \textbf{.8} & .8 & \textbf{.89} & \textbf{.95} & \textbf{.95} & \textbf{.96} & \textbf{1.8} \\
 & C & .35 & .35 & .42 & .54 & .64 & .62 & .67 & .71 & .74 & .77 & 2.7\\
 & D & .26 & .29 & .38 & .52 & .52 & .62 & .72 & .71 & .72 & .75 & 2.9\\
 & E & \textbf{.44} & .39 & .52 & .71 & .76 & \textbf{.81} & .88 & .92 & .93 & .95 & 1.9\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & \textbf{.28} & \textbf{.3} & .16 & .14 & .27 & .3 & .34 & .25 & .29 & .3 & 1.2\\
 & B & .1 & .18 & .24 & \textbf{.5} & \textbf{.63} & \textbf{.68} & .64 & \textbf{.69} & .69 & \textbf{1.0} & 2.3\\
 & C & .15 & .22 & .32 & .45 & .58 & .6 & .61 & .68 & .73 & .8 & 2.7\\
 & D & .16 & .25 & \textbf{.36} & \textbf{.5} & .57 & .63 & \textbf{.68} & .64 & \textbf{.83} & .87 & 1.9\\
 & E & .05 & .25 & .3 & .46 & .57 & .5 & .46 & .43 & .57 & .79 & \textbf{1.1} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & .32 & .36 & .57 & .68 & .82 & .95 & .96 & .98 & \textbf{1.0} & \textbf{1.0} & 1.2\\
 & B & .34 & .46 & .64 & .74 & .86 & .93 & .95 & .96 & \textbf{1.0} & \textbf{1.0} & 1.9\\
 & C & .28 & .29 & .38 & .48 & .59 & .73 & .83 & .89 & .93 & .96 & 1.8\\
 & D & .22 & .3 & .42 & .52 & .6 & .65 & .85 & .92 & .95 & \textbf{1.0} & 2.4\\
 & E & \textbf{.45} & \textbf{.68} & \textbf{.8} & \textbf{.86} & \textbf{.95} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.1} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{average}}
 & A & .3 & .38 & .44 & .53 & .61 & .68 & .71 & .75 & .78 & .81 & 2.1\\
 & B & .3 & .41 & .49 & \textbf{.6} & \textbf{.67} & \textbf{.72} & \textbf{.78} & \textbf{.84} & \textbf{.9} & \textbf{.97} & 1.7\\
 & C & .27 & .37 & .45 & .54 & .61 & .66 & .71 & .75 & .81 & .86 & 2.4\\
 & D & .18 & .28 & .38 & .47 & .54 & .6 & .68 & .71 & .8 & .86 & 2.7\\
 & E & \textbf{.31} & \textbf{.42} & \textbf{.51} & .58 & .66 & .71 & .76 & .8 & .86 & .9 & \textbf{1.6} \\
\hline
\end{tabular}
}
\end{table}

==> tables/evaluationTable_VSAPN.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MS, PLR, RG09, LPBased, VSAPN) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{5}{*}{\rotatebox[origin=c]{90}{average}}
 & A & .33 & .41 & .47 & .55 & .62 & .67 & .72 & .76 & .78 & .8 & 2.0\\
 & B & .31 & .41 & .51 & .6 & .68 & .73 & .81 & .86 & .92 & \textbf{.98} & 1.4\\
 & C & .3 & .41 & .48 & .58 & .64 & .68 & .74 & .77 & .82 & .87 & 2.3\\
 & D & .21 & .32 & .41 & .5 & .57 & .63 & .71 & .73 & .82 & .87 & 2.6\\
 & E & \textbf{.38} & \textbf{.48} & \textbf{.57} & \textbf{.64} & \textbf{.72} & \textbf{.76} & \textbf{.84} & \textbf{.88} & \textbf{.93} & .96 & \textbf{1.1} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{blocks-world}}
 & A & .1 & .13 & .14 & .24 & .29 & .36 & .41 & .47 & .54 & .55 & 7.1\\
 & B & .09 & .23 & \textbf{.28} & .32 & \textbf{.43} & \textbf{.56} & \textbf{.62} & \textbf{.71} & \textbf{.85} & \textbf{.92} & \textbf{1.5} \\
 & C & .08 & .22 & .23 & .29 & .38 & .42 & .53 & .63 & .81 & .9 & 4.1\\
 & D & .06 & .13 & .15 & .2 & .33 & .38 & .46 & .52 & .76 & .81 & 5.4\\
 & E & \textbf{.12} & \textbf{.29} & .23 & \textbf{.33} & .42 & .46 & .57 & .63 & .78 & .88 & 1.8\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{campus}}
 & A & .73 & .73 & .73 & .53 & .57 & .43 & .57 & .63 & .6 & .6 & 1.4\\
 & B & .73 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & C & .73 & .8 & .8 & .83 & .83 & .83 & .83 & .8 & .8 & .8 & 1.2\\
 & D & .5 & .87 & .87 & .97 & .97 & .97 & .97 & .97 & .97 & .97 & 1.2\\
 & E & \textbf{.8} & .93 & .93 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{depots}}
 & A & \textbf{.21} & .16 & .16 & .22 & .38 & .49 & .48 & .54 & .59 & .59 & 1.8\\
 & B & .13 & .17 & .24 & .27 & .33 & .42 & .75 & .83 & .91 & .93 & 1.9\\
 & C & .16 & \textbf{.29} & .28 & \textbf{.32} & .45 & .62 & .59 & .6 & .61 & .78 & 2.6\\
 & D & .09 & .16 & .17 & .27 & .34 & .44 & .57 & .69 & .75 & .89 & 2.4\\
 & E & \textbf{.21} & .14 & \textbf{.32} & .29 & \textbf{.54} & \textbf{.68} & \textbf{.86} & \textbf{.89} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & A & .29 & \textbf{.37} & \textbf{.5} & \textbf{.63} & \textbf{.73} & \textbf{.84} & \textbf{.92} & \textbf{.91} & \textbf{.91} & \textbf{.96} & 1.4\\
 & B & .19 & .29 & .42 & .54 & .64 & .71 & .75 & .84 & .88 & .92 & 1.3\\
 & C & .22 & .27 & .35 & .46 & .52 & .6 & .75 & .77 & .81 & .81 & 2.9\\
 & D & .2 & .26 & .37 & .5 & .58 & .68 & .67 & .68 & .76 & .8 & 2.3\\
 & E & \textbf{.32} & .36 & \textbf{.5} & .57 & .57 & .57 & .79 & .89 & .89 & .93 & \textbf{1.0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{dwr}}
 & A & .13 & .23 & .2 & .34 & .34 & .39 & .43 & .47 & .46 & .55 & 2.0\\
 & B & \textbf{.36} & .38 & \textbf{.46} & \textbf{.54} & \textbf{.52} & \textbf{.5} & .66 & \textbf{.77} & \textbf{.91} & \textbf{1.0} & 1.2\\
 & C & .25 & .33 & .32 & .26 & .2 & .22 & .3 & .27 & .31 & .41 & 2.7\\
 & D & .19 & .18 & .24 & .29 & .28 & .33 & .51 & .51 & .65 & .81 & 2.0\\
 & E & \textbf{.36} & \textbf{.39} & \textbf{.46} & .39 & .43 & \textbf{.5} & \textbf{.68} & .68 & .86 & .89 & \textbf{1.0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & .29 & .32 & .44 & \textbf{.52} & .56 & .63 & .71 & .76 & .83 & .94 & 2.4\\
 & B & .09 & .09 & .14 & .15 & .26 & .32 & .42 & .51 & .68 & \textbf{1.0} & 1.6\\
 & C & \textbf{.32} & .34 & \textbf{.45} & .48 & .57 & .63 & .69 & .78 & .85 & \textbf{1.0} & 3.0\\
 & D & .13 & .24 & .28 & .35 & .39 & .47 & .5 & .57 & .7 & .78 & 3.3\\
 & E & .3 & \textbf{.35} & .41 & \textbf{.52} & \textbf{.58} & \textbf{.65} & \textbf{.72} & \textbf{.81} & \textbf{.88} & .93 & \textbf{1.0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{ferry}}
 & A & .38 & \textbf{.7} & \textbf{.8} & .83 & .89 & .95 & .93 & .96 & .96 & .96 & \textbf{1.2} \\
 & B & .37 & .56 & .7 & .82 & .88 & .95 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & C & .28 & .58 & .73 & .8 & .89 & .91 & .95 & .96 & .96 & .96 & 1.6\\
 & D & .19 & .34 & .54 & .75 & .85 & .88 & .91 & .91 & .93 & .96 & 2.1\\
 & E & \textbf{.42} & .67 & .75 & \textbf{.87} & \textbf{.98} & \textbf{.98} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{intrusion-detection}}
 & A & \textbf{.26} & \textbf{.45} & .59 & \textbf{.8} & \textbf{.83} & \textbf{.83} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.8\\
 & B & .22 & .4 & \textbf{.65} & .77 & .81 & .81 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.1} \\
 & C & \textbf{.26} & \textbf{.45} & .59 & \textbf{.8} & \textbf{.83} & \textbf{.83} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.8\\
 & D & .18 & .24 & .35 & .38 & .66 & .67 & .72 & .78 & .94 & .96 & 2.9\\
 & E & .22 & .4 & \textbf{.65} & .77 & .81 & .81 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.1} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{logistics}}
 & A & .35 & .41 & .47 & .6 & .7 & .73 & .76 & \textbf{.89} & \textbf{.97} & \textbf{1.0} & 1.5\\
 & B & .26 & .31 & .41 & .63 & .69 & .73 & .81 & \textbf{.89} & \textbf{.97} & \textbf{1.0} & 1.3\\
 & C & .34 & .47 & .58 & .69 & .72 & .77 & .8 & .82 & .93 & \textbf{1.0} & 1.9\\
 & D & .16 & .35 & .41 & .48 & .5 & .53 & .68 & .68 & .69 & .74 & 3.7\\
 & E & \textbf{.41} & \textbf{.51} & \textbf{.59} & \textbf{.71} & \textbf{.8} & \textbf{.82} & \textbf{.82} & \textbf{.89} & \textbf{.97} & \textbf{1.0} & \textbf{1.2} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & .41 & .65 & .73 & \textbf{.84} & .88 & .86 & .89 & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.3\\
 & B & \textbf{.61} & \textbf{.77} & \textbf{.8} & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & C & .32 & .49 & .59 & .74 & .82 & .87 & .9 & .95 & \textbf{1.0} & \textbf{1.0} & 1.7\\
 & D & .24 & .43 & .58 & .57 & .76 & .8 & .82 & .86 & .95 & .93 & 2.0\\
 & E & \textbf{.61} & \textbf{.77} & \textbf{.8} & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & \textbf{.46} & .6 & .69 & .89 & .89 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.2\\
 & B & \textbf{.46} & \textbf{.64} & .8 & .88 & .88 & .91 & .95 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.2\\
 & C & .43 & .6 & .74 & \textbf{.91} & \textbf{.92} & .93 & .93 & .96 & .98 & .98 & 1.5\\
 & D & .31 & .48 & .64 & .67 & .7 & .74 & .81 & .84 & .91 & .93 & 2.0\\
 & E & \textbf{.46} & \textbf{.64} & \textbf{.82} & .86 & .89 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{satellite}}
 & A & .35 & .31 & .36 & .43 & .59 & .66 & .74 & .81 & .81 & .81 & 2.4\\
 & B & .4 & .4 & .54 & \textbf{.72} & \textbf{.8} & \textbf{.8} & \textbf{.89} & \textbf{.95} & \textbf{.95} & .96 & 1.6\\
 & C & .35 & .35 & .42 & .54 & .64 & .62 & .67 & .71 & .74 & .77 & 2.7\\
 & D & .26 & .29 & .38 & .52 & .52 & .62 & .72 & .71 & .72 & .75 & 2.9\\
 & E & \textbf{.5} & \textbf{.46} & \textbf{.58} & .65 & .73 & \textbf{.8} & \textbf{.89} & \textbf{.95} & \textbf{.95} & \textbf{.98} & \textbf{1.1} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & \textbf{.28} & .3 & .16 & .14 & .27 & .3 & .34 & .25 & .29 & .3 & 1.2\\
 & B & .19 & .21 & .24 & .37 & .57 & .61 & .63 & .65 & .69 & \textbf{1.0} & 2.4\\
 & C & .15 & .22 & .32 & .45 & .58 & .6 & .61 & \textbf{.68} & .73 & .8 & 2.7\\
 & D & .16 & .25 & .36 & \textbf{.5} & .57 & \textbf{.63} & \textbf{.68} & .64 & \textbf{.83} & .87 & 1.9\\
 & E & .18 & \textbf{.39} & \textbf{.39} & \textbf{.5} & \textbf{.64} & .54 & .61 & .61 & .71 & .79 & \textbf{1.0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & .32 & .36 & \textbf{.57} & \textbf{.68} & .82 & \textbf{.95} & \textbf{.96} & .98 & \textbf{1.0} & \textbf{1.0} & 1.2\\
 & B & .2 & .34 & .46 & .62 & \textbf{.83} & .93 & .95 & .96 & \textbf{1.0} & \textbf{1.0} & 1.6\\
 & C & .28 & .29 & .38 & .48 & .59 & .73 & .83 & .89 & .93 & .96 & 1.8\\
 & D & .22 & .3 & .42 & .52 & .6 & .65 & .85 & .92 & .95 & \textbf{1.0} & 2.4\\
 & E & \textbf{.39} & \textbf{.46} & \textbf{.57} & .64 & .82 & .93 & .93 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\end{tabular}
}
\end{table}

==> tables/evaluationTable_VSAPN_060324.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MS, RG09, LPBased, PLR-rhw, VSAPN) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{5}{*}{\rotatebox[origin=c]{90}{average}}
 & A & .33 & .41 & .47 & .55 & .62 & .67 & .72 & .76 & .78 & .8 & 2.0\\
 & B & .3 & .41 & .48 & .58 & .64 & .68 & .74 & .77 & .82 & .87 & 2.3\\
 & C & .21 & .32 & .41 & .5 & .57 & .63 & .71 & .73 & .82 & .87 & 2.6\\
 & D & .3 & .35 & .44 & .53 & .61 & .69 & .73 & .78 & .85 & .92 & 1.2\\
 & E & \textbf{.38} & \textbf{.48} & \textbf{.57} & \textbf{.64} & \textbf{.72} & \textbf{.76} & \textbf{.84} & \textbf{.88} & \textbf{.93} & \textbf{.96} & \textbf{1.1} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{blocks-world}}
 & A & .1 & .13 & .14 & .24 & .29 & .36 & .41 & .47 & .54 & .55 & 7.1\\
 & B & .08 & .22 & \textbf{.23} & .29 & .38 & .42 & .53 & \textbf{.63} & \textbf{.81} & \textbf{.9} & 4.1\\
 & C & .06 & .13 & .15 & .2 & .33 & .38 & .46 & .52 & .76 & .81 & 5.4\\
 & D & .09 & .09 & .1 & .1 & .09 & .09 & .09 & .07 & .21 & .27 & 2.8\\
 & E & \textbf{.12} & \textbf{.29} & \textbf{.23} & \textbf{.33} & \textbf{.42} & \textbf{.46} & \textbf{.57} & \textbf{.63} & .78 & .88 & \textbf{1.8} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{campus}}
 & A & .73 & .73 & .73 & .53 & .57 & .43 & .57 & .63 & .6 & .6 & 1.4\\
 & B & .73 & .8 & .8 & .83 & .83 & .83 & .83 & .8 & .8 & .8 & 1.2\\
 & C & .5 & .87 & .87 & .97 & .97 & .97 & .97 & .97 & .97 & .97 & 1.2\\
 & D & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & E & .8 & .93 & .93 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{depots}}
 & A & \textbf{.21} & .16 & .16 & .22 & .38 & .49 & .48 & .54 & .59 & .59 & 1.8\\
 & B & .16 & \textbf{.29} & .28 & \textbf{.32} & .45 & .62 & .59 & .6 & .61 & .78 & 2.6\\
 & C & .09 & .16 & .17 & .27 & .34 & .44 & .57 & .69 & .75 & .89 & 2.4\\
 & D & .18 & .14 & .2 & .2 & .23 & .3 & .5 & .64 & .61 & .82 & 1.2\\
 & E & \textbf{.21} & .14 & \textbf{.32} & .29 & \textbf{.54} & \textbf{.68} & \textbf{.86} & \textbf{.89} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & A & .29 & \textbf{.37} & \textbf{.5} & \textbf{.63} & \textbf{.73} & \textbf{.84} & \textbf{.92} & \textbf{.91} & \textbf{.91} & \textbf{.96} & 1.4\\
 & B & .22 & .27 & .35 & .46 & .52 & .6 & .75 & .77 & .81 & .81 & 2.9\\
 & C & .2 & .26 & .37 & .5 & .58 & .68 & .67 & .68 & .76 & .8 & 2.3\\
 & D & .25 & .23 & .39 & .52 & .61 & .75 & .8 & .8 & .82 & .92 & 1.1\\
 & E & \textbf{.32} & .36 & \textbf{.5} & .57 & .57 & .57 & .79 & .89 & .89 & .93 & \textbf{1.0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{dwr}}
 & A & .13 & .23 & .2 & .34 & .34 & .39 & .43 & .47 & .46 & .55 & 2.0\\
 & B & .25 & .33 & .32 & .26 & .2 & .22 & .3 & .27 & .31 & .41 & 2.7\\
 & C & .19 & .18 & .24 & .29 & .28 & .33 & .51 & .51 & .65 & .81 & 2.0\\
 & D & .23 & .16 & .27 & \textbf{.45} & \textbf{.5} & \textbf{.54} & .52 & .63 & .79 & \textbf{1.0} & 1.1\\
 & E & \textbf{.36} & \textbf{.39} & \textbf{.46} & .39 & .43 & .5 & \textbf{.68} & \textbf{.68} & \textbf{.86} & .89 & \textbf{1.0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & .29 & .32 & .44 & \textbf{.52} & .56 & .63 & .71 & .76 & .83 & .94 & 2.4\\
 & B & \textbf{.32} & .34 & \textbf{.45} & .48 & .57 & .63 & .69 & .78 & .85 & \textbf{1.0} & 3.0\\
 & C & .13 & .24 & .28 & .35 & .39 & .47 & .5 & .57 & .7 & .78 & 3.3\\
 & D & .2 & .22 & .36 & .42 & .42 & .5 & .58 & .59 & .72 & \textbf{1.0} & \textbf{1.0} \\
 & E & .3 & \textbf{.35} & .41 & \textbf{.52} & \textbf{.58} & \textbf{.65} & \textbf{.72} & \textbf{.81} & \textbf{.88} & .93 & \textbf{1.0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{ferry}}
 & A & .38 & \textbf{.7} & \textbf{.8} & .83 & .89 & .95 & .93 & .96 & .96 & .96 & 1.2\\
 & B & .28 & .58 & .73 & .8 & .89 & .91 & .95 & .96 & .96 & .96 & 1.6\\
 & C & .19 & .34 & .54 & .75 & .85 & .88 & .91 & .91 & .93 & .96 & 2.1\\
 & D & .25 & .38 & .64 & .73 & .84 & .89 & .96 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.1} \\
 & E & \textbf{.42} & .67 & .75 & \textbf{.87} & \textbf{.98} & \textbf{.98} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.2\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{intrusion-detection}}
 & A & \textbf{.26} & \textbf{.45} & .59 & \textbf{.8} & \textbf{.83} & \textbf{.83} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.8\\
 & B & \textbf{.26} & \textbf{.45} & .59 & \textbf{.8} & \textbf{.83} & \textbf{.83} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.8\\
 & C & .18 & .24 & .35 & .38 & .66 & .67 & .72 & .78 & .94 & .96 & 2.9\\
 & D & .16 & .33 & .34 & .62 & .64 & .77 & .81 & .92 & \textbf{1.0} & \textbf{1.0} & \textbf{1.1} \\
 & E & .22 & .4 & \textbf{.65} & .77 & .81 & .81 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.1} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{logistics}}
 & A & .35 & .41 & .47 & .6 & .7 & .73 & .76 & \textbf{.89} & \textbf{.97} & \textbf{1.0} & 1.5\\
 & B & .34 & .47 & .58 & .69 & .72 & .77 & .8 & .82 & .93 & \textbf{1.0} & 1.9\\
 & C & .16 & .35 & .41 & .48 & .5 & .53 & .68 & .68 & .69 & .74 & 3.7\\
 & D & .23 & .39 & .42 & .51 & .58 & .76 & \textbf{.83} & \textbf{.89} & \textbf{.97} & \textbf{1.0} & \textbf{1.2} \\
 & E & \textbf{.41} & \textbf{.51} & \textbf{.59} & \textbf{.71} & \textbf{.8} & \textbf{.82} & .82 & \textbf{.89} & \textbf{.97} & \textbf{1.0} & \textbf{1.2} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & .41 & .65 & .73 & \textbf{.84} & .88 & .86 & .89 & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.3\\
 & B & .32 & .49 & .59 & .74 & .82 & .87 & .9 & .95 & \textbf{1.0} & \textbf{1.0} & 1.7\\
 & C & .24 & .43 & .58 & .57 & .76 & .8 & .82 & .86 & .95 & .93 & 2.0\\
 & D & .34 & .54 & .64 & .71 & .77 & .86 & .89 & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & E & \textbf{.61} & \textbf{.77} & \textbf{.8} & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.2\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & .46 & .6 & .69 & .89 & .89 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.2\\
 & B & .43 & .6 & .74 & \textbf{.91} & \textbf{.92} & .93 & .93 & .96 & .98 & .98 & 1.5\\
 & C & .31 & .48 & .64 & .67 & .7 & .74 & .81 & .84 & .91 & .93 & 2.0\\
 & D & \textbf{.48} & .52 & .8 & .82 & .86 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.1\\
 & E & .46 & \textbf{.64} & \textbf{.82} & .86 & .89 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{satellite}}
 & A & .35 & .31 & .36 & .43 & .59 & .66 & .74 & .81 & .81 & .81 & 2.4\\
 & B & .35 & .35 & .42 & .54 & .64 & .62 & .67 & .71 & .74 & .77 & 2.7\\
 & C & .26 & .29 & .38 & .52 & .52 & .62 & .72 & .71 & .72 & .75 & 2.9\\
 & D & .34 & .24 & .29 & .6 & \textbf{.77} & \textbf{.8} & .82 & .91 & \textbf{.95} & .96 & 1.4\\
 & E & \textbf{.5} & \textbf{.46} & \textbf{.58} & \textbf{.65} & .73 & \textbf{.8} & \textbf{.89} & \textbf{.95} & \textbf{.95} & \textbf{.98} & \textbf{1.1} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & \textbf{.28} & .3 & .16 & .14 & .27 & .3 & .34 & .25 & .29 & .3 & 1.2\\
 & B & .15 & .22 & .32 & .45 & .58 & .6 & .61 & \textbf{.68} & .73 & .8 & 2.7\\
 & C & .16 & .25 & .36 & \textbf{.5} & .57 & \textbf{.63} & \textbf{.68} & .64 & .83 & .87 & 1.9\\
 & D & .13 & .21 & .25 & .32 & .5 & .57 & .57 & .5 & \textbf{.86} & \textbf{.96} & \textbf{1.0} \\
 & E & .18 & \textbf{.39} & \textbf{.39} & \textbf{.5} & \textbf{.64} & .54 & .61 & .61 & .71 & .79 & \textbf{1.0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & .32 & .36 & \textbf{.57} & \textbf{.68} & \textbf{.82} & \textbf{.95} & \textbf{.96} & .98 & \textbf{1.0} & \textbf{1.0} & 1.2\\
 & B & .28 & .29 & .38 & .48 & .59 & .73 & .83 & .89 & .93 & .96 & 1.8\\
 & C & .22 & .3 & .42 & .52 & .6 & .65 & .85 & .92 & .95 & \textbf{1.0} & 2.4\\
 & D & .3 & .41 & .45 & .48 & .73 & .82 & .89 & .96 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & E & \textbf{.39} & \textbf{.46} & \textbf{.57} & .64 & \textbf{.82} & .93 & .93 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\end{tabular}
}
\end{table}

==> tables/evaluationTable_VS_repeated.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (VS-10-1, VS-10-2, VS-10-3, VS-10-4, VS-10-5, VS-10-6, VS-10-7, VS-10-8, VS-10-9, VS-10-10) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{10}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & .05 & .25 & .3 & .46 & .57 & .5 & .46 & .43 & .57 & .79 & \textbf{1.1} \\
 & B & .06 & .25 & .39 & .46 & .61 & .46 & .57 & .5 & .54 & .82 & 1.2\\
 & C & .09 & .27 & .33 & .38 & .48 & .51 & .46 & .43 & .61 & .71 & 1.2\\
 & D & .08 & .33 & \textbf{.46} & .5 & .54 & .5 & \textbf{.61} & \textbf{.59} & \textbf{.68} & .82 & 1.2\\
 & E & \textbf{.13} & \textbf{.36} & \textbf{.46} & \textbf{.61} & .61 & .54 & \textbf{.61} & .5 & .64 & \textbf{.89} & 1.2\\
 & F & .1 & .32 & .34 & .54 & .5 & .46 & .54 & .46 & .61 & .82 & 1.2\\
 & G & .1 & .34 & .38 & .55 & \textbf{.64} & \textbf{.64} & .57 & .5 & .61 & .86 & 1.2\\
 & H & .11 & .32 & .29 & .46 & .57 & .61 & .57 & .54 & .64 & .82 & \textbf{1.1} \\
 & I & .08 & .29 & .43 & .5 & .5 & .46 & .5 & .46 & .57 & .79 & 1.2\\
 & J & .08 & .21 & .32 & .46 & .54 & .46 & .54 & .43 & .61 & .75 & 1.2\\
\hline
\multirow{10}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & \textbf{.45} & \textbf{.68} & .8 & .86 & .95 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.1\\
 & B & .39 & .57 & .75 & .82 & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & C & .32 & .5 & .54 & .68 & .86 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & D & .34 & .55 & .63 & .8 & .93 & .93 & .93 & .93 & \textbf{1.0} & \textbf{1.0} & 1.1\\
 & E & .42 & .43 & .64 & \textbf{.89} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & F & .3 & .48 & .64 & .86 & .93 & .96 & .96 & .96 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & G & .28 & .49 & .64 & .82 & .89 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.1\\
 & H & .4 & .61 & \textbf{.82} & .75 & .93 & .96 & .96 & .96 & \textbf{1.0} & \textbf{1.0} & 1.1\\
 & I & .34 & .48 & .57 & .8 & .89 & .96 & .93 & .96 & \textbf{1.0} & \textbf{1.0} & 1.1\\
 & J & .35 & .66 & .79 & .79 & \textbf{.96} & .96 & .96 & .96 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\end{tabular}
}
\end{table}

==> tables/evaluationTable_new.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MastersSardina, Landmarks-EX-wInitial, RG09, LPBased, VS-10-1) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Precision (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{5}{*}{\rotatebox[origin=c]{90}{average}}
 & A & \textbf{.35} & .43 & .49 & .57 & .63 & .67 & .73 & .77 & .79 & .81 & 1.9\\
 & B & .33 & .44 & .54 & .61 & .68 & .73 & \textbf{.8} & \textbf{.85} & \textbf{.9} & \textbf{.96} & \textbf{1.5} \\
 & C & .32 & .43 & .5 & .59 & .65 & .69 & .75 & .78 & .82 & .86 & 2.2\\
 & D & .19 & .3 & .38 & .46 & .54 & .59 & .66 & .69 & .77 & .81 & 2.4\\
 & E & \textbf{.35} & \textbf{.46} & \textbf{.55} & \textbf{.64} & \textbf{.7} & \textbf{.74} & \textbf{.8} & .83 & .87 & .91 & 1.6\\
\hline
\end{tabular}
}
\end{table}

==> tables/evaluationTable_old.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MastersSardina, Landmarks-woInitial, RG09, LPBased, Greedy, HAdd, HMax) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{7}{*}{\rotatebox[origin=c]{90}{blocks-world}}
 & A & \textbf{.1} & .13 & .14 & .24 & .29 & .36 & .41 & .47 & .54 & .55 & 7.1\\
 & B & .09 & .18 & .22 & .28 & \textbf{.44} & \textbf{.5} & \textbf{.61} & \textbf{.67} & \textbf{.88} & \textbf{.95} & \textbf{1.5} \\
 & C & .08 & \textbf{.22} & \textbf{.23} & \textbf{.29} & .38 & .42 & .53 & .63 & .81 & .9 & 4.1\\
 & D & .06 & .13 & .15 & .2 & .33 & .38 & .46 & .52 & .76 & .81 & 5.4\\
 & E & .08 & \textbf{.22} & \textbf{.23} & \textbf{.29} & .38 & .42 & .53 & .61 & .83 & .93 & 4.0\\
 & F & .08 & \textbf{.22} & \textbf{.23} & \textbf{.29} & .38 & .42 & .53 & .61 & .83 & .93 & 4.0\\
 & G & .08 & \textbf{.22} & \textbf{.23} & \textbf{.29} & .38 & .42 & .53 & .61 & .83 & .93 & 4.0\\
\hline
\multirow{7}{*}{\rotatebox[origin=c]{90}{depots}}
 & A & \textbf{.21} & .16 & .16 & .22 & .38 & .49 & .48 & .54 & .59 & .59 & 1.8\\
 & B & .11 & .16 & .15 & .19 & .32 & .6 & \textbf{.78} & \textbf{.89} & \textbf{.95} & \textbf{.96} & \textbf{1.5} \\
 & C & .16 & \textbf{.29} & \textbf{.28} & \textbf{.32} & .45 & .62 & .59 & .6 & .61 & .78 & 2.6\\
 & D & .09 & .16 & .17 & .27 & .34 & .44 & .57 & .69 & .75 & .89 & 2.4\\
 & E & .11 & .13 & .21 & .21 & .38 & .41 & .55 & .67 & .81 & .88 & 2.4\\
 & F & .16 & .22 & .24 & .27 & \textbf{.46} & \textbf{.68} & .77 & .88 & .9 & .93 & 2.9\\
 & G & .15 & .17 & .25 & .3 & .45 & .57 & .7 & .75 & .86 & .89 & 2.7\\
\hline
\multirow{7}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & A & \textbf{.29} & \textbf{.37} & \textbf{.5} & \textbf{.63} & \textbf{.73} & \textbf{.84} & \textbf{.92} & \textbf{.91} & \textbf{.91} & \textbf{.96} & \textbf{1.4} \\
 & B & .17 & .24 & .38 & .46 & .59 & .69 & .75 & .81 & \textbf{.91} & .93 & 1.8\\
 & C & .22 & .27 & .35 & .46 & .52 & .6 & .75 & .77 & .81 & .81 & 2.9\\
 & D & .2 & .26 & .37 & .5 & .58 & .68 & .67 & .68 & .76 & .8 & 2.3\\
 & E & .19 & .24 & .37 & .41 & .44 & .56 & .68 & .71 & .8 & .83 & 2.7\\
 & F & .21 & .23 & .26 & .38 & .44 & .49 & .62 & .66 & .8 & .85 & 2.6\\
 & G & .22 & .23 & .26 & .4 & .49 & .56 & .69 & .74 & .82 & .86 & 2.4\\
\hline
\multirow{7}{*}{\rotatebox[origin=c]{90}{dwr}}
 & A & .13 & .23 & .2 & .34 & .34 & .39 & .43 & .47 & .46 & .55 & 2.0\\
 & B & \textbf{.32} & \textbf{.46} & \textbf{.49} & \textbf{.5} & \textbf{.54} & \textbf{.54} & \textbf{.6} & \textbf{.72} & \textbf{.88} & \textbf{1.0} & \textbf{1.1} \\
 & C & .25 & .33 & .32 & .26 & .2 & .22 & .3 & .27 & .31 & .41 & 2.7\\
 & D & .19 & .18 & .24 & .29 & .28 & .33 & .51 & .51 & .65 & .81 & 2.0\\
 & E & .2 & .24 & .34 & .25 & .29 & .38 & .47 & .5 & .55 & .79 & 2.4\\
 & F & .24 & .32 & .36 & .37 & .37 & .44 & .52 & .59 & .74 & .82 & 2.1\\
 & G & .22 & .29 & .3 & .28 & .28 & .36 & .43 & .52 & .73 & .91 & 2.4\\
\hline
\multirow{7}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & .29 & .32 & .44 & \textbf{.52} & .56 & \textbf{.63} & \textbf{.71} & .76 & .83 & .94 & 2.4\\
 & B & .2 & .19 & .23 & .27 & .29 & .34 & .42 & .48 & .62 & \textbf{1.0} & \textbf{1.3} \\
 & C & \textbf{.32} & .34 & \textbf{.45} & .48 & \textbf{.57} & \textbf{.63} & .69 & \textbf{.78} & \textbf{.85} & \textbf{1.0} & 3.0\\
 & D & .13 & .24 & .28 & .35 & .39 & .47 & .5 & .57 & .7 & .78 & 3.3\\
 & E & .31 & \textbf{.36} & .43 & .45 & .55 & .58 & .63 & .67 & .77 & .91 & 2.9\\
 & F & .3 & .35 & .43 & .48 & .55 & .58 & .64 & .7 & .8 & .91 & 2.7\\
 & G & \textbf{.32} & .35 & .43 & .46 & .55 & .58 & .63 & .69 & .77 & .91 & 2.7\\
\hline
\multirow{7}{*}{\rotatebox[origin=c]{90}{ferry}}
 & A & .38 & \textbf{.7} & \textbf{.8} & .83 & .89 & \textbf{.95} & .93 & \textbf{.96} & \textbf{.96} & \textbf{.96} & \textbf{1.2} \\
 & B & \textbf{.4} & .6 & .72 & .81 & .89 & .93 & \textbf{.96} & \textbf{.96} & \textbf{.96} & \textbf{.96} & \textbf{1.2} \\
 & C & .28 & .58 & .73 & .8 & .89 & .91 & .95 & \textbf{.96} & \textbf{.96} & \textbf{.96} & 1.6\\
 & D & .19 & .34 & .54 & .75 & .85 & .88 & .91 & .91 & .93 & \textbf{.96} & 2.1\\
 & E & .28 & .58 & .74 & \textbf{.85} & \textbf{.93} & .93 & .95 & \textbf{.96} & \textbf{.96} & \textbf{.96} & 1.6\\
 & F & .28 & .58 & .74 & \textbf{.85} & \textbf{.93} & .93 & .95 & \textbf{.96} & \textbf{.96} & \textbf{.96} & 1.6\\
 & G & .28 & .58 & .74 & \textbf{.85} & \textbf{.93} & .93 & .95 & \textbf{.96} & \textbf{.96} & \textbf{.96} & 1.6\\
\hline
\end{tabular}
}
\end{table}

==> tables/evaluationTable_old_2.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MastersSardina, Landmarks-woInitial, RG09, LPBased, Greedy, HAdd, HMax) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{7}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & .41 & .65 & .73 & \textbf{.84} & .88 & .86 & .89 & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.3\\
 & B & \textbf{.61} & \textbf{.77} & \textbf{.8} & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & C & .32 & .49 & .59 & .74 & .82 & .87 & .9 & .95 & \textbf{1.0} & \textbf{1.0} & 1.7\\
 & D & .24 & .43 & .58 & .57 & .76 & .8 & .82 & .86 & .95 & .93 & 2.0\\
 & E & .51 & .72 & .76 & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.4\\
 & F & .51 & .72 & .76 & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.4\\
 & G & .51 & .72 & .76 & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.4\\
\hline
\multirow{7}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & \textbf{.46} & .6 & .69 & .89 & .89 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & B & .43 & .59 & \textbf{.8} & .88 & .88 & .9 & .93 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & C & .43 & .6 & .74 & \textbf{.91} & \textbf{.92} & .93 & .93 & .96 & .98 & .98 & 1.5\\
 & D & .31 & .48 & .64 & .67 & .7 & .74 & .81 & .84 & .91 & .93 & 2.0\\
 & E & .39 & .6 & .7 & .85 & .88 & .93 & .93 & .98 & \textbf{1.0} & \textbf{1.0} & 1.5\\
 & F & .45 & \textbf{.63} & .73 & .83 & .85 & .91 & .95 & .98 & .98 & \textbf{1.0} & 1.4\\
 & G & .39 & .53 & .65 & .82 & .84 & .91 & .88 & .93 & .93 & .93 & 1.5\\
\hline
\multirow{7}{*}{\rotatebox[origin=c]{90}{satellite}}
 & A & .35 & .31 & .36 & .43 & .59 & .66 & .74 & .81 & .81 & .81 & 2.4\\
 & B & .36 & .36 & .49 & .67 & .76 & \textbf{.8} & \textbf{.86} & \textbf{.92} & \textbf{.92} & \textbf{.92} & 1.8\\
 & C & .35 & .35 & .42 & .54 & .64 & .62 & .67 & .71 & .74 & .77 & 2.7\\
 & D & .26 & .29 & .38 & .52 & .52 & .62 & .72 & .71 & .72 & .75 & 2.9\\
 & E & \textbf{.42} & \textbf{.43} & \textbf{.56} & \textbf{.7} & \textbf{.78} & .76 & \textbf{.86} & .89 & \textbf{.92} & \textbf{.92} & 2.0\\
 & F & .33 & .29 & .34 & .39 & .45 & .54 & .58 & .65 & .66 & .71 & \textbf{1.7} \\
 & G & .33 & .3 & .3 & .39 & .47 & .52 & .62 & .74 & .79 & .79 & \textbf{1.7} \\
\hline
\multirow{7}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & \textbf{.28} & \textbf{.3} & .16 & .14 & .27 & .3 & .34 & .25 & .29 & .3 & \textbf{1.2} \\
 & B & .17 & .2 & .22 & .38 & .53 & .55 & .61 & .6 & .66 & \textbf{1.0} & 1.5\\
 & C & .15 & .22 & .32 & .45 & \textbf{.58} & .6 & .61 & \textbf{.68} & .73 & .8 & 2.7\\
 & D & .16 & .25 & \textbf{.36} & \textbf{.5} & .57 & \textbf{.63} & \textbf{.68} & .64 & \textbf{.83} & .87 & 1.9\\
 & E & .09 & .16 & .35 & .39 & .51 & .53 & .5 & .54 & .52 & .63 & 2.0\\
 & F & .1 & .14 & .28 & .32 & .38 & .42 & .43 & .5 & .55 & .6 & 1.6\\
 & G & .14 & .12 & .31 & .28 & .34 & .42 & .46 & .47 & .55 & .62 & 1.8\\
\hline
\multirow{7}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & \textbf{.32} & .36 & \textbf{.57} & \textbf{.68} & \textbf{.82} & \textbf{.95} & \textbf{.96} & \textbf{.98} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & B & .31 & \textbf{.41} & .56 & .64 & \textbf{.82} & .9 & .93 & .96 & \textbf{1.0} & \textbf{1.0} & 1.6\\
 & C & .28 & .29 & .38 & .48 & .59 & .73 & .83 & .89 & .93 & .96 & 1.8\\
 & D & .22 & .3 & .42 & .52 & .6 & .65 & .85 & .92 & .95 & \textbf{1.0} & 2.4\\
 & E & .28 & .37 & .43 & .52 & .67 & .75 & .82 & .8 & .86 & .92 & 1.6\\
 & F & .28 & .26 & .38 & .47 & .54 & .69 & .71 & .68 & .73 & .79 & 1.5\\
 & G & .26 & .3 & .37 & .38 & .51 & .6 & .63 & .63 & .68 & .79 & 1.5\\
\hline
\multirow{7}{*}{\rotatebox[origin=c]{90}{average}}
 & A & \textbf{.3} & \textbf{.38} & .44 & .53 & .61 & .68 & .71 & .75 & .78 & .81 & 2.1\\
 & B & .28 & .37 & .44 & .53 & \textbf{.62} & \textbf{.68} & \textbf{.75} & \textbf{.81} & \textbf{.89} & \textbf{.98} & \textbf{1.4} \\
 & C & .27 & .37 & .45 & \textbf{.54} & .61 & .66 & .71 & .75 & .81 & .86 & 2.4\\
 & D & .18 & .28 & .38 & .47 & .54 & .6 & .68 & .71 & .8 & .86 & 2.7\\
 & E & .27 & .38 & \textbf{.47} & .53 & .61 & .66 & .72 & .76 & .83 & .9 & 2.2\\
 & F & .27 & .37 & .44 & .51 & .58 & .64 & .7 & .75 & .83 & .88 & 2.1\\
 & G & .27 & .35 & .42 & .49 & .56 & .62 & .68 & .73 & .82 & .88 & 2.1\\
\hline
\end{tabular}
}
\end{table}

==> tables/evaluationTable_shortest_goals.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MS, PLR, LPBased, VSAPN) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{4}{*}{\rotatebox[origin=c]{90}{average}}
 & A & .32 & .39 & .44 & .51 & .57 & .61 & .65 & .69 & .69 & .71 & 1.6\\
 & B & .34 & .38 & .43 & .46 & .54 & .61 & .67 & .75 & .82 & .91 & 1.2\\
 & C & .2 & .29 & .33 & .38 & .46 & .51 & .56 & .62 & .68 & .72 & 3.5\\
 & D & \textbf{.37} & \textbf{.44} & \textbf{.5} & \textbf{.58} & \textbf{.7} & \textbf{.78} & \textbf{.83} & \textbf{.86} & \textbf{.89} & \textbf{.92} & \textbf{1.1} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{blocks-world}}
 & A & .07 & .09 & .11 & .14 & .23 & .23 & .24 & .31 & .38 & .38 & 2.3\\
 & B & .15 & .15 & .17 & .17 & .28 & .35 & .38 & .5 & \textbf{.67} & \textbf{.69} & \textbf{1.2} \\
 & C & .05 & .06 & .06 & .08 & .17 & .18 & .21 & .32 & .33 & .36 & 9.7\\
 & D & \textbf{.2} & \textbf{.2} & \textbf{.21} & \textbf{.23} & \textbf{.43} & \textbf{.43} & \textbf{.44} & \textbf{.56} & .63 & .66 & 1.7\\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{campus}}
 & A & .53 & .57 & .53 & .6 & .6 & .63 & .73 & .73 & .57 & .57 & 1.7\\
 & B & \textbf{.93} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & C & .7 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.1\\
 & D & .87 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{depots}}
 & A & .25 & .22 & .22 & \textbf{.32} & .33 & .35 & .5 & .51 & .5 & .59 & 1.5\\
 & B & .2 & .23 & .23 & .27 & .3 & .36 & .57 & .61 & .63 & \textbf{.86} & 1.3\\
 & C & .12 & .2 & .17 & .25 & .24 & .34 & .41 & .47 & .6 & .72 & 2.8\\
 & D & \textbf{.29} & \textbf{.29} & \textbf{.36} & \textbf{.32} & \textbf{.36} & \textbf{.61} & \textbf{.68} & \textbf{.71} & \textbf{.75} & .82 & \textbf{1.0} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & A & .18 & .25 & .23 & .26 & .26 & .33 & .38 & .4 & .36 & .39 & 1.6\\
 & B & .17 & .19 & .27 & .37 & .48 & .59 & .59 & .6 & .74 & .76 & 1.3\\
 & C & .18 & .22 & .23 & .25 & .48 & .48 & .49 & .53 & .6 & .62 & 3.2\\
 & D & \textbf{.41} & \textbf{.39} & \textbf{.42} & \textbf{.51} & \textbf{.62} & \textbf{.69} & \textbf{.81} & \textbf{.82} & \textbf{.81} & \textbf{.85} & \textbf{1.0} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{dwr}}
 & A & .06 & .04 & .12 & .16 & .21 & .25 & .19 & .26 & .3 & .27 & 1.4\\
 & B & .43 & \textbf{.39} & \textbf{.43} & \textbf{.43} & \textbf{.43} & .46 & .43 & .5 & .63 & \textbf{.84} & \textbf{1.0} \\
 & C & .2 & .23 & .23 & .25 & .29 & .33 & .32 & .3 & .36 & .48 & 2.5\\
 & D & \textbf{.46} & \textbf{.39} & .39 & \textbf{.43} & \textbf{.43} & \textbf{.54} & \textbf{.64} & \textbf{.61} & \textbf{.68} & .82 & \textbf{1.0} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & \textbf{.35} & \textbf{.38} & \textbf{.49} & \textbf{.54} & \textbf{.63} & \textbf{.65} & \textbf{.7} & \textbf{.76} & .81 & .93 & 2.4\\
 & B & .09 & .09 & .14 & .15 & .26 & .32 & .42 & .49 & .68 & \textbf{1.0} & 1.7\\
 & C & .15 & .23 & .3 & .36 & .37 & .44 & .49 & .55 & .68 & .78 & 3.4\\
 & D & .2 & .24 & .35 & .42 & .47 & .5 & \textbf{.7} & \textbf{.76} & \textbf{.84} & .94 & \textbf{1.0} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{ferry}}
 & A & .33 & .6 & .73 & .74 & .89 & .89 & .95 & .96 & .96 & .96 & 1.4\\
 & B & .38 & .52 & .52 & .59 & .71 & .75 & .79 & .96 & .95 & .96 & \textbf{1.0} \\
 & C & .16 & .25 & .38 & .45 & .53 & .58 & .63 & .69 & .74 & .75 & 3.2\\
 & D & \textbf{.48} & \textbf{.7} & \textbf{.8} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{intrusion-detection}}
 & A & \textbf{.65} & \textbf{.84} & \textbf{.86} & \textbf{.89} & .98 & .98 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.3\\
 & B & .33 & .37 & .63 & .66 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & C & .12 & .38 & .37 & .4 & .58 & .67 & .72 & .77 & .89 & .89 & 3.5\\
 & D & .13 & .13 & .14 & .38 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{logistics}}
 & A & .24 & .36 & .55 & .55 & .53 & .58 & .64 & .71 & .84 & .86 & 1.4\\
 & B & .3 & .47 & .54 & .59 & .62 & .67 & .77 & .86 & .98 & .99 & 1.1\\
 & C & .13 & .24 & .27 & .33 & .37 & .39 & .49 & .52 & .55 & .57 & 3.8\\
 & D & \textbf{.45} & \textbf{.57} & \textbf{.66} & \textbf{.74} & \textbf{.82} & \textbf{.89} & \textbf{.98} & \textbf{.98} & \textbf{.99} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & \textbf{.73} & \textbf{.81} & \textbf{.9} & \textbf{.92} & \textbf{.96} & .96 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.2\\
 & B & .7 & .73 & .88 & .86 & .84 & .89 & .91 & .96 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & C & .24 & .34 & .58 & .61 & .75 & .78 & .84 & .89 & .89 & .9 & 2.1\\
 & D & .29 & .54 & .73 & .75 & .95 & \textbf{.98} & .98 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & .33 & .45 & .47 & \textbf{.77} & \textbf{.85} & .9 & \textbf{.96} & \textbf{.96} & \textbf{.96} & \textbf{.96} & 1.3\\
 & B & .29 & .32 & .36 & .45 & .48 & .55 & .71 & .82 & .86 & .86 & \textbf{0.9} \\
 & C & .22 & .29 & .37 & .43 & .54 & .6 & .73 & .78 & .82 & .82 & 2.8\\
 & D & \textbf{.38} & \textbf{.5} & \textbf{.58} & .67 & .83 & \textbf{.96} & \textbf{.96} & \textbf{.96} & \textbf{.96} & \textbf{.96} & 1.0\\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{satellite}}
 & A & .26 & .28 & .34 & .43 & \textbf{.56} & .73 & .78 & .89 & .89 & .89 & 2.3\\
 & B & .25 & .25 & .28 & .27 & .3 & .57 & .75 & .89 & .96 & .96 & 1.1\\
 & C & .16 & .17 & .19 & .23 & .29 & .38 & .48 & .6 & .64 & .64 & 4.1\\
 & D & \textbf{.32} & \textbf{.36} & \textbf{.39} & \textbf{.45} & .5 & \textbf{.79} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & .22 & .19 & .17 & .29 & .23 & .23 & .23 & .27 & .22 & .19 & 1.2\\
 & B & .25 & .25 & .26 & .26 & .35 & .35 & .38 & .47 & .48 & \textbf{.93} & 2.2\\
 & C & .2 & .24 & .28 & \textbf{.45} & .46 & .56 & \textbf{.67} & \textbf{.75} & .81 & .87 & 2.9\\
 & D & \textbf{.29} & \textbf{.29} & \textbf{.36} & .43 & \textbf{.57} & \textbf{.61} & .64 & \textbf{.75} & \textbf{.86} & .86 & \textbf{1.0} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & .22 & .33 & .47 & .51 & .73 & .78 & .81 & \textbf{.9} & .9 & .9 & 1.9\\
 & B & .32 & .32 & .36 & .39 & .46 & .63 & .66 & .84 & .91 & .92 & \textbf{1.0} \\
 & C & .17 & .2 & .25 & .28 & .31 & .37 & .4 & .53 & .65 & .67 & 4.1\\
 & D & \textbf{.36} & \textbf{.57} & \textbf{.61} & \textbf{.79} & \textbf{.86} & \textbf{.89} & \textbf{.89} & .89 & \textbf{.96} & \textbf{.96} & \textbf{1.0} \\
\hline
\end{tabular}
}
\end{table}

==> tables/evaluationTable_v1.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MS(A), PLR(B), RG09(C), VSG(D), VSA(E), VSM(F)) when applied to different domains.}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|ll|l}
\multicolumn{1}{c}{}                 & \multicolumn{1}{c|}{} & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}                          & \multicolumn{2}{c|}{\textbf{T}} & \textbf{S} \\
                                     &                                   & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & 0.8 & 0.9 & 1      & $t_{1}$   & $t_{2}$              &  \\ \hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{block-worlds}}        & A                    &0.65   &0.63   &0.61   &0.62   &0.69   &0.71   &0.73   &0.74   &0.78   &0.79      & 6.8         & 9.3              & 0   \\
                                                 & B                   &0.2   &0.27   &0.23   &0.37   &0.55   &0.68   &0.75   &0.8   &0.97   &1.0      & 0.05         & 0              & 0    \\
                                                 & C                  &0.86   &0.73   &0.65   &0.68   &0.71   &0.86   &0.9   &0.9   &0.97   &1.0      & 0         & 0.36              & 0    \\
                                                 & D                   &0.86   &0.73   &0.65   &0.68   &0.71   &0.84   &0.88   &0.88   &1.0   &1.0      & 0.003         & 0              & 0    \\
                                                 & E                   &0.86   &0.73   &0.65   &0.68   &0.71   &0.84   &0.88   &0.88   &1.0   &1.0      & 0.03         & 0              & 0    \\
                                                 & F                   &0.86   &0.73   &0.65   &0.68   &0.71   &0.84   &0.88   &0.88   &1.0   &1.0      & 0.03         & 0              & 0    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{depots}}                          & A                    &0.36   &0.25   &0.25   &0.32   &0.46   &0.54   &0.5   &0.57   &0.61   &0.61      & 4.8         & 4.6              & 0    \\
                                                 & B                   &0.14   &0.21   &0.21   &0.29   &0.46   &0.75   &0.86   &0.96   &1.0   &1.0      & 0.13         & 0              & 0    \\
                                                 & C                  &0.82   &0.79   &0.57   &0.68   &0.79   &0.86   &0.79   &0.82   &0.75   &0.93      & 0         & 0.53              & 0   \\
                                                 & D                   &0.64   &0.5   &0.54   &0.43   &0.57   &0.64   &0.75   &0.79   &0.89   &0.93      & 0.007         & 0              & 0    \\
                                                 & E                   &0.71   &0.75   &0.79   &0.71   &0.89   &0.96   &0.96   &1.0   &1.0   &1.0      & 0.03         & 0              & 0    \\
                                                 & F                   &0.68   &0.61   &0.68   &0.68   &0.75   &0.82   &0.86   &0.89   &0.93   &0.93      & 0.03         & 0              & 0    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{driverlog}}            & A                    &0.46   &0.54   &0.64   &0.79   &0.86   &0.93   &0.96   &0.93   &0.93   &1.0      & 0.098         & 0.14              & 0    \\
                                                 & B                   &0.82   &0.75   &0.82   &0.86   &0.89   &0.86   &0.93   &0.96   &0.96   &1.0      & 0.51         & 0              & 0    \\
                                                 & C                  &1.0   &0.96   &0.96   &0.96   &0.92   &0.96   &0.96   &0.96   &0.96   &0.96       & 0         & 0.27              & 0    \\
                                                 & D                   &0.82   &0.79   &0.86   &0.79   &0.79   &0.82   &0.89   &0.89   &0.93   &0.93      & 0.01         & 0              & 0    \\
                                                 & E                   &0.86   &0.75   &0.75   &0.71   &0.75   &0.75   &0.82   &0.86   &0.89   &0.93      & 0.04         & 0              & 0    \\
                                                 & F                   &0.86   &0.71   &0.71   &0.71   &0.79   &0.82   &0.86   &0.86   &0.86   &0.89      & 0.04         & 0              & 0    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{dwr}}                             & A                    &0.36   &0.39   &0.39   &0.57   &0.57   &0.64   &0.64   &0.71   &0.75   &0.79      & 3.9         & 3.4              & 0    \\
                                                 & B                   &0.5   &0.61   &0.61   &0.57   &0.61   &0.61   &0.68   &0.79   &0.89   &1.0      & 0.14         & 0              & 0    \\
                                                 & C                  &0.88   &0.82   &0.78   &0.63   &0.5   &0.55   &0.6   &0.57   &0.57   &0.63      & 0         & 1.6              & 0    \\
                                                 & D                   &0.82   &0.82   &0.79   &0.54   &0.61   &0.61   &0.57   &0.64   &0.68   &0.82      & 0.009         & 0              & 0    \\
                                                 & E                   &0.79   &0.75   &0.75   &0.64   &0.71   &0.68   &0.68   &0.75   &0.89   &0.89      & 0.05         & 0              & 0    \\
                                                 & F                   &0.89   &0.79   &0.71   &0.57   &0.5   &0.64   &0.57   &0.68   &0.86   &0.93      & 0.05         & 0              & 0    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}        & A                    &0.7   &0.85   &0.89   &0.96   &0.9   &0.92   &0.94   &0.94   &0.94   &0.94      & 0.01         & 0.01              & 0    \\
                                                 & B                   &0.39   &0.4   &0.42   &0.46   &0.43   &0.5   &0.56   &0.61   &0.7   &1.0      & 0.54         & 0              & 0    \\
                                                 & C                  &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0      & 0         & 0.54              & 0    \\
                                                 & D                   &0.95   &0.92   &0.93   &0.91   &0.89   &0.89   &0.89   &0.89   &0.9   &0.93      & 0.04         & 0              & 0    \\
                                                 & E                   &0.87   &0.84   &0.86   &0.84   &0.84   &0.86   &0.89   &0.89   &0.9   &0.93      & 0.07         & 0              & 0    \\
                                                 & F                   &0.89   &0.85   &0.87   &0.85   &0.85   &0.85   &0.88   &0.88   &0.9   &0.93      & 0.06         & 0              & 0    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{ferry}}                           & A                    &0.71   &0.89   &0.89   &0.89   &0.93   &0.96   &0.93   &0.96   &0.96   &0.96      & 0.02         & 0.01              & 0    \\
                                                 & B                   &0.64   &0.79   &0.86   &0.93   &0.93   &0.96   &0.96   &0.96   &0.96   &0.96      & 0.09         & 0              & 0    \\
                                                 & C                  &1.0   &1.0   &0.96   &1.0   &1.0   &1.0   &1.0   &0.96   &0.96   &0.96      & 0         & 0.33              & 0    \\
                                                 & D                   &1.0   &1.0   &0.96   &0.96   &0.96   &0.96   &0.96   &0.96   &0.96   &0.96      & 0.005         & 0              & 0    \\
                                                 & E                   &1.0   &1.0   &0.96   &0.96   &0.96   &0.96   &0.96   &0.96   &0.96   &0.96      & 0.02         & 0              & 0    \\
                                                 & F                   &1.0   &1.0   &0.96   &0.96   &0.96   &0.96   &0.96   &0.96   &0.96   &0.96       & 0.02         & 0              & 0    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{\scriptsize{intrusion-detection}}}   & A                    &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0      & 0.008         & 0.008              & 0    \\
                                                 & B                   &0.24   &0.42   &0.76   &0.88   &0.91   &0.91   &1.0   &1.0   &1.0   &1.0      & 0.03         & 0              & 0    \\
                                                 & C                  &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0     & 0         & 0.11              & 0    \\
                                                 & D                   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0      & 0.002         & 0              & 0    \\
                                                 & E                   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0      & 0.007         & 0              & 0    \\
                                                 & F                   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0      & 0.006         & 0              & 0    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{logistics}}                       & A                    &0.73   &0.72   &0.72   &0.75   &0.82   &0.85   &0.85   &0.94   &1.0   &1.0      & 0.02         & 0.01              & 0    \\
                                                 & B                   &0.45   &0.47   &0.53   &0.63   &0.6   &0.7   &0.8   &0.95   &1.0   &1.0      & 0.15         & 0              & 0    \\
                                                 & C                  &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0      & 0         & 0.57              & 0    \\
                                                 & D                   &0.95   &0.95   &0.95   &0.92   &0.94   &0.94   &1.0   &1.0   &1.0   &1.0      & 0.01         & 0              & 0    \\
                                                 & E                   &0.9   &0.93   &0.95   &0.92   &0.92   &0.92   &0.97   &1.0   &1.0   &1.0      & 0.06         & 0              & 0    \\
                                                 & F                   &0.88   &0.85   &0.82   &0.84   &0.84   &0.84   &0.92   &0.97   &1.0   &1.0      & 0.06         & 0              & 0    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{miconic}}                         & A                    &0.86   &0.89   &0.93   &0.96   &0.93   &0.93   &0.96   &1.0   &1.0   &1.0      & 0.02         & 0.02              & 0    \\
                                                 & B                   &0.75   &0.93   &0.93   &0.93   &0.96   &0.96   &0.96   &1.0   &1.0   &1.0      & 1.64         & 0              & 0    \\
                                                 & C                  &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0      & 0         & 0.53              & 0    \\
                                                 & D                   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0      & 0.02         & 0              & 0    \\
                                                 & E                   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0      & 0.07         & 0              & 0    \\
                                                 & F                   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0       & 0.08         & 0              & 0    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{rovers}}                          & A                    &0.71   &0.82   &0.86   &0.96   &0.96   &1.0   &1.0   &1.0   &1.0   &1.0      & 0.02         & 0.02              & 0    \\
                                                 & B                   &0.86   &0.86   &0.89   &0.93   &0.93   &1.0   &1.0   &1.0   &1.0   &1.0      & 1.03         & 0              & 0    \\
                                                 & C                  &0.96   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0   &1.0      & 0         & 0.26              & 0    \\
                                                 & D                   &1.0   &0.93   &0.96   &0.96   &0.96   &0.96   &0.96   &1.0   &1.0   &1.0      & 0.01         & 0              & 0    \\
                                                 & E                   &0.96   &0.93   &0.93   &0.96   &0.93   &0.96   &1.0   &1.0   &1.0   &1.0      & 0.11         & 0              & 0    \\
                                                 & F                   &0.96   &0.86   &0.89   &0.93   &0.93   &0.96   &0.93   &0.93   &0.93   &0.93      & 0.11         & 0              & 0    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{satellite}}                       & A                    &0.75   &0.71   &0.75   &0.79   &0.86   &0.89   &0.96   &0.96   &0.96   &0.96      & 0.02         & 0.01              & 0    \\
                                                 & B                   &0.96   &0.96   &0.96   &0.93   &0.93   &0.93   &0.89   &0.93   &0.93   &0.93      & 0.26         & 0              & 0    \\
                                                 & C                  &0.96   &0.93   &0.93   &0.96   &0.96   &0.93   &0.93   &0.93   &0.93   &0.93      & 0         & 0.22              & 0    \\
                                                 & D                   &0.96   &0.92   &0.96   &0.96   &0.96   &0.96   &0.96   &0.96   &0.96   &0.96      & 0.007         & 0              & 0    \\
                                                 & E                   &0.75   &0.64   &0.64   &0.64   &0.61   &0.75   &0.68   &0.75   &0.75   &0.79        & 0              & 0        & 0    \\
                                                 & F                   &0.75   &0.68   &0.57   &0.61   &0.64   &0.68   &0.79   &0.82   &0.82   &0.86         & 0              & 0       & 0    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{sokoban}}                         & A                    &0.46   &0.32   &0.18   &0.14   &0.29   &0.32   &0.36   &0.25   &0.29   &0.36      & 0.05         & 0.04              & 0    \\
                                                 & B                   &0.68   &0.61   &0.46   &0.54   &0.61   &0.68   &0.79   &0.79   &0.86   &1.0      & 1.27         & 0              & 0    \\
                                                 & C                  &1.0   &0.86   &0.79   &0.86   &0.89   &0.86   &0.86   &0.86   &0.86   &0.89      & 0         & 1.02              & 0    \\
                                                 & D                   &0.5   &0.54   &0.63   &0.58   &0.63   &0.67   &0.58   &0.63   &0.58   &0.67      & 0.03         & 0              & 0    \\
                                                 & E                   &0.5   &0.32   &0.5   &0.5   &0.5   &0.54   &0.54   &0.57   &0.61   &0.64         & 0              & 0           & 0    \\
                                                 & F                   &0.64   &0.39   &0.54   &0.5   &0.46   &0.5   &0.5   &0.57   &0.64   &0.71         & 0              & 0          & 0    \\ \hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{zeno-travel}}           & A                    &0.46   &0.43   &0.68   &0.75   &0.89   &0.96   &0.96   &1.0   &1.0   &1.0      & 0.02         & 0.02              & 0    \\
                                                 & B                   &0.89   &0.93   &0.96   &0.93   &0.96   &0.96   &1.0   &1.0   &1.0   &1.0      & 2.8         & 0              & 0    \\
                                                 & C                  &0.86   &0.64   &0.64   &0.71   &0.79   &0.89   &0.93   &1.0   &1.0   &1.0      & 0         & 0.39              & 0    \\
                                                 & D                   &0.68   &0.75   &0.82   &0.79   &0.86   &0.86   &0.89   &0.86   &0.93   &0.96      & 0.006         & 0              & 0    \\
                                                 & E                   &0.57   &0.36   &0.57   &0.57   &0.68   &0.75   &0.75   &0.68   &0.75   &0.82      & 0.05         & 0              & 0    \\
                                                 & F                   &0.54   &0.46   &0.54   &0.54   &0.61   &0.68   &0.71   &0.68   &0.71   &0.86       & 0.06         & 0              & 0   
\end{tabular}
}
\end{table}

==> tables/evaluationTable_v2.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MastersSardina, Landmarks-EX-wInitial, RG09, LPBased, VS-euclidean, VSAPN) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{6}{*}{\rotatebox[origin=c]{90}{average}}
 & A & .35 & .43 & .49 & .57 & .63 & .67 & .73 & .77 & .79 & .81 & 1.9\\
 & B & .33 & .44 & .54 & .61 & .68 & .73 & .8 & .85 & \textbf{.9} & \textbf{.96} & 1.5\\
 & C & .32 & .43 & .5 & .59 & .65 & .69 & .75 & .78 & .82 & .86 & 2.2\\
 & D & .19 & .3 & .38 & .46 & .54 & .59 & .66 & .69 & .77 & .81 & 2.4\\
 & E & \textbf{.37} & .47 & .54 & .63 & .68 & .73 & .78 & .81 & .86 & .89 & \textbf{1.4} \\
 & F & .35 & \textbf{.48} & \textbf{.57} & \textbf{.64} & \textbf{.7} & \textbf{.75} & \textbf{.82} & \textbf{.85} & .9 & .93 & 1.6\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{blocks-world}}
 & A & .1 & .13 & .14 & .24 & .29 & .36 & .41 & .47 & .54 & .55 & 7.1\\
 & B & .09 & .23 & \textbf{.28} & .32 & .43 & \textbf{.56} & \textbf{.62} & \textbf{.71} & \textbf{.85} & \textbf{.92} & \textbf{1.5} \\
 & C & .08 & .22 & .23 & .29 & .38 & .42 & .53 & .63 & .81 & .9 & 4.1\\
 & D & .06 & .13 & .15 & .2 & .33 & .38 & .46 & .52 & .76 & .81 & 5.4\\
 & E & \textbf{.11} & \textbf{.24} & .24 & \textbf{.38} & \textbf{.49} & .52 & .61 & .61 & .8 & .84 & \textbf{1.5} \\
 & F & .07 & .21 & .2 & .26 & .39 & .41 & .5 & .55 & .74 & .81 & 3.4\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{campus}}
 & A & \textbf{.73} & .73 & .73 & .53 & .57 & .43 & .57 & .63 & .6 & .6 & 1.4\\
 & B & \textbf{.73} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & C & \textbf{.73} & .8 & .8 & .83 & .83 & .83 & .83 & .8 & .8 & .8 & 1.2\\
 & D & .5 & .87 & .87 & .97 & .97 & .97 & .97 & .97 & .97 & .97 & 1.2\\
 & E & .67 & .9 & .9 & .9 & .87 & .93 & .97 & .93 & .93 & .93 & 1.2\\
 & F & .67 & .9 & .9 & .9 & .87 & .93 & .97 & .93 & .93 & .93 & 1.2\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{depots}}
 & A & \textbf{.21} & .16 & .16 & .22 & .38 & .49 & .48 & .54 & .59 & .59 & 1.8\\
 & B & .13 & .17 & .24 & .27 & .33 & .42 & \textbf{.75} & .83 & .91 & .93 & 1.9\\
 & C & .16 & \textbf{.29} & .28 & \textbf{.32} & .45 & .62 & .59 & .6 & .61 & .78 & 2.6\\
 & D & .09 & .16 & .17 & .27 & .34 & .44 & .57 & .69 & .75 & .89 & 2.4\\
 & E & .2 & .18 & .18 & .25 & .32 & .43 & .55 & .59 & .68 & .82 & \textbf{1.2} \\
 & F & .16 & .27 & \textbf{.33} & .23 & \textbf{.49} & \textbf{.63} & .71 & \textbf{.88} & \textbf{.95} & \textbf{.95} & 1.6\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & A & .29 & \textbf{.37} & .5 & \textbf{.63} & \textbf{.73} & \textbf{.84} & \textbf{.92} & \textbf{.91} & \textbf{.91} & \textbf{.96} & 1.4\\
 & B & .19 & .33 & .42 & .54 & .64 & .71 & .75 & .84 & .88 & .92 & \textbf{1.3} \\
 & C & .22 & .27 & .35 & .46 & .52 & .6 & .75 & .77 & .81 & .81 & 2.9\\
 & D & .2 & .26 & .37 & .5 & .58 & .68 & .67 & .68 & .76 & .8 & 2.3\\
 & E & .26 & .32 & .37 & .41 & .48 & .59 & .71 & .71 & .79 & .75 & \textbf{1.3} \\
 & F & \textbf{.3} & \textbf{.37} & \textbf{.59} & .58 & .64 & .66 & .84 & .89 & .89 & .91 & 1.4\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{dwr}}
 & A & .13 & .23 & .2 & .34 & .34 & .39 & .43 & .47 & .46 & .55 & 2.0\\
 & B & \textbf{.36} & \textbf{.38} & \textbf{.46} & \textbf{.54} & \textbf{.52} & \textbf{.5} & \textbf{.66} & \textbf{.77} & \textbf{.91} & \textbf{1.0} & 1.2\\
 & C & .25 & .33 & .32 & .26 & .2 & .22 & .3 & .27 & .31 & .41 & 2.7\\
 & D & .19 & .18 & .24 & .29 & .28 & .33 & .51 & .51 & .65 & .81 & 2.0\\
 & E & .23 & .27 & .34 & .3 & .3 & .36 & .39 & .39 & .57 & .71 & \textbf{1.0} \\
 & F & .26 & .35 & .37 & .45 & .42 & .49 & .62 & .69 & .77 & .86 & 1.5\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & .29 & .32 & .44 & \textbf{.52} & .56 & .63 & \textbf{.71} & .76 & .83 & .94 & 2.4\\
 & B & .09 & .09 & .14 & .15 & .26 & .32 & .42 & .51 & .68 & \textbf{1.0} & \textbf{1.6} \\
 & C & .32 & .34 & .45 & .48 & .57 & .63 & .69 & \textbf{.78} & \textbf{.85} & \textbf{1.0} & 3.0\\
 & D & .13 & .24 & .28 & .35 & .39 & .47 & .5 & .57 & .7 & .78 & 3.3\\
 & E & \textbf{.34} & \textbf{.38} & .45 & .51 & .6 & \textbf{.65} & .68 & .77 & .84 & .93 & 2.2\\
 & F & .31 & \textbf{.38} & \textbf{.46} & .51 & \textbf{.61} & \textbf{.65} & .68 & .77 & .83 & .93 & 2.7\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{ferry}}
 & A & .38 & \textbf{.7} & \textbf{.8} & .83 & .89 & .95 & .93 & .96 & .96 & .96 & \textbf{1.2} \\
 & B & .37 & .56 & .7 & .82 & .88 & .95 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & C & .28 & .58 & .73 & .8 & .89 & .91 & .95 & .96 & .96 & .96 & 1.6\\
 & D & .19 & .34 & .54 & .75 & .85 & .88 & .91 & .91 & .93 & .96 & 2.1\\
 & E & \textbf{.45} & .62 & .7 & .82 & .91 & \textbf{.98} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & F & .28 & .56 & .73 & \textbf{.89} & \textbf{.96} & .96 & .98 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.6\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{intrusion-detection}}
 & A & \textbf{.26} & \textbf{.45} & .59 & \textbf{.8} & \textbf{.83} & \textbf{.83} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.8\\
 & B & .22 & .4 & \textbf{.65} & .77 & .81 & .81 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.1} \\
 & C & \textbf{.26} & \textbf{.45} & .59 & \textbf{.8} & \textbf{.83} & \textbf{.83} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.8\\
 & D & .18 & .24 & .35 & .38 & .66 & .67 & .72 & .78 & .94 & .96 & 2.9\\
 & E & \textbf{.26} & \textbf{.45} & .59 & \textbf{.8} & \textbf{.83} & \textbf{.83} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.8\\
 & F & \textbf{.26} & \textbf{.45} & .59 & \textbf{.8} & \textbf{.83} & \textbf{.83} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.8\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{kitchen}}
 & A & \textbf{.7} & .77 & .87 & \textbf{.87} & .67 & .67 & .8 & .9 & \textbf{.9} & \textbf{.9} & \textbf{1.2} \\
 & B & .58 & \textbf{.8} & \textbf{.9} & .8 & .8 & .83 & .73 & .8 & .8 & .8 & 1.3\\
 & C & .66 & .73 & .77 & .83 & .83 & .83 & .83 & \textbf{.93} & .8 & .8 & 1.4\\
 & E & \textbf{.7} & .77 & .87 & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & .87 & .77 & .77 & \textbf{1.2} \\
 & F & \textbf{.7} & .77 & .87 & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & .87 & .77 & .77 & \textbf{1.2} \\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{logistics}}
 & A & .35 & .41 & .47 & .6 & .7 & .73 & .76 & \textbf{.89} & \textbf{.97} & \textbf{1.0} & \textbf{1.5} \\
 & B & .27 & .32 & .4 & .56 & .62 & .66 & .72 & .8 & .88 & .91 & 2.4\\
 & C & .34 & .47 & \textbf{.58} & \textbf{.69} & .72 & \textbf{.77} & \textbf{.8} & .82 & .93 & \textbf{1.0} & 1.9\\
 & D & .16 & .35 & .41 & .48 & .5 & .53 & .68 & .68 & .69 & .74 & 3.7\\
 & E & .36 & \textbf{.5} & .52 & .67 & \textbf{.74} & .76 & .79 & .88 & .95 & \textbf{1.0} & 1.6\\
 & F & \textbf{.4} & .47 & .56 & .64 & .66 & .73 & .76 & .88 & .95 & \textbf{1.0} & 1.6\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & .41 & .65 & .73 & \textbf{.84} & .88 & .86 & .89 & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.3\\
 & B & \textbf{.61} & \textbf{.77} & \textbf{.8} & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & C & .32 & .49 & .59 & .74 & .82 & .87 & .9 & .95 & \textbf{1.0} & \textbf{1.0} & 1.7\\
 & D & .24 & .43 & .58 & .57 & .76 & .8 & .82 & .86 & .95 & .93 & 2.0\\
 & E & .51 & .72 & .76 & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.4\\
 & F & .51 & .72 & .76 & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.4\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & .46 & .6 & .69 & .89 & .89 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & B & .46 & .64 & \textbf{.8} & .88 & .88 & .91 & .95 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & C & .43 & .6 & .74 & \textbf{.91} & \textbf{.92} & .93 & .93 & .96 & .98 & .98 & 1.5\\
 & D & .31 & .48 & .64 & .67 & .7 & .74 & .81 & .84 & .91 & .93 & 2.0\\
 & E & .43 & \textbf{.67} & .77 & .88 & .88 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & F & \textbf{.51} & .64 & .78 & .89 & .88 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.3\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{satellite}}
 & A & .35 & .31 & .36 & .43 & .59 & .66 & .74 & .81 & .81 & .81 & 2.4\\
 & B & .4 & .4 & .54 & .72 & \textbf{.8} & \textbf{.8} & \textbf{.89} & \textbf{.95} & .95 & \textbf{.96} & \textbf{1.6} \\
 & C & .35 & .35 & .42 & .54 & .64 & .62 & .67 & .71 & .74 & .77 & 2.7\\
 & D & .26 & .29 & .38 & .52 & .52 & .62 & .72 & .71 & .72 & .75 & 2.9\\
 & E & .49 & .46 & .51 & .64 & .74 & .76 & .83 & .87 & .88 & .89 & 1.7\\
 & F & \textbf{.51} & \textbf{.47} & \textbf{.6} & \textbf{.73} & .79 & .78 & .85 & .93 & \textbf{.96} & \textbf{.96} & \textbf{1.6} \\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & \textbf{.28} & \textbf{.3} & .16 & .14 & .27 & .3 & .34 & .25 & .29 & .3 & 1.2\\
 & B & .19 & .21 & .24 & .37 & .57 & .61 & .63 & .65 & .69 & \textbf{1.0} & 2.4\\
 & C & .15 & .22 & .32 & .45 & \textbf{.58} & .6 & .61 & \textbf{.68} & .73 & .8 & 2.7\\
 & D & .16 & .25 & \textbf{.36} & \textbf{.5} & .57 & \textbf{.63} & \textbf{.68} & .64 & \textbf{.83} & .87 & 1.9\\
 & E & .13 & .18 & .32 & .43 & .32 & .39 & .43 & .61 & .68 & .71 & \textbf{1.0} \\
 & F & .05 & .25 & \textbf{.36} & .46 & .5 & .57 & .61 & .5 & .71 & .82 & 1.2\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & .32 & .36 & \textbf{.57} & .68 & .82 & .95 & .96 & .98 & \textbf{1.0} & \textbf{1.0} & 1.2\\
 & B & .2 & .34 & .46 & .62 & .83 & .93 & .95 & .96 & \textbf{1.0} & \textbf{1.0} & 1.6\\
 & C & .28 & .29 & .38 & .48 & .59 & .73 & .83 & .89 & .93 & .96 & 1.8\\
 & D & .22 & .3 & .42 & .52 & .6 & .65 & .85 & .92 & .95 & \textbf{1.0} & 2.4\\
 & E & \textbf{.39} & .39 & \textbf{.57} & \textbf{.79} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & F & .33 & \textbf{.41} & .52 & .52 & .68 & .93 & .96 & .96 & \textbf{1.0} & \textbf{1.0} & 1.1\\
\hline
\end{tabular}
}
\end{table}

==> tables/evaluationTable_wKitchen.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MastersSardina, Landmarks-EX-wInitial, RG09, VRL10-woActions) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{4}{*}{\rotatebox[origin=c]{90}{blocks-world}}
 & A & .1 & .13 & .14 & .24 & .29 & .36 & .41 & .47 & .54 & .55 & 7.1\\
 & B & .09 & .23 & \textbf{.28} & \textbf{.32} & \textbf{.43} & \textbf{.56} & \textbf{.62} & \textbf{.71} & \textbf{.85} & \textbf{.92} & \textbf{1.5} \\
 & C & .08 & .22 & .23 & .29 & .38 & .42 & .53 & .63 & .81 & .9 & 4.1\\
 & D & \textbf{.12} & \textbf{.27} & .18 & .27 & .36 & .39 & .53 & .59 & .77 & .87 & 2.5\\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{campus}}
 & A & \textbf{.73} & .73 & .73 & .53 & .57 & .43 & .57 & .63 & .6 & .6 & 1.4\\
 & B & \textbf{.73} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & C & \textbf{.73} & .8 & .8 & .83 & .83 & .83 & .83 & .8 & .8 & .8 & 1.2\\
 & D & .57 & .7 & .7 & .93 & .9 & .93 & .97 & .97 & .97 & .97 & 1.2\\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{depots}}
 & A & \textbf{.21} & .16 & .16 & .22 & .38 & .49 & .48 & .54 & .59 & .59 & 1.8\\
 & B & .13 & .17 & .24 & .27 & .33 & .42 & .75 & .83 & .91 & .93 & 1.9\\
 & C & .16 & \textbf{.29} & .28 & \textbf{.32} & .45 & .62 & .59 & .6 & .61 & .78 & 2.6\\
 & D & .19 & .18 & \textbf{.29} & .23 & \textbf{.5} & \textbf{.7} & \textbf{.86} & \textbf{.86} & \textbf{.96} & \textbf{.96} & \textbf{1.4} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & A & \textbf{.29} & \textbf{.37} & \textbf{.5} & \textbf{.63} & \textbf{.73} & \textbf{.84} & \textbf{.92} & \textbf{.91} & \textbf{.91} & \textbf{.96} & 1.4\\
 & B & .19 & .33 & .42 & .54 & .64 & .71 & .75 & .84 & .88 & .92 & \textbf{1.3} \\
 & C & .22 & .27 & .35 & .46 & .52 & .6 & .75 & .77 & .81 & .81 & 2.9\\
 & D & .19 & .19 & .29 & .36 & .45 & .52 & .68 & .79 & .79 & .79 & 1.7\\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{dwr}}
 & A & .13 & .23 & .2 & .34 & .34 & .39 & .43 & .47 & .46 & .55 & 2.0\\
 & B & \textbf{.36} & \textbf{.38} & \textbf{.46} & \textbf{.54} & \textbf{.52} & \textbf{.5} & \textbf{.66} & \textbf{.77} & \textbf{.91} & \textbf{1.0} & \textbf{1.2} \\
 & C & .25 & .33 & .32 & .26 & .2 & .22 & .3 & .27 & .31 & .41 & 2.7\\
 & D & .22 & .24 & .3 & .26 & .26 & .32 & .39 & .43 & .46 & .57 & \textbf{1.2} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & .29 & .32 & .44 & \textbf{.52} & .56 & .63 & \textbf{.71} & .76 & .83 & .94 & 2.4\\
 & B & .09 & .09 & .14 & .15 & .26 & .32 & .42 & .51 & .68 & \textbf{1.0} & \textbf{1.6} \\
 & C & \textbf{.32} & .34 & \textbf{.45} & .48 & .57 & .63 & .69 & \textbf{.78} & \textbf{.85} & \textbf{1.0} & 3.0\\
 & D & \textbf{.32} & \textbf{.38} & .43 & .5 & \textbf{.6} & \textbf{.64} & .69 & .76 & .84 & .93 & 2.6\\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{ferry}}
 & A & \textbf{.38} & \textbf{.7} & \textbf{.8} & .83 & .89 & .95 & .93 & .96 & .96 & .96 & \textbf{1.2} \\
 & B & .37 & .56 & .7 & .82 & .88 & .95 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & C & .28 & .58 & .73 & .8 & .89 & .91 & .95 & .96 & .96 & .96 & 1.6\\
 & D & .28 & .57 & .76 & \textbf{.89} & \textbf{.96} & \textbf{.96} & .98 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.5\\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{intrusion-detection}}
 & A & \textbf{.26} & \textbf{.45} & .59 & \textbf{.8} & \textbf{.83} & \textbf{.83} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.8\\
 & B & .22 & .4 & \textbf{.65} & .77 & .81 & .81 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.1} \\
 & C & \textbf{.26} & \textbf{.45} & .59 & \textbf{.8} & \textbf{.83} & \textbf{.83} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.8\\
 & D & \textbf{.26} & \textbf{.45} & .59 & \textbf{.8} & \textbf{.83} & \textbf{.83} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.8\\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{kitchen}}
 & A & \textbf{.7} & .77 & .87 & \textbf{.87} & .67 & .67 & .8 & .9 & \textbf{.9} & \textbf{.9} & \textbf{1.2} \\
 & B & .58 & \textbf{.8} & \textbf{.9} & .8 & .8 & .83 & .73 & .8 & .8 & .8 & 1.3\\
 & C & .66 & .73 & .77 & .83 & .83 & .83 & .83 & \textbf{.93} & .8 & .8 & 1.4\\
 & D & \textbf{.7} & .77 & .87 & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & .87 & .77 & .77 & \textbf{1.2} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{logistics}}
 & A & .35 & .41 & .47 & .6 & .7 & .73 & .76 & \textbf{.89} & \textbf{.97} & \textbf{1.0} & \textbf{1.5} \\
 & B & .27 & .32 & .4 & .56 & .62 & .66 & .72 & .8 & .88 & .91 & 2.4\\
 & C & .34 & .47 & .58 & .69 & .72 & \textbf{.77} & \textbf{.8} & .82 & .93 & \textbf{1.0} & 1.9\\
 & D & \textbf{.38} & \textbf{.54} & \textbf{.65} & \textbf{.71} & \textbf{.73} & .76 & .79 & .87 & .95 & \textbf{1.0} & 1.6\\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & .41 & .65 & .73 & \textbf{.84} & .88 & .86 & .89 & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.3\\
 & B & \textbf{.61} & \textbf{.77} & \textbf{.8} & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & C & .32 & .49 & .59 & .74 & .82 & .87 & .9 & .95 & \textbf{1.0} & \textbf{1.0} & 1.7\\
 & D & .51 & .72 & .76 & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.4\\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & .46 & .6 & .69 & .89 & .89 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & B & .46 & \textbf{.64} & .8 & .88 & .88 & .91 & .95 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & C & .43 & .6 & .74 & \textbf{.91} & \textbf{.92} & .93 & .93 & .96 & .98 & .98 & 1.5\\
 & D & \textbf{.51} & .62 & \textbf{.83} & .9 & .88 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{satellite}}
 & A & .35 & .31 & .36 & .43 & .59 & .66 & .74 & .81 & .81 & .81 & 2.4\\
 & B & .4 & \textbf{.4} & \textbf{.54} & \textbf{.72} & \textbf{.8} & .8 & \textbf{.89} & \textbf{.95} & \textbf{.95} & \textbf{.96} & \textbf{1.6} \\
 & C & .35 & .35 & .42 & .54 & .64 & .62 & .67 & .71 & .74 & .77 & 2.7\\
 & D & \textbf{.44} & .39 & .52 & .71 & .76 & \textbf{.81} & .88 & .92 & .93 & .95 & 1.9\\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & \textbf{.28} & \textbf{.3} & .16 & .14 & .27 & .3 & .34 & .25 & .29 & .3 & 1.2\\
 & B & .19 & .21 & .24 & .37 & .57 & \textbf{.61} & \textbf{.63} & .65 & .69 & \textbf{1.0} & 2.4\\
 & C & .15 & .22 & \textbf{.32} & .45 & \textbf{.58} & .6 & .61 & \textbf{.68} & \textbf{.73} & .8 & 2.7\\
 & D & .05 & .25 & .3 & \textbf{.46} & .57 & .5 & .46 & .43 & .57 & .79 & \textbf{1.1} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & .32 & .36 & .57 & .68 & .82 & .95 & .96 & .98 & \textbf{1.0} & \textbf{1.0} & 1.2\\
 & B & .2 & .34 & .46 & .62 & .83 & .93 & .95 & .96 & \textbf{1.0} & \textbf{1.0} & 1.6\\
 & C & .28 & .29 & .38 & .48 & .59 & .73 & .83 & .89 & .93 & .96 & 1.8\\
 & D & \textbf{.45} & \textbf{.68} & \textbf{.8} & \textbf{.86} & \textbf{.95} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.1} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{average}}
 & A & \textbf{.35} & .43 & .49 & .57 & .63 & .67 & .73 & .77 & .79 & .81 & 1.9\\
 & B & .33 & .44 & .54 & .61 & .68 & .73 & \textbf{.8} & \textbf{.85} & \textbf{.9} & \textbf{.96} & \textbf{1.5} \\
 & C & .32 & .43 & .5 & .59 & .65 & .69 & .75 & .78 & .82 & .86 & 2.2\\
 & D & \textbf{.35} & \textbf{.46} & \textbf{.55} & \textbf{.64} & \textbf{.7} & \textbf{.74} & \textbf{.8} & .83 & .87 & .91 & 1.6\\
\hline
\end{tabular}
}
\end{table}

==> tables/evaluationVRL_comparison.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MastersSardina, Landmarks-woInitial, RG09, LPBased, VRL10-woActions) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{5}{*}{\rotatebox[origin=c]{90}{blocks-world}}
 & A & .1 & .13 & .14 & .24 & .29 & .36 & .41 & .47 & .54 & .55 & 7.1\\
 & B & .09 & .18 & .22 & .28 & \textbf{.44} & \textbf{.5} & \textbf{.61} & \textbf{.67} & \textbf{.88} & \textbf{.95} & \textbf{1.5} \\
 & C & .08 & .22 & \textbf{.23} & \textbf{.29} & .38 & .42 & .53 & .63 & .81 & .9 & 4.1\\
 & D & .06 & .13 & .15 & .2 & .33 & .38 & .46 & .52 & .76 & .81 & 5.4\\
 & E & \textbf{.12} & \textbf{.27} & .18 & .27 & .36 & .39 & .53 & .59 & .77 & .87 & 2.5\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{depots}}
 & A & \textbf{.21} & .16 & .16 & .22 & .38 & .49 & .48 & .54 & .59 & .59 & 1.8\\
 & B & .11 & .16 & .15 & .19 & .32 & .6 & .78 & \textbf{.89} & .95 & \textbf{.96} & 1.5\\
 & C & .16 & \textbf{.29} & .28 & \textbf{.32} & .45 & .62 & .59 & .6 & .61 & .78 & 2.6\\
 & D & .09 & .16 & .17 & .27 & .34 & .44 & .57 & .69 & .75 & .89 & 2.4\\
 & E & .19 & .18 & \textbf{.29} & .23 & \textbf{.5} & \textbf{.7} & \textbf{.86} & .86 & \textbf{.96} & \textbf{.96} & \textbf{1.4} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & A & \textbf{.29} & \textbf{.37} & \textbf{.5} & \textbf{.63} & \textbf{.73} & \textbf{.84} & \textbf{.92} & \textbf{.91} & \textbf{.91} & \textbf{.96} & \textbf{1.4} \\
 & B & .17 & .24 & .38 & .46 & .59 & .69 & .75 & .81 & \textbf{.91} & .93 & 1.8\\
 & C & .22 & .27 & .35 & .46 & .52 & .6 & .75 & .77 & .81 & .81 & 2.9\\
 & D & .2 & .26 & .37 & .5 & .58 & .68 & .67 & .68 & .76 & .8 & 2.3\\
 & E & .19 & .19 & .29 & .36 & .45 & .52 & .68 & .79 & .79 & .79 & 1.7\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{dwr}}
 & A & .13 & .23 & .2 & .34 & .34 & .39 & .43 & .47 & .46 & .55 & 2.0\\
 & B & \textbf{.32} & \textbf{.46} & \textbf{.49} & \textbf{.5} & \textbf{.54} & \textbf{.54} & \textbf{.6} & \textbf{.72} & \textbf{.88} & \textbf{1.0} & \textbf{1.1} \\
 & C & .25 & .33 & .32 & .26 & .2 & .22 & .3 & .27 & .31 & .41 & 2.7\\
 & D & .19 & .18 & .24 & .29 & .28 & .33 & .51 & .51 & .65 & .81 & 2.0\\
 & E & .22 & .24 & .3 & .26 & .26 & .32 & .39 & .43 & .46 & .57 & 1.2\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & .29 & .32 & .44 & \textbf{.52} & .56 & .63 & \textbf{.71} & .76 & .83 & .94 & 2.4\\
 & B & .2 & .19 & .23 & .27 & .29 & .34 & .42 & .48 & .62 & \textbf{1.0} & \textbf{1.3} \\
 & C & \textbf{.32} & .34 & \textbf{.45} & .48 & .57 & .63 & .69 & \textbf{.78} & \textbf{.85} & \textbf{1.0} & 3.0\\
 & D & .13 & .24 & .28 & .35 & .39 & .47 & .5 & .57 & .7 & .78 & 3.3\\
 & E & \textbf{.32} & \textbf{.38} & .43 & .5 & \textbf{.6} & \textbf{.64} & .69 & .76 & .84 & .93 & 2.6\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{ferry}}
 & A & .38 & \textbf{.7} & \textbf{.8} & .83 & .89 & .95 & .93 & .96 & .96 & .96 & \textbf{1.2} \\
 & B & \textbf{.4} & .6 & .72 & .81 & .89 & .93 & .96 & .96 & .96 & .96 & \textbf{1.2} \\
 & C & .28 & .58 & .73 & .8 & .89 & .91 & .95 & .96 & .96 & .96 & 1.6\\
 & D & .19 & .34 & .54 & .75 & .85 & .88 & .91 & .91 & .93 & .96 & 2.1\\
 & E & .28 & .57 & .76 & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{.98} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.5\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{logistics}}
 & A & .35 & .41 & .47 & .6 & .7 & .73 & .76 & \textbf{.89} & \textbf{.97} & \textbf{1.0} & \textbf{1.5} \\
 & B & .2 & .23 & .26 & .42 & .43 & .52 & .63 & .79 & .91 & \textbf{1.0} & 1.6\\
 & C & .34 & .47 & .58 & .69 & .72 & \textbf{.77} & \textbf{.8} & .82 & .93 & \textbf{1.0} & 1.9\\
 & D & .16 & .35 & .41 & .48 & .5 & .53 & .68 & .68 & .69 & .74 & 3.7\\
 & E & \textbf{.38} & \textbf{.54} & \textbf{.65} & \textbf{.71} & \textbf{.73} & .76 & .79 & .87 & .95 & \textbf{1.0} & 1.6\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & .41 & .65 & .73 & \textbf{.84} & .88 & .86 & .89 & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.3\\
 & B & \textbf{.61} & \textbf{.77} & \textbf{.8} & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & C & .32 & .49 & .59 & .74 & .82 & .87 & .9 & .95 & \textbf{1.0} & \textbf{1.0} & 1.7\\
 & D & .24 & .43 & .58 & .57 & .76 & .8 & .82 & .86 & .95 & .93 & 2.0\\
 & E & .51 & .72 & .76 & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.4\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & .46 & .6 & .69 & .89 & .89 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & B & .43 & .59 & .8 & .88 & .88 & .9 & .93 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
 & C & .43 & .6 & .74 & \textbf{.91} & \textbf{.92} & .93 & .93 & .96 & .98 & .98 & 1.5\\
 & D & .31 & .48 & .64 & .67 & .7 & .74 & .81 & .84 & .91 & .93 & 2.0\\
 & E & \textbf{.51} & \textbf{.62} & \textbf{.83} & .9 & .88 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.2} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{satellite}}
 & A & .35 & .31 & .36 & .43 & .59 & .66 & .74 & .81 & .81 & .81 & 2.4\\
 & B & .36 & .36 & .49 & .67 & \textbf{.76} & .8 & .86 & \textbf{.92} & .92 & .92 & \textbf{1.8} \\
 & C & .35 & .35 & .42 & .54 & .64 & .62 & .67 & .71 & .74 & .77 & 2.7\\
 & D & .26 & .29 & .38 & .52 & .52 & .62 & .72 & .71 & .72 & .75 & 2.9\\
 & E & \textbf{.44} & \textbf{.39} & \textbf{.52} & \textbf{.71} & \textbf{.76} & \textbf{.81} & \textbf{.88} & \textbf{.92} & \textbf{.93} & \textbf{.95} & 1.9\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & \textbf{.28} & \textbf{.3} & .16 & .14 & .27 & .3 & .34 & .25 & .29 & .3 & 1.2\\
 & B & .17 & .2 & .22 & .38 & .53 & .55 & .61 & .6 & .66 & \textbf{1.0} & 1.5\\
 & C & .15 & .22 & .32 & .45 & \textbf{.58} & .6 & .61 & \textbf{.68} & .73 & .8 & 2.7\\
 & D & .16 & .25 & \textbf{.36} & \textbf{.5} & .57 & \textbf{.63} & \textbf{.68} & .64 & \textbf{.83} & .87 & 1.9\\
 & E & .05 & .25 & .3 & .46 & .57 & .5 & .46 & .43 & .57 & .79 & \textbf{1.1} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & .32 & .36 & .57 & .68 & .82 & .95 & .96 & .98 & \textbf{1.0} & \textbf{1.0} & 1.2\\
 & B & .31 & .41 & .56 & .64 & .82 & .9 & .93 & .96 & \textbf{1.0} & \textbf{1.0} & 1.6\\
 & C & .28 & .29 & .38 & .48 & .59 & .73 & .83 & .89 & .93 & .96 & 1.8\\
 & D & .22 & .3 & .42 & .52 & .6 & .65 & .85 & .92 & .95 & \textbf{1.0} & 2.4\\
 & E & \textbf{.45} & \textbf{.68} & \textbf{.8} & \textbf{.86} & \textbf{.95} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.1} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{average}}
 & A & .3 & .38 & .44 & .53 & .61 & .68 & .71 & .75 & .78 & .81 & 2.1\\
 & B & .28 & .37 & .44 & .53 & .62 & .68 & .75 & \textbf{.81} & \textbf{.89} & \textbf{.98} & \textbf{1.4} \\
 & C & .27 & .37 & .45 & .54 & .61 & .66 & .71 & .75 & .81 & .86 & 2.4\\
 & D & .18 & .28 & .38 & .47 & .54 & .6 & .68 & .71 & .8 & .86 & 2.7\\
 & E & \textbf{.31} & \textbf{.42} & \textbf{.51} & \textbf{.58} & \textbf{.66} & \textbf{.71} & \textbf{.76} & .8 & .86 & .9 & 1.6\\
\hline
\end{tabular}
}
\end{table}

==> tables/fpv_norm_experiment.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (3, 4, 5, 6, 7, 8, 9, 10, 11, 12, 13, 14, 15, 16, 17, 18, 19, 20) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{18}{*}{\rotatebox[origin=c]{90}{average}}
 & A & .39 & .5 & .59 & .65 & .72 & .77 & .83 & .86 & .91 & .94 & \textbf{1.1} \\
 & B & .39 & .49 & .6 & .66 & .72 & .76 & .83 & .86 & .91 & .93 & \textbf{1.1} \\
 & C & .39 & .49 & .6 & .66 & .72 & .77 & .83 & .86 & \textbf{.91} & .94 & \textbf{1.1} \\
 & D & .39 & .49 & .59 & .66 & .72 & .77 & \textbf{.84} & .87 & .91 & .93 & \textbf{1.1} \\
 & E & .4 & .5 & .6 & .65 & .72 & .77 & .83 & .87 & .9 & .94 & \textbf{1.1} \\
 & F & .39 & .5 & .59 & .64 & .71 & .76 & .82 & .87 & .91 & .93 & \textbf{1.1} \\
 & G & .4 & .5 & .58 & .64 & .72 & .76 & .83 & .87 & .91 & .94 & \textbf{1.1} \\
 & H & .39 & .49 & .59 & .65 & .72 & .76 & .83 & .86 & .91 & .94 & \textbf{1.1} \\
 & I & .4 & .5 & \textbf{.61} & .66 & .73 & .77 & .82 & .87 & .91 & .94 & \textbf{1.1} \\
 & J & .39 & .49 & .59 & .65 & .73 & .76 & .83 & .86 & .91 & .93 & \textbf{1.1} \\
 & K & .4 & .48 & .58 & .65 & .71 & .76 & .82 & .87 & .9 & .93 & \textbf{1.1} \\
 & L & .38 & .49 & .58 & .65 & .72 & .76 & .84 & .87 & .91 & .94 & \textbf{1.1} \\
 & M & .39 & .49 & .6 & \textbf{.66} & .72 & .77 & .83 & .87 & .91 & .94 & \textbf{1.1} \\
 & N & .4 & .49 & .6 & .65 & .73 & .77 & .83 & .86 & .91 & .93 & \textbf{1.1} \\
 & O & .4 & \textbf{.51} & .59 & .64 & .72 & .76 & .82 & .86 & .91 & .94 & \textbf{1.1} \\
 & P & .39 & .49 & .59 & .65 & .73 & .76 & .83 & .87 & .91 & \textbf{.94} & \textbf{1.1} \\
 & Q & .39 & .5 & .58 & .65 & \textbf{.74} & \textbf{.77} & .83 & .87 & .91 & .94 & \textbf{1.1} \\
 & R & \textbf{.4} & .51 & .6 & .66 & .73 & .77 & .83 & \textbf{.87} & .91 & .94 & \textbf{1.1} \\
\hline
\multirow{18}{*}{\rotatebox[origin=c]{90}{blocks-world}}
 & A & \textbf{.13} & \textbf{.31} & \textbf{.24} & \textbf{.32} & \textbf{.42} & \textbf{.47} & \textbf{.57} & \textbf{.66} & \textbf{.8} & \textbf{.9} & \textbf{1.5} \\
 & B & \textbf{.13} & \textbf{.31} & \textbf{.24} & \textbf{.32} & \textbf{.42} & \textbf{.47} & \textbf{.57} & \textbf{.66} & \textbf{.8} & \textbf{.9} & \textbf{1.5} \\
 & C & \textbf{.13} & \textbf{.31} & \textbf{.24} & \textbf{.32} & \textbf{.42} & \textbf{.47} & \textbf{.57} & \textbf{.66} & \textbf{.8} & \textbf{.9} & \textbf{1.5} \\
 & D & \textbf{.13} & \textbf{.31} & \textbf{.24} & \textbf{.32} & \textbf{.42} & \textbf{.47} & \textbf{.57} & \textbf{.66} & \textbf{.8} & \textbf{.9} & \textbf{1.5} \\
 & E & \textbf{.13} & \textbf{.31} & \textbf{.24} & \textbf{.32} & \textbf{.42} & \textbf{.47} & \textbf{.57} & \textbf{.66} & \textbf{.8} & \textbf{.9} & \textbf{1.5} \\
 & F & \textbf{.13} & \textbf{.31} & \textbf{.24} & \textbf{.32} & \textbf{.42} & \textbf{.47} & \textbf{.57} & \textbf{.66} & \textbf{.8} & \textbf{.9} & \textbf{1.5} \\
 & G & \textbf{.13} & \textbf{.31} & \textbf{.24} & \textbf{.32} & \textbf{.42} & \textbf{.47} & \textbf{.57} & \textbf{.66} & \textbf{.8} & \textbf{.9} & \textbf{1.5} \\
 & H & \textbf{.13} & \textbf{.31} & \textbf{.24} & \textbf{.32} & \textbf{.42} & \textbf{.47} & \textbf{.57} & \textbf{.66} & \textbf{.8} & \textbf{.9} & \textbf{1.5} \\
 & I & \textbf{.13} & \textbf{.31} & \textbf{.24} & \textbf{.32} & \textbf{.42} & \textbf{.47} & \textbf{.57} & \textbf{.66} & \textbf{.8} & \textbf{.9} & \textbf{1.5} \\
 & J & \textbf{.13} & \textbf{.31} & \textbf{.24} & \textbf{.32} & \textbf{.42} & \textbf{.47} & \textbf{.57} & \textbf{.66} & \textbf{.8} & \textbf{.9} & \textbf{1.5} \\
 & K & \textbf{.13} & \textbf{.31} & \textbf{.24} & \textbf{.32} & \textbf{.42} & \textbf{.47} & \textbf{.57} & \textbf{.66} & \textbf{.8} & \textbf{.9} & \textbf{1.5} \\
 & L & \textbf{.13} & \textbf{.31} & \textbf{.24} & \textbf{.32} & \textbf{.42} & \textbf{.47} & \textbf{.57} & \textbf{.66} & \textbf{.8} & \textbf{.9} & \textbf{1.5} \\
 & M & \textbf{.13} & \textbf{.31} & \textbf{.24} & \textbf{.32} & \textbf{.42} & \textbf{.47} & \textbf{.57} & \textbf{.66} & \textbf{.8} & \textbf{.9} & \textbf{1.5} \\
 & N & \textbf{.13} & \textbf{.31} & \textbf{.24} & \textbf{.32} & \textbf{.42} & \textbf{.47} & \textbf{.57} & \textbf{.66} & \textbf{.8} & \textbf{.9} & \textbf{1.5} \\
 & O & \textbf{.13} & \textbf{.31} & \textbf{.24} & \textbf{.32} & \textbf{.42} & \textbf{.47} & \textbf{.57} & \textbf{.66} & \textbf{.8} & \textbf{.9} & \textbf{1.5} \\
 & P & \textbf{.13} & \textbf{.31} & \textbf{.24} & \textbf{.32} & \textbf{.42} & \textbf{.47} & \textbf{.57} & \textbf{.66} & \textbf{.8} & \textbf{.9} & \textbf{1.5} \\
 & Q & \textbf{.13} & \textbf{.31} & \textbf{.24} & \textbf{.32} & \textbf{.42} & \textbf{.47} & \textbf{.57} & \textbf{.66} & \textbf{.8} & \textbf{.9} & \textbf{1.5} \\
 & R & \textbf{.13} & \textbf{.31} & \textbf{.24} & \textbf{.32} & \textbf{.42} & \textbf{.47} & \textbf{.57} & \textbf{.66} & \textbf{.8} & \textbf{.9} & \textbf{1.5} \\
\hline
\multirow{18}{*}{\rotatebox[origin=c]{90}{campus}}
 & A & \textbf{.77} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{.97} & \textbf{.97} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & B & \textbf{.77} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{.97} & \textbf{.97} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & C & \textbf{.77} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{.97} & \textbf{.97} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & D & \textbf{.77} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{.97} & \textbf{.97} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & E & \textbf{.77} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{.97} & \textbf{.97} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & F & \textbf{.77} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{.97} & \textbf{.97} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & G & \textbf{.77} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{.97} & \textbf{.97} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & H & \textbf{.77} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{.97} & \textbf{.97} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & I & \textbf{.77} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{.97} & \textbf{.97} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & J & \textbf{.77} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{.97} & \textbf{.97} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & K & \textbf{.77} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{.97} & \textbf{.97} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & L & \textbf{.77} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{.97} & \textbf{.97} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & M & \textbf{.77} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{.97} & \textbf{.97} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & N & \textbf{.77} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{.97} & \textbf{.97} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & O & \textbf{.77} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{.97} & \textbf{.97} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & P & \textbf{.77} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{.97} & \textbf{.97} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & Q & \textbf{.77} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{.97} & \textbf{.97} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & R & \textbf{.77} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{.97} & \textbf{.97} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
\hline
\multirow{18}{*}{\rotatebox[origin=c]{90}{depots}}
 & A & .21 & .21 & .25 & .25 & .54 & .68 & .82 & .86 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & B & .21 & .21 & .25 & .29 & .46 & .64 & .86 & .89 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & C & .21 & .21 & .36 & \textbf{.39} & .46 & .68 & .82 & .86 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & D & \textbf{.29} & .29 & \textbf{.43} & \textbf{.39} & \textbf{.64} & .68 & .82 & .82 & .93 & \textbf{1} & \textbf{1} \\
 & E & .21 & .21 & .29 & .32 & .57 & \textbf{.75} & .86 & .93 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & F & .27 & .23 & .3 & .34 & .46 & .7 & .88 & .93 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & G & .23 & .23 & .27 & .3 & .52 & .61 & .86 & .89 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & H & .2 & .16 & .23 & .3 & .48 & .61 & .86 & .89 & \textbf{1} & \textbf{1} & 1.1 \\
 & I & .21 & .25 & \textbf{.43} & \textbf{.39} & .52 & .73 & .84 & .89 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & J & .18 & .21 & .21 & .29 & .54 & .64 & .82 & .89 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & K & .25 & .25 & .29 & .32 & .57 & .73 & .8 & .93 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & L & .21 & .29 & .29 & .32 & .57 & .68 & .86 & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & M & .21 & .21 & .25 & .32 & .54 & .68 & \textbf{.89} & .93 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & N & \textbf{.29} & \textbf{.32} & .36 & .36 & .54 & .71 & .86 & .93 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & O & .2 & .25 & .3 & .29 & .54 & .66 & .79 & .89 & .96 & \textbf{1} & \textbf{1} \\
 & P & .16 & .2 & .27 & .34 & .59 & .68 & .86 & .89 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & Q & .21 & .21 & .32 & \textbf{.39} & .54 & .68 & .79 & .89 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & R & .2 & .2 & .27 & .34 & .55 & .7 & .82 & .89 & \textbf{1} & \textbf{1} & 1.1 \\
\hline
\multirow{18}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & A & .29 & \textbf{.39} & .61 & .61 & .5 & .64 & .79 & .86 & .89 & .89 & \textbf{1} \\
 & B & .36 & \textbf{.39} & \textbf{.68} & .61 & .61 & .64 & .82 & .86 & .89 & .89 & \textbf{1} \\
 & C & .32 & \textbf{.39} & .57 & .57 & .61 & .68 & .82 & .86 & .89 & .89 & \textbf{1} \\
 & D & .29 & .36 & .61 & .57 & .57 & .64 & .86 & \textbf{.89} & .89 & .89 & \textbf{1} \\
 & E & .36 & \textbf{.39} & \textbf{.68} & .64 & .64 & \textbf{.71} & .86 & .86 & .89 & .89 & \textbf{1} \\
 & F & .32 & .32 & .54 & .54 & .57 & .68 & .82 & .86 & .89 & .89 & \textbf{1} \\
 & G & .29 & .32 & .57 & .61 & .68 & \textbf{.71} & .82 & \textbf{.89} & \textbf{.93} & \textbf{.93} & \textbf{1} \\
 & H & .39 & \textbf{.39} & .61 & .64 & .64 & .61 & .82 & .86 & .89 & .89 & \textbf{1} \\
 & I & .36 & \textbf{.39} & .61 & .57 & .64 & .68 & .82 & .86 & .89 & .89 & \textbf{1} \\
 & J & .32 & .29 & .57 & \textbf{.68} & \textbf{.75} & \textbf{.71} & \textbf{.89} & \textbf{.89} & .89 & .89 & \textbf{1} \\
 & K & .39 & .29 & .54 & .5 & .5 & .61 & .86 & .86 & .86 & .86 & \textbf{1} \\
 & L & .29 & .25 & .54 & .57 & .57 & .61 & .82 & .86 & \textbf{.93} & \textbf{.93} & \textbf{1} \\
 & M & .36 & .29 & .64 & .64 & .68 & .64 & .82 & .86 & \textbf{.93} & \textbf{.93} & \textbf{1} \\
 & N & .39 & .36 & .61 & .57 & .64 & .68 & \textbf{.89} & \textbf{.89} & .89 & .89 & \textbf{1} \\
 & O & \textbf{.46} & \textbf{.39} & .57 & .54 & .61 & .68 & .86 & \textbf{.89} & \textbf{.93} & \textbf{.93} & \textbf{1} \\
 & P & .32 & .36 & .57 & .54 & .64 & .64 & .86 & \textbf{.89} & \textbf{.93} & \textbf{.93} & \textbf{1} \\
 & Q & .36 & \textbf{.39} & .57 & .61 & .68 & .64 & .86 & \textbf{.89} & \textbf{.93} & \textbf{.93} & \textbf{1} \\
 & R & \textbf{.46} & \textbf{.39} & .61 & .54 & .61 & .64 & \textbf{.89} & \textbf{.89} & \textbf{.93} & \textbf{.93} & \textbf{1} \\
\hline
\multirow{18}{*}{\rotatebox[origin=c]{90}{dwr}}
 & A & .32 & .46 & .5 & .5 & .43 & \textbf{.54} & \textbf{.64} & .57 & .68 & .89 & \textbf{1} \\
 & B & .32 & .46 & .54 & .5 & .39 & .39 & .57 & .57 & .71 & .82 & \textbf{1} \\
 & C & .32 & .39 & .5 & .43 & .43 & .5 & .61 & .57 & .79 & .89 & \textbf{1} \\
 & D & .29 & .36 & .36 & .43 & .39 & .43 & .61 & .57 & .79 & .82 & \textbf{1} \\
 & E & .32 & .46 & .5 & .46 & .43 & .46 & .57 & .64 & .71 & .89 & \textbf{1} \\
 & F & .21 & .43 & .43 & .46 & .43 & .46 & .61 & .64 & .71 & .82 & \textbf{1} \\
 & G & .36 & \textbf{.54} & .43 & .43 & .36 & .43 & .61 & .61 & .71 & .89 & \textbf{1} \\
 & H & .29 & .39 & .43 & \textbf{.54} & .46 & .5 & .57 & .57 & \textbf{.82} & \textbf{.93} & \textbf{1} \\
 & I & .36 & .5 & \textbf{.57} & .5 & .43 & .46 & .61 & .64 & .75 & \textbf{.93} & \textbf{1} \\
 & J & .36 & .46 & .5 & .46 & .46 & .46 & .57 & .54 & .71 & .82 & \textbf{1} \\
 & K & \textbf{.39} & .46 & .5 & \textbf{.54} & .46 & .43 & .57 & .57 & .71 & .82 & \textbf{1} \\
 & L & .29 & .46 & .46 & .43 & .43 & .46 & \textbf{.64} & .64 & .71 & .89 & \textbf{1} \\
 & M & .32 & .39 & .46 & \textbf{.54} & .43 & .5 & .54 & .54 & .71 & .82 & \textbf{1} \\
 & N & .34 & .38 & .48 & .45 & \textbf{.48} & .45 & .57 & .54 & .71 & .82 & \textbf{1} \\
 & O & .27 & .41 & .43 & .43 & .36 & .43 & .57 & .61 & .79 & .86 & \textbf{1} \\
 & P & .36 & .46 & .54 & .46 & .46 & .5 & .61 & \textbf{.68} & .71 & .89 & \textbf{1} \\
 & Q & .38 & .45 & .45 & .38 & .45 & .52 & .61 & .64 & .75 & .82 & \textbf{1} \\
 & R & .36 & .43 & .43 & .43 & .39 & .46 & .61 & .61 & .71 & .82 & \textbf{1} \\
\hline
\multirow{18}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & .27 & .35 & .42 & .46 & .64 & .65 & .65 & .75 & \textbf{.89} & \textbf{.93} & \textbf{1} \\
 & B & .28 & .34 & .43 & .48 & \textbf{.66} & .66 & .65 & .75 & \textbf{.89} & \textbf{.93} & \textbf{1} \\
 & C & \textbf{.29} & \textbf{.37} & \textbf{.48} & .48 & .65 & .67 & .66 & .76 & \textbf{.89} & \textbf{.93} & \textbf{1} \\
 & D & .27 & .33 & .45 & .47 & .62 & .66 & .68 & .75 & \textbf{.89} & \textbf{.93} & \textbf{1} \\
 & E & .28 & .36 & .47 & .47 & .62 & .65 & .68 & .77 & \textbf{.89} & \textbf{.93} & \textbf{1} \\
 & F & .28 & .36 & .47 & .47 & .62 & .66 & .65 & .77 & \textbf{.89} & \textbf{.93} & \textbf{1} \\
 & G & .27 & .35 & .46 & \textbf{.51} & .64 & .66 & .65 & .77 & \textbf{.89} & \textbf{.93} & \textbf{1} \\
 & H & .27 & .36 & .47 & .47 & .62 & .66 & .68 & .78 & .87 & \textbf{.93} & \textbf{1} \\
 & I & .28 & .34 & .45 & .48 & .64 & .66 & .65 & .77 & \textbf{.89} & \textbf{.93} & \textbf{1} \\
 & J & .27 & .36 & .47 & .49 & .64 & \textbf{.68} & \textbf{.7} & \textbf{.81} & .87 & \textbf{.93} & \textbf{1} \\
 & K & .28 & .32 & .43 & .47 & .62 & .66 & .68 & .75 & .87 & \textbf{.93} & \textbf{1} \\
 & L & .28 & .36 & .47 & .47 & .62 & .66 & .68 & .78 & .87 & \textbf{.93} & \textbf{1} \\
 & M & .28 & .36 & .46 & .49 & .64 & .66 & .68 & .78 & .87 & \textbf{.93} & \textbf{1} \\
 & N & .27 & .34 & .45 & .49 & .64 & \textbf{.68} & \textbf{.7} & .77 & .87 & \textbf{.93} & \textbf{1} \\
 & O & .28 & .34 & .45 & .47 & .62 & .65 & .68 & .77 & .87 & \textbf{.93} & \textbf{1} \\
 & P & .27 & .34 & .45 & .47 & .62 & .65 & .68 & .78 & .87 & \textbf{.93} & \textbf{1} \\
 & Q & \textbf{.29} & .35 & .45 & .49 & .64 & .66 & .65 & .78 & .87 & \textbf{.93} & \textbf{1} \\
 & R & .27 & .36 & .47 & .49 & .64 & .65 & .65 & .78 & .87 & \textbf{.93} & \textbf{1} \\
\hline
\multirow{18}{*}{\rotatebox[origin=c]{90}{ferry}}
 & A & \textbf{.41} & \textbf{.65} & \textbf{.75} & \textbf{.87} & \textbf{.98} & \textbf{.98} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & B & \textbf{.41} & \textbf{.65} & \textbf{.75} & \textbf{.87} & \textbf{.98} & \textbf{.98} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & C & \textbf{.41} & \textbf{.65} & \textbf{.75} & \textbf{.87} & \textbf{.98} & \textbf{.98} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & D & \textbf{.41} & \textbf{.65} & \textbf{.75} & \textbf{.87} & \textbf{.98} & \textbf{.98} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & E & \textbf{.41} & \textbf{.65} & \textbf{.75} & \textbf{.87} & \textbf{.98} & \textbf{.98} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & F & \textbf{.41} & \textbf{.65} & \textbf{.75} & \textbf{.87} & \textbf{.98} & \textbf{.98} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & G & \textbf{.41} & \textbf{.65} & \textbf{.75} & \textbf{.87} & \textbf{.98} & \textbf{.98} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & H & \textbf{.41} & \textbf{.65} & \textbf{.75} & \textbf{.87} & \textbf{.98} & \textbf{.98} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & I & \textbf{.41} & \textbf{.65} & \textbf{.75} & \textbf{.87} & \textbf{.98} & \textbf{.98} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & J & \textbf{.41} & \textbf{.65} & \textbf{.75} & \textbf{.87} & \textbf{.98} & \textbf{.98} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & K & \textbf{.41} & \textbf{.65} & \textbf{.75} & \textbf{.87} & \textbf{.98} & \textbf{.98} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & L & \textbf{.41} & \textbf{.65} & \textbf{.75} & \textbf{.87} & \textbf{.98} & \textbf{.98} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & M & \textbf{.41} & \textbf{.65} & \textbf{.75} & \textbf{.87} & \textbf{.98} & \textbf{.98} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & N & \textbf{.41} & \textbf{.65} & \textbf{.75} & \textbf{.87} & \textbf{.98} & \textbf{.98} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & O & \textbf{.41} & \textbf{.65} & \textbf{.75} & \textbf{.87} & \textbf{.98} & \textbf{.98} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & P & \textbf{.41} & \textbf{.65} & \textbf{.75} & \textbf{.87} & \textbf{.98} & \textbf{.98} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & Q & \textbf{.41} & \textbf{.65} & \textbf{.75} & \textbf{.87} & \textbf{.98} & \textbf{.98} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & R & \textbf{.41} & \textbf{.65} & \textbf{.75} & \textbf{.87} & \textbf{.98} & \textbf{.98} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
\hline
\multirow{18}{*}{\rotatebox[origin=c]{90}{intrusion-detection}}
 & A & \textbf{.22} & \textbf{.4} & \textbf{.65} & \textbf{.77} & \textbf{.81} & \textbf{.81} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.1} \\
 & B & \textbf{.22} & \textbf{.4} & \textbf{.65} & \textbf{.77} & \textbf{.81} & \textbf{.81} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.1} \\
 & C & \textbf{.22} & \textbf{.4} & \textbf{.65} & \textbf{.77} & \textbf{.81} & \textbf{.81} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.1} \\
 & D & \textbf{.22} & \textbf{.4} & \textbf{.65} & \textbf{.77} & \textbf{.81} & \textbf{.81} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.1} \\
 & E & \textbf{.22} & \textbf{.4} & \textbf{.65} & \textbf{.77} & \textbf{.81} & \textbf{.81} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.1} \\
 & F & \textbf{.22} & \textbf{.4} & \textbf{.65} & \textbf{.77} & \textbf{.81} & \textbf{.81} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.1} \\
 & G & \textbf{.22} & \textbf{.4} & \textbf{.65} & \textbf{.77} & \textbf{.81} & \textbf{.81} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.1} \\
 & H & \textbf{.22} & \textbf{.4} & \textbf{.65} & \textbf{.77} & \textbf{.81} & \textbf{.81} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.1} \\
 & I & \textbf{.22} & \textbf{.4} & \textbf{.65} & \textbf{.77} & \textbf{.81} & \textbf{.81} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.1} \\
 & J & \textbf{.22} & \textbf{.4} & \textbf{.65} & \textbf{.77} & \textbf{.81} & \textbf{.81} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.1} \\
 & K & \textbf{.22} & \textbf{.4} & \textbf{.65} & \textbf{.77} & \textbf{.81} & \textbf{.81} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.1} \\
 & L & \textbf{.22} & \textbf{.4} & \textbf{.65} & \textbf{.77} & \textbf{.81} & \textbf{.81} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.1} \\
 & M & \textbf{.22} & \textbf{.4} & \textbf{.65} & \textbf{.77} & \textbf{.81} & \textbf{.81} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.1} \\
 & N & \textbf{.22} & \textbf{.4} & \textbf{.65} & \textbf{.77} & \textbf{.81} & \textbf{.81} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.1} \\
 & O & \textbf{.22} & \textbf{.4} & \textbf{.65} & \textbf{.77} & \textbf{.81} & \textbf{.81} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.1} \\
 & P & \textbf{.22} & \textbf{.4} & \textbf{.65} & \textbf{.77} & \textbf{.81} & \textbf{.81} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.1} \\
 & Q & \textbf{.22} & \textbf{.4} & \textbf{.65} & \textbf{.77} & \textbf{.81} & \textbf{.81} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.1} \\
 & R & \textbf{.22} & \textbf{.4} & \textbf{.65} & \textbf{.77} & \textbf{.81} & \textbf{.81} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1.1} \\
\hline
\multirow{18}{*}{\rotatebox[origin=c]{90}{kitchen}}
 & A & \textbf{.77} & \textbf{.77} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.77} & \textbf{.77} & \textbf{1.2} \\
 & B & \textbf{.77} & \textbf{.77} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.77} & \textbf{.77} & \textbf{1.2} \\
 & C & \textbf{.77} & \textbf{.77} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.77} & \textbf{.77} & \textbf{1.2} \\
 & D & \textbf{.77} & \textbf{.77} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.77} & \textbf{.77} & \textbf{1.2} \\
 & E & \textbf{.77} & \textbf{.77} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.77} & \textbf{.77} & \textbf{1.2} \\
 & F & \textbf{.77} & \textbf{.77} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.77} & \textbf{.77} & \textbf{1.2} \\
 & G & \textbf{.77} & \textbf{.77} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.77} & \textbf{.77} & \textbf{1.2} \\
 & H & \textbf{.77} & \textbf{.77} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.77} & \textbf{.77} & \textbf{1.2} \\
 & I & \textbf{.77} & \textbf{.77} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.77} & \textbf{.77} & \textbf{1.2} \\
 & J & \textbf{.77} & \textbf{.77} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.77} & \textbf{.77} & \textbf{1.2} \\
 & K & \textbf{.77} & \textbf{.77} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.77} & \textbf{.77} & \textbf{1.2} \\
 & L & \textbf{.77} & \textbf{.77} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.77} & \textbf{.77} & \textbf{1.2} \\
 & M & \textbf{.77} & \textbf{.77} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.77} & \textbf{.77} & \textbf{1.2} \\
 & N & \textbf{.77} & \textbf{.77} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.77} & \textbf{.77} & \textbf{1.2} \\
 & O & \textbf{.77} & \textbf{.77} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.77} & \textbf{.77} & \textbf{1.2} \\
 & P & \textbf{.77} & \textbf{.77} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.77} & \textbf{.77} & \textbf{1.2} \\
 & Q & \textbf{.77} & \textbf{.77} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.77} & \textbf{.77} & \textbf{1.2} \\
 & R & \textbf{.77} & \textbf{.77} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.87} & \textbf{.77} & \textbf{.77} & \textbf{1.2} \\
\hline
\multirow{18}{*}{\rotatebox[origin=c]{90}{logistics}}
 & A & \textbf{.44} & .52 & .61 & .72 & .79 & \textbf{.81} & \textbf{.84} & \textbf{.89} & \textbf{.97} & \textbf{1} & \textbf{1.2} \\
 & B & .42 & .49 & .56 & .66 & .76 & .79 & .82 & \textbf{.89} & \textbf{.97} & \textbf{1} & \textbf{1.2} \\
 & C & .42 & .49 & .57 & .68 & .78 & \textbf{.81} & .82 & \textbf{.89} & \textbf{.97} & \textbf{1} & \textbf{1.2} \\
 & D & .36 & .48 & .57 & .68 & .73 & .79 & .82 & \textbf{.89} & \textbf{.97} & \textbf{1} & \textbf{1.2} \\
 & E & .41 & .51 & .54 & .64 & .74 & .77 & \textbf{.84} & \textbf{.89} & \textbf{.97} & \textbf{1} & \textbf{1.2} \\
 & F & .4 & .51 & .56 & .67 & .76 & .77 & .82 & \textbf{.89} & \textbf{.97} & \textbf{1} & \textbf{1.2} \\
 & G & .39 & .49 & .54 & .68 & .75 & .79 & \textbf{.84} & \textbf{.89} & \textbf{.97} & \textbf{1} & \textbf{1.2} \\
 & H & .43 & .53 & .6 & .68 & .75 & .79 & .82 & \textbf{.89} & \textbf{.97} & \textbf{1} & \textbf{1.2} \\
 & I & .39 & .44 & .51 & .73 & .78 & .8 & .82 & .88 & \textbf{.97} & \textbf{1} & \textbf{1.2} \\
 & J & \textbf{.44} & .51 & .61 & .73 & .76 & .78 & .81 & \textbf{.89} & \textbf{.97} & \textbf{1} & \textbf{1.2} \\
 & K & .42 & .51 & .56 & .69 & .76 & .76 & .8 & \textbf{.89} & \textbf{.97} & \textbf{1} & \textbf{1.2} \\
 & L & .36 & .43 & .51 & .76 & .79 & \textbf{.81} & .82 & \textbf{.89} & \textbf{.97} & \textbf{1} & \textbf{1.2} \\
 & M & \textbf{.44} & \textbf{.61} & \textbf{.66} & .76 & .79 & .79 & .82 & \textbf{.89} & \textbf{.97} & \textbf{1} & \textbf{1.2} \\
 & N & .42 & .44 & .56 & .76 & .78 & .8 & .82 & \textbf{.89} & \textbf{.97} & \textbf{1} & \textbf{1.2} \\
 & O & \textbf{.44} & .53 & .64 & \textbf{.77} & .79 & .79 & .82 & \textbf{.89} & \textbf{.97} & \textbf{1} & \textbf{1.2} \\
 & P & \textbf{.44} & .51 & .61 & .73 & .78 & .79 & .82 & \textbf{.89} & \textbf{.97} & \textbf{1} & \textbf{1.2} \\
 & Q & .39 & .49 & .61 & .7 & \textbf{.8} & .8 & .82 & \textbf{.89} & \textbf{.97} & \textbf{1} & \textbf{1.2} \\
 & R & \textbf{.44} & .56 & \textbf{.66} & .74 & .79 & .79 & .82 & \textbf{.89} & \textbf{.97} & \textbf{1} & \textbf{1.2} \\
\hline
\multirow{18}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & \textbf{.61} & \textbf{.77} & \textbf{.8} & \textbf{.83} & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & B & \textbf{.61} & \textbf{.77} & \textbf{.8} & \textbf{.83} & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & C & \textbf{.61} & \textbf{.77} & \textbf{.8} & \textbf{.83} & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & D & \textbf{.61} & \textbf{.77} & \textbf{.8} & \textbf{.83} & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & E & \textbf{.61} & \textbf{.77} & \textbf{.8} & \textbf{.83} & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & F & \textbf{.61} & \textbf{.77} & \textbf{.8} & \textbf{.83} & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & G & \textbf{.61} & \textbf{.77} & \textbf{.8} & \textbf{.83} & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & H & \textbf{.61} & \textbf{.77} & \textbf{.8} & \textbf{.83} & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & I & \textbf{.61} & \textbf{.77} & \textbf{.8} & \textbf{.83} & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & J & \textbf{.61} & \textbf{.77} & \textbf{.8} & \textbf{.83} & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & K & \textbf{.61} & \textbf{.77} & \textbf{.8} & \textbf{.83} & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & L & \textbf{.61} & \textbf{.77} & \textbf{.8} & \textbf{.83} & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & M & \textbf{.61} & \textbf{.77} & \textbf{.8} & \textbf{.83} & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & N & \textbf{.61} & \textbf{.77} & \textbf{.8} & \textbf{.83} & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & O & \textbf{.61} & \textbf{.77} & \textbf{.8} & \textbf{.83} & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & P & \textbf{.61} & \textbf{.77} & \textbf{.8} & \textbf{.83} & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & Q & \textbf{.61} & \textbf{.77} & \textbf{.8} & \textbf{.83} & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
 & R & \textbf{.61} & \textbf{.77} & \textbf{.8} & \textbf{.83} & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1.2} \\
\hline
\multirow{18}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & .5 & .54 & \textbf{.79} & .86 & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & B & .5 & .54 & \textbf{.79} & .86 & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & C & \textbf{.54} & .61 & \textbf{.79} & .86 & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & D & .5 & .57 & \textbf{.79} & \textbf{.89} & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & E & .5 & .61 & \textbf{.79} & .86 & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & F & .5 & .68 & \textbf{.79} & .86 & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & G & .5 & \textbf{.71} & \textbf{.79} & .86 & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & H & .46 & .57 & \textbf{.79} & .86 & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & I & .5 & .68 & \textbf{.79} & \textbf{.89} & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & J & .39 & .64 & .75 & .86 & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & K & .46 & .54 & .75 & .86 & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & L & .5 & .64 & \textbf{.79} & .86 & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & M & .39 & .61 & \textbf{.79} & .86 & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & N & .43 & .54 & \textbf{.79} & .86 & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & O & .5 & .68 & \textbf{.79} & .86 & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & P & .5 & .68 & \textbf{.79} & .86 & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & Q & .46 & .64 & \textbf{.79} & .86 & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & R & .5 & .64 & \textbf{.79} & \textbf{.89} & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
\hline
\multirow{18}{*}{\rotatebox[origin=c]{90}{satellite}}
 & A & .5 & .5 & .54 & .67 & .8 & .82 & .86 & \textbf{.96} & \textbf{.96} & \textbf{.96} & \textbf{1} \\
 & B & .52 & .48 & .52 & .7 & .79 & \textbf{.88} & .91 & \textbf{.96} & \textbf{.96} & \textbf{.96} & 1.1 \\
 & C & .49 & .49 & .6 & .73 & .79 & .8 & .88 & .93 & .93 & \textbf{.96} & 1.3 \\
 & D & .5 & .46 & .5 & .75 & \textbf{.82} & \textbf{.88} & \textbf{.93} & \textbf{.96} & \textbf{.96} & \textbf{.96} & \textbf{1} \\
 & E & \textbf{.55} & \textbf{.59} & \textbf{.63} & \textbf{.76} & .8 & .82 & .88 & .93 & .93 & .93 & 1.1 \\
 & F & .46 & .46 & .57 & .7 & .79 & .84 & .88 & .93 & \textbf{.96} & \textbf{.96} & \textbf{1} \\
 & G & .49 & .42 & .52 & .69 & .75 & .8 & .88 & .93 & .93 & \textbf{.96} & 1.3 \\
 & H & .46 & .46 & .54 & .63 & .77 & .86 & .91 & .93 & .93 & \textbf{.96} & \textbf{1} \\
 & I & .46 & .5 & .57 & .67 & .77 & .82 & .86 & .93 & .93 & \textbf{.96} & \textbf{1} \\
 & J & .54 & .5 & .57 & .74 & .77 & .86 & .89 & \textbf{.96} & \textbf{.96} & \textbf{.96} & \textbf{1} \\
 & K & .45 & .38 & .52 & .65 & .75 & .8 & .84 & .93 & .93 & .93 & 1.3 \\
 & L & .46 & .46 & .54 & .64 & .79 & .8 & .86 & .93 & .93 & \textbf{.96} & \textbf{1} \\
 & M & .5 & .43 & .57 & .68 & .73 & .86 & .89 & \textbf{.96} & \textbf{.96} & \textbf{.96} & 1.1 \\
 & N & .52 & .45 & .55 & .68 & .7 & .82 & .88 & .93 & .93 & \textbf{.96} & 1.1 \\
 & O & .46 & .54 & .57 & .7 & .8 & .82 & .84 & .93 & .93 & .93 & 1.1 \\
 & P & .43 & .46 & .54 & .7 & .77 & .82 & .88 & .93 & .93 & .93 & \textbf{1} \\
 & Q & .45 & .45 & .52 & .69 & .79 & .84 & .88 & .93 & .93 & \textbf{.96} & 1.3 \\
 & R & .52 & .55 & \textbf{.63} & .75 & .8 & .86 & .89 & \textbf{.96} & .93 & \textbf{.96} & 1.1 \\
\hline
\multirow{18}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & .07 & \textbf{.25} & .29 & .43 & .54 & \textbf{.54} & .54 & .57 & .64 & .71 & \textbf{1} \\
 & B & .07 & .18 & \textbf{.36} & \textbf{.5} & \textbf{.57} & .5 & .5 & .54 & .61 & .75 & \textbf{1} \\
 & C & .04 & .11 & .29 & .43 & .5 & \textbf{.54} & .54 & \textbf{.61} & .64 & .75 & \textbf{1} \\
 & D & .07 & .14 & .32 & .46 & .54 & .5 & .54 & \textbf{.61} & .64 & .71 & \textbf{1} \\
 & E & .04 & .14 & .25 & .43 & .54 & \textbf{.54} & .54 & .54 & .61 & .75 & \textbf{1} \\
 & F & \textbf{.14} & \textbf{.25} & .32 & .39 & .5 & .46 & .46 & .57 & .61 & .75 & \textbf{1} \\
 & G & .11 & .11 & .29 & .39 & .54 & .5 & .46 & .54 & .61 & .75 & \textbf{1} \\
 & H & .07 & .11 & \textbf{.36} & .43 & .54 & .46 & .54 & .54 & .57 & .75 & \textbf{1} \\
 & I & \textbf{.14} & .18 & \textbf{.36} & .43 & .54 & .5 & .54 & .57 & .64 & .75 & \textbf{1} \\
 & J & .11 & .18 & .29 & .39 & .54 & .46 & .54 & .5 & .64 & .75 & \textbf{1} \\
 & K & .07 & .11 & .32 & \textbf{.5} & \textbf{.57} & .5 & .46 & .57 & .61 & .75 & \textbf{1} \\
 & L & .07 & .11 & .29 & .39 & .5 & .5 & \textbf{.57} & .54 & \textbf{.68} & .75 & \textbf{1} \\
 & M & .11 & .11 & .29 & .43 & .5 & .46 & .46 & .57 & .61 & .79 & \textbf{1} \\
 & N & .04 & .11 & .32 & .43 & .5 & .5 & .46 & .54 & .64 & .75 & \textbf{1} \\
 & O & \textbf{.14} & \textbf{.25} & .32 & .39 & .5 & .5 & .5 & .5 & .64 & .79 & \textbf{1} \\
 & P & .11 & .14 & .32 & .46 & .54 & .46 & .5 & .54 & .64 & \textbf{.82} & \textbf{1} \\
 & Q & .11 & .14 & .21 & .43 & .54 & \textbf{.54} & .5 & .54 & .64 & .75 & \textbf{1} \\
 & R & .07 & .14 & .25 & .43 & .46 & .5 & .5 & \textbf{.61} & .64 & .75 & \textbf{1} \\
\hline
\multirow{18}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & .29 & .39 & .5 & \textbf{.61} & .79 & .93 & .93 & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & B & .32 & .39 & .54 & .57 & .68 & .93 & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & C & .36 & .39 & \textbf{.57} & \textbf{.61} & .68 & .93 & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & D & .39 & .43 & .46 & .54 & .71 & .93 & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & E & .36 & .32 & .5 & .57 & .68 & .93 & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & F & .36 & .36 & .54 & .57 & .64 & .86 & .89 & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & G & \textbf{.43} & .39 & .5 & .54 & .71 & .93 & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & H & .36 & \textbf{.46} & \textbf{.57} & \textbf{.61} & .64 & .86 & .89 & .96 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & I & \textbf{.43} & .39 & \textbf{.57} & .54 & .75 & .93 & .89 & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & J & .36 & .36 & .5 & .5 & .64 & .86 & .89 & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & K & .39 & .39 & .54 & .5 & .64 & .86 & .89 & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & L & .36 & \textbf{.46} & .54 & \textbf{.61} & .75 & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & M & .36 & .39 & .54 & .5 & .71 & .93 & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & N & .39 & \textbf{.46} & .5 & .54 & .79 & .93 & \textbf{.96} & .96 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & O & .32 & .43 & .54 & .54 & .79 & .93 & .89 & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & P & .39 & .36 & .5 & .54 & .68 & .89 & .89 & .96 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & Q & .32 & .43 & .54 & .54 & .75 & \textbf{.96} & \textbf{.96} & .96 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & R & .32 & .43 & \textbf{.57} & .57 & \textbf{.82} & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
\hline
\end{tabular}
}
\end{table}

==> tables/full/04042024.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MS, RG09, LPBased, PLR-rhw, VSAPN-adjusted-new) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{5}{*}{\rotatebox[origin=c]{90}{average}}
 & A & .33 & .41 & .47 & .55 & .62 & .67 & .72 & .76 & .78 & .8 & 2.0\\
 & B & .3 & .41 & .48 & .58 & .64 & .68 & .74 & .77 & .82 & .87 & 2.3\\
 & C & .21 & .32 & .41 & .5 & .57 & .63 & .71 & .73 & .82 & .87 & 2.6\\
 & D & .3 & .35 & .44 & .53 & .61 & .69 & .73 & .78 & .85 & .92 & 1.2\\
 & E & \textbf{.36} & \textbf{.46} & \textbf{.57} & \textbf{.66} & \textbf{.72} & \textbf{.77} & \textbf{.83} & \textbf{.87} & \textbf{.93} & \textbf{.95} & \textbf{1.1} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{blocks-world}}
 & A & .1 & .13 & .14 & .24 & .29 & .36 & .41 & .47 & .54 & .55 & 7.1\\
 & B & .08 & .22 & .23 & .29 & .38 & .42 & .53 & .63 & \textbf{.81} & \textbf{.9} & 4.1\\
 & C & .06 & .13 & .15 & .2 & .33 & .38 & .46 & .52 & .76 & .81 & 5.4\\
 & D & .09 & .09 & .1 & .1 & .09 & .09 & .09 & .07 & .21 & .27 & 2.8\\
 & E & \textbf{.13} & \textbf{.31} & \textbf{.24} & \textbf{.32} & \textbf{.42} & \textbf{.47} & \textbf{.57} & \textbf{.66} & .8 & \textbf{.9} & \textbf{1.5} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{campus}}
 & A & .73 & .73 & .73 & .53 & .57 & .43 & .57 & .63 & .6 & .6 & 1.4\\
 & B & .73 & .8 & .8 & .83 & .83 & .83 & .83 & .8 & .8 & .8 & 1.2\\
 & C & .5 & .87 & .87 & .97 & .97 & .97 & .97 & .97 & .97 & .97 & 1.2\\
 & D & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & E & .67 & .87 & .87 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{depots}}
 & A & \textbf{.21} & .16 & .16 & .22 & .38 & .49 & .48 & .54 & .59 & .59 & 1.8\\
 & B & .16 & \textbf{.29} & .28 & .32 & .45 & .62 & .59 & .6 & .61 & .78 & 2.6\\
 & C & .09 & .16 & .17 & .27 & .34 & .44 & .57 & .69 & .75 & .89 & 2.4\\
 & D & .18 & .14 & .2 & .2 & .23 & .3 & .5 & .64 & .61 & .82 & 1.2\\
 & E & .18 & .18 & \textbf{.32} & \textbf{.39} & \textbf{.64} & \textbf{.77} & \textbf{.88} & \textbf{.93} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & A & \textbf{.29} & \textbf{.37} & \textbf{.5} & .63 & \textbf{.73} & \textbf{.84} & \textbf{.92} & \textbf{.91} & \textbf{.91} & \textbf{.96} & 1.4\\
 & B & .22 & .27 & .35 & .46 & .52 & .6 & .75 & .77 & .81 & .81 & 2.9\\
 & C & .2 & .26 & .37 & .5 & .58 & .68 & .67 & .68 & .76 & .8 & 2.3\\
 & D & .25 & .23 & .39 & .52 & .61 & .75 & .8 & .8 & .82 & .92 & 1.1\\
 & E & .25 & .32 & .43 & \textbf{.64} & .57 & .61 & .79 & .86 & .89 & .89 & \textbf{1.0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{dwr}}
 & A & .13 & .23 & .2 & .34 & .34 & .39 & .43 & .47 & .46 & .55 & 2.0\\
 & B & .25 & .33 & .32 & .26 & .2 & .22 & .3 & .27 & .31 & .41 & 2.7\\
 & C & .19 & .18 & .24 & .29 & .28 & .33 & .51 & .51 & .65 & .81 & 2.0\\
 & D & .23 & .16 & .27 & \textbf{.45} & \textbf{.5} & \textbf{.54} & .52 & \textbf{.63} & \textbf{.79} & \textbf{1.0} & 1.1\\
 & E & \textbf{.32} & \textbf{.46} & \textbf{.5} & .43 & .32 & .46 & \textbf{.61} & .57 & .75 & .89 & \textbf{1.0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & .29 & .32 & .44 & \textbf{.52} & .56 & .63 & .71 & .76 & .83 & .94 & 2.4\\
 & B & \textbf{.32} & \textbf{.34} & .45 & .48 & .57 & .63 & .69 & .78 & .85 & \textbf{1.0} & 3.0\\
 & C & .13 & .24 & .28 & .35 & .39 & .47 & .5 & .57 & .7 & .78 & 3.3\\
 & D & .2 & .22 & .36 & .42 & .42 & .5 & .58 & .59 & .72 & \textbf{1.0} & \textbf{1.0} \\
 & E & .27 & .31 & \textbf{.48} & .51 & \textbf{.68} & \textbf{.69} & \textbf{.72} & \textbf{.79} & \textbf{.89} & .93 & \textbf{1.0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{ferry}}
 & A & .38 & \textbf{.7} & \textbf{.8} & .83 & .89 & .95 & .93 & .96 & .96 & .96 & 1.2\\
 & B & .28 & .58 & .73 & .8 & .89 & .91 & .95 & .96 & .96 & .96 & 1.6\\
 & C & .19 & .34 & .54 & .75 & .85 & .88 & .91 & .91 & .93 & .96 & 2.1\\
 & D & .25 & .38 & .64 & .73 & .84 & .89 & .96 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.1} \\
 & E & \textbf{.41} & .65 & .75 & \textbf{.87} & \textbf{.98} & \textbf{.98} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.2\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{intrusion-detection}}
 & A & \textbf{.26} & \textbf{.45} & .59 & \textbf{.8} & \textbf{.83} & \textbf{.83} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.8\\
 & B & \textbf{.26} & \textbf{.45} & .59 & \textbf{.8} & \textbf{.83} & \textbf{.83} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.8\\
 & C & .18 & .24 & .35 & .38 & .66 & .67 & .72 & .78 & .94 & .96 & 2.9\\
 & D & .16 & .33 & .34 & .62 & .64 & .77 & .81 & .92 & \textbf{1.0} & \textbf{1.0} & \textbf{1.1} \\
 & E & .22 & .4 & \textbf{.65} & .77 & .81 & .81 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.1} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{logistics}}
 & A & .35 & .41 & .47 & .6 & .7 & .73 & .76 & \textbf{.89} & \textbf{.97} & \textbf{1.0} & 1.5\\
 & B & .34 & .47 & .58 & .69 & .72 & .77 & .8 & .82 & .93 & \textbf{1.0} & 1.9\\
 & C & .16 & .35 & .41 & .48 & .5 & .53 & .68 & .68 & .69 & .74 & 3.7\\
 & D & .23 & .39 & .42 & .51 & .58 & .76 & .83 & \textbf{.89} & \textbf{.97} & \textbf{1.0} & \textbf{1.2} \\
 & E & \textbf{.46} & \textbf{.53} & \textbf{.64} & \textbf{.77} & \textbf{.79} & \textbf{.82} & \textbf{.84} & .88 & \textbf{.97} & \textbf{1.0} & \textbf{1.2} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & .41 & .65 & .73 & \textbf{.84} & .88 & .86 & .89 & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.3\\
 & B & .32 & .49 & .59 & .74 & .82 & .87 & .9 & .95 & \textbf{1.0} & \textbf{1.0} & 1.7\\
 & C & .24 & .43 & .58 & .57 & .76 & .8 & .82 & .86 & .95 & .93 & 2.0\\
 & D & .34 & .54 & .64 & .71 & .77 & .86 & .89 & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & E & \textbf{.61} & \textbf{.77} & \textbf{.8} & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.2\\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & .46 & \textbf{.6} & .69 & .89 & .89 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.2\\
 & B & .43 & \textbf{.6} & .74 & \textbf{.91} & \textbf{.92} & .93 & .93 & .96 & .98 & .98 & 1.5\\
 & C & .31 & .48 & .64 & .67 & .7 & .74 & .81 & .84 & .91 & .93 & 2.0\\
 & D & \textbf{.48} & .52 & \textbf{.8} & .82 & .86 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.1\\
 & E & .43 & .54 & .79 & .89 & .89 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{satellite}}
 & A & .35 & .31 & .36 & .43 & .59 & .66 & .74 & .81 & .81 & .81 & 2.4\\
 & B & .35 & .35 & .42 & .54 & .64 & .62 & .67 & .71 & .74 & .77 & 2.7\\
 & C & .26 & .29 & .38 & .52 & .52 & .62 & .72 & .71 & .72 & .75 & 2.9\\
 & D & .34 & .24 & .29 & .6 & \textbf{.77} & \textbf{.8} & .82 & .91 & .95 & \textbf{.96} & 1.4\\
 & E & \textbf{.49} & \textbf{.52} & \textbf{.63} & \textbf{.69} & .75 & \textbf{.8} & \textbf{.88} & \textbf{.93} & \textbf{.96} & \textbf{.96} & \textbf{1.3} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & \textbf{.28} & \textbf{.3} & .16 & .14 & .27 & .3 & .34 & .25 & .29 & .3 & 1.2\\
 & B & .15 & .22 & .32 & .45 & \textbf{.58} & .6 & .61 & \textbf{.68} & .73 & .8 & 2.7\\
 & C & .16 & .25 & \textbf{.36} & \textbf{.5} & .57 & \textbf{.63} & \textbf{.68} & .64 & .83 & .87 & 1.9\\
 & D & .13 & .21 & .25 & .32 & .5 & .57 & .57 & .5 & \textbf{.86} & \textbf{.96} & \textbf{1.0} \\
 & E & .04 & .21 & \textbf{.36} & .43 & .5 & .54 & .57 & .64 & .71 & .79 & \textbf{1.0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & .32 & .36 & \textbf{.57} & .68 & \textbf{.82} & \textbf{.95} & \textbf{.96} & .98 & \textbf{1.0} & \textbf{1.0} & 1.2\\
 & B & .28 & .29 & .38 & .48 & .59 & .73 & .83 & .89 & .93 & .96 & 1.8\\
 & C & .22 & .3 & .42 & .52 & .6 & .65 & .85 & .92 & .95 & \textbf{1.0} & 2.4\\
 & D & .3 & .41 & .45 & .48 & .73 & .82 & .89 & .96 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & E & \textbf{.5} & \textbf{.43} & \textbf{.57} & \textbf{.71} & \textbf{.82} & .93 & .93 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\end{tabular}
}
\end{table}

==> tables/full/04042024_average.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MS, RG09, LPBased, PLR-rhw, VSAPN-adjusted-new) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Precision (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{5}{*}{\rotatebox[origin=c]{90}{average}}
 & MS & .33 & .41 & .47 & .55 & .62 & .67 & .72 & .76 & .78 & .8 & 2.0\\
 & RG09 & .3 & .41 & .48 & .58 & .64 & .68 & .74 & .77 & .82 & .87 & 2.3\\
 & LP & .21 & .32 & .41 & .5 & .57 & .63 & .71 & .73 & .82 & .87 & 2.6\\
 & PLR & .3 & .35 & .44 & .53 & .61 & .69 & .73 & .78 & .85 & .92 & 1.2\\
 & VS(ours) & \textbf{.36} & \textbf{.46} & \textbf{.57} & \textbf{.66} & \textbf{.72} & \textbf{.77} & \textbf{.83} & \textbf{.87} & \textbf{.93} & \textbf{.95} & \textbf{1.1} \\
\hline
\end{tabular}
}
\end{table}

==> tables/grid/04042024.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MS, RG09, LPBased, PLR, VSAPN-adjusted) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Precision (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{5}{*}{\rotatebox[origin=c]{90}{grid-world}}
 & MS & .14 & .17 & .2 & .24 & .31 & .35 & .4 & .49 & .58 & .59 & 5.4\\
 & RG09 & .15 & .16 & .18 & .21 & .27 & .28 & .3 & .38 & .44 & .44 & 2.3\\
 & LP & .1 & .11 & .13 & .16 & .2 & .22 & .25 & .32 & .37 & .37 & 7.6\\
 & PLR & .11 & .11 & .1 & .09 & .15 & .15 & .26 & .39 & .75 & .87 & 10.4\\
 & VS(ours) & \textbf{.2} & \textbf{.24} & \textbf{.29} & \textbf{.36} & \textbf{.48} & \textbf{.53} & \textbf{.63} & \textbf{.77} & \textbf{.9} & \textbf{.94} & \textbf{1.0} \\
\hline
\end{tabular}
}
\end{table}

==> tables/grid_accuracy.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MS, LPBased, PLR, VSAPN) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{4}{*}{\rotatebox[origin=c]{90}{grid-world}}
 & MS & .99 & .99 & .99 & .99 & .99 & .99 & .99 & .99 & .99 & .99 & 5.4\\
 & LPBased & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 7.6\\
 & PLR & \textbf{1.0} & .98 & .94 & .86 & .79 & .78 & .81 & .85 & .92 & \textbf{1.0} & 10.4\\
 & VS & .2 & .29 & .29 & .37 & .44 & .47 & .6 & .78 & .92 & .96 & \textbf{1.0} \\
\hline
\end{tabular}
}
\end{table}

==> tables/grid_precision.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MS, LPBased, PLR, VSAPN) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Precision (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{4}{*}{\rotatebox[origin=c]{90}{grid-world}}
 & MS & .14 & .17 & .2 & .24 & .31 & .35 & .4 & .49 & .58 & .59 & 5.4\\
 & LPBased & .1 & .11 & .13 & .16 & .2 & .22 & .25 & .32 & .37 & .37 & 7.6\\
 & PLR & .11 & .11 & .1 & .09 & .15 & .15 & .26 & .39 & .75 & .87 & 10.4\\
 & VS & \textbf{.2} & \textbf{.29} & \textbf{.29} & \textbf{.37} & \textbf{.44} & \textbf{.47} & \textbf{.6} & \textbf{.78} & \textbf{.92} & \textbf{.96} & \textbf{1.0} \\
\hline
\end{tabular}
}
\end{table}

==> tables/missingObs/evaluationTable_missingObs_10.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (RG09, LP, PLR, standardDeviationPerformance) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{4}{*}{\rotatebox[origin=c]{90}{average}}
 & A & .28 & .28 & .3 & .32 & .38 & .38 & .39 & .41 & .42 & .42 & 1 \\
 & B & .17 & .17 & .18 & .19 & .23 & .24 & .27 & .29 & .3 & .3 & 1 \\
 & C & .3 & .3 & .3 & .31 & .37 & .37 & .4 & .41 & .41 & .41 & \textbf{1} \\
 & D & \textbf{.34$\pm$ .01} & \textbf{.35$\pm$ .01} & \textbf{.36$\pm$ .01} & \textbf{.39$\pm$ .01} & \textbf{.47$\pm$ .01} & \textbf{.48$\pm$ .01} & \textbf{.49$\pm$ .01} & \textbf{.52$\pm$ .01} & \textbf{.52$\pm$ .01} & \textbf{.52$\pm$ .01} & \textbf{1$\pm$ .01} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{blocks-world}}
 & A & .08 & .08 & .08 & .09 & .09 & .11 & .11 & .13 & .13 & .13 & 1 \\
 & B & .05 & .05 & .06 & .06 & .07 & .09 & .09 & .12 & .12 & .12 & 1 \\
 & C & .06 & .06 & .06 & .06 & .07 & .07 & .07 & .07 & .07 & .07 & \textbf{1} \\
 & D & \textbf{.11$\pm$ 0} & \textbf{.09$\pm$ 0} & \textbf{.09$\pm$ 0} & \textbf{.12$\pm$ 0} & \textbf{.11$\pm$ 0} & \textbf{.12$\pm$ 0} & \textbf{.12$\pm$ 0} & \textbf{.15$\pm$ 0} & \textbf{.15$\pm$ 0} & \textbf{.15$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{campus}}
 & A & .8 & .8 & .8 & .8 & .8 & .8 & .8 & .8 & .8 & .8 & 1 \\
 & B & .5 & .5 & .5 & .5 & .5 & .5 & .5 & .5 & .5 & .5 & 1 \\
 & C & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & D & .93$\pm$ 0 & .93$\pm$ 0 & .93$\pm$ 0 & .93$\pm$ 0 & .93$\pm$ 0 & .93$\pm$ 0 & .93$\pm$ 0 & .93$\pm$ 0 & .93$\pm$ 0 & .93$\pm$ 0 & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{depots}}
 & A & \textbf{.15} & .15 & .18 & .23 & .28 & .28 & .28 & .32 & .32 & .32 & 1 \\
 & B & .11 & .11 & .11 & .13 & .11 & .11 & .16 & .19 & .19 & .19 & 1 \\
 & C & .13 & .13 & .13 & .2 & .27 & .27 & .34 & .38 & .38 & .38 & \textbf{1} \\
 & D & \textbf{.15$\pm$ .03} & \textbf{.18$\pm$ .03} & \textbf{.22$\pm$ .03} & \textbf{.29$\pm$ .03} & \textbf{.36$\pm$ .03} & \textbf{.36$\pm$ .03} & \textbf{.39$\pm$ .03} & \textbf{.46$\pm$ .04} & \textbf{.46$\pm$ .04} & \textbf{.46$\pm$ .04} & \textbf{1$\pm$ .04} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & A & .19 & .2 & .2 & .21 & .26 & .26 & .28 & .28 & .28 & .28 & 1 \\
 & B & .15 & .14 & .14 & .15 & .18 & .17 & .2 & .22 & .22 & .22 & 1 \\
 & C & .18 & \textbf{.21} & \textbf{.21} & .25 & .25 & .25 & .29 & .29 & .29 & .29 & \textbf{1} \\
 & D & \textbf{.2$\pm$ .04} & .2$\pm$ .04 & .2$\pm$ .04 & \textbf{.29$\pm$ .04} & \textbf{.29$\pm$ .04} & \textbf{.29$\pm$ .04} & \textbf{.31$\pm$ .04} & \textbf{.31$\pm$ .04} & \textbf{.31$\pm$ .04} & \textbf{.31$\pm$ .04} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{dwr}}
 & A & .15 & .17 & .17 & .19 & .2 & .21 & .22 & .23 & .24 & .24 & 1 \\
 & B & .14 & .14 & .12 & .14 & .17 & .18 & .24 & .23 & .28 & .28 & 1 \\
 & C & .16 & .2 & \textbf{.2} & .16 & .16 & .16 & .2 & .23 & .2 & .2 & \textbf{1} \\
 & D & \textbf{.23$\pm$ .02} & \textbf{.23$\pm$ .02} & \textbf{.2$\pm$ .02} & \textbf{.21$\pm$ .02} & \textbf{.29$\pm$ .03} & \textbf{.29$\pm$ .03} & \textbf{.32$\pm$ .03} & \textbf{.35$\pm$ .03} & \textbf{.32$\pm$ .04} & \textbf{.32$\pm$ .04} & 1$\pm$ .04 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & \textbf{.35} & \textbf{.35} & \textbf{.35} & \textbf{.36} & .44 & .46 & .46 & .48 & .51 & .51 & 1 \\
 & B & .14 & .13 & .14 & .14 & .25 & .27 & .27 & .34 & .34 & .34 & 1 \\
 & C & .3 & .3 & .3 & .31 & .39 & .44 & .46 & .46 & .46 & .46 & \textbf{1} \\
 & D & .33$\pm$ .02 & .33$\pm$ .02 & .33$\pm$ .02 & .33$\pm$ .02 & \textbf{.46$\pm$ .01} & \textbf{.5$\pm$ .01} & \textbf{.5$\pm$ .01} & \textbf{.57$\pm$ .01} & \textbf{.59$\pm$ .01} & \textbf{.59$\pm$ .01} & 1$\pm$ .02 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{ferry}}
 & A & .27 & .27 & .3 & .34 & .35 & .35 & .36 & .39 & .39 & .39 & 1 \\
 & B & .14 & .14 & .15 & .17 & .17 & .17 & .24 & .24 & .24 & .24 & 1 \\
 & C & .38 & .38 & .38 & .32 & .32 & .32 & .48 & .48 & .48 & .48 & \textbf{1} \\
 & D & \textbf{.39$\pm$ 0} & \textbf{.39$\pm$ 0} & \textbf{.39$\pm$ 0} & \textbf{.53$\pm$ 0} & \textbf{.54$\pm$ 0} & \textbf{.54$\pm$ 0} & \textbf{.6$\pm$ 0} & \textbf{.63$\pm$ 0} & \textbf{.63$\pm$ 0} & \textbf{.63$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{intrusion-detection}}
 & A & \textbf{.2} & \textbf{.2} & \textbf{.2} & \textbf{.2} & \textbf{.33} & \textbf{.33} & \textbf{.33} & \textbf{.33} & \textbf{.33} & \textbf{.33} & 1 \\
 & B & .07 & .07 & .07 & .07 & .13 & .13 & .13 & .13 & .13 & .13 & 1 \\
 & C & .19 & .19 & .19 & .19 & .28 & .28 & .28 & .28 & .28 & .28 & \textbf{1} \\
 & D & \textbf{.2$\pm$ 0} & \textbf{.2$\pm$ 0} & \textbf{.2$\pm$ 0} & \textbf{.2$\pm$ 0} & .28$\pm$ 0 & .28$\pm$ 0 & .28$\pm$ 0 & .28$\pm$ 0 & .28$\pm$ 0 & .28$\pm$ 0 & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{kitchen}}
 & A & .58 & .58 & .58 & .58 & .58 & .58 & .58 & .58 & .58 & .58 & \textbf{1} \\
 & B & .33 & .33 & .33 & .33 & .33 & .33 & .33 & .33 & .33 & .33 & 1 \\
 & C & .44 & .44 & .44 & .44 & .44 & .44 & .44 & .44 & .44 & .44 & 1 \\
 & D & \textbf{.67$\pm$ 0} & \textbf{.67$\pm$ 0} & \textbf{.67$\pm$ 0} & \textbf{.67$\pm$ 0} & \textbf{.67$\pm$ 0} & \textbf{.67$\pm$ 0} & \textbf{.67$\pm$ 0} & \textbf{.67$\pm$ 0} & \textbf{.67$\pm$ 0} & \textbf{.67$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{logistics}}
 & A & .22 & .24 & .25 & .29 & .4 & .39 & .4 & .48 & .5 & .5 & 1 \\
 & B & .1 & .11 & .14 & .17 & .23 & .26 & .26 & .38 & .38 & .38 & 1 \\
 & C & .25 & .25 & .27 & .29 & .37 & .37 & .39 & .46 & .46 & .46 & \textbf{1} \\
 & D & \textbf{.27$\pm$ .03} & \textbf{.29$\pm$ .05} & \textbf{.28$\pm$ .04} & \textbf{.3$\pm$ .03} & \textbf{.54$\pm$ .03} & \textbf{.53$\pm$ .03} & \textbf{.53$\pm$ .03} & \textbf{.64$\pm$ .02} & \textbf{.64$\pm$ .02} & \textbf{.64$\pm$ .02} & 1$\pm$ .01 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & .22 & .22 & .24 & .25 & .32 & .32 & .33 & .33 & .41 & .41 & 1 \\
 & B & .17 & .19 & .19 & .21 & .28 & .29 & .34 & .36 & .34 & .34 & 1 \\
 & C & .29 & .29 & .3 & .36 & .46 & .46 & .52 & .52 & .55 & .55 & \textbf{1} \\
 & D & \textbf{.37$\pm$ 0} & \textbf{.44$\pm$ 0} & \textbf{.51$\pm$ 0} & \textbf{.51$\pm$ 0} & \textbf{.64$\pm$ 0} & \textbf{.64$\pm$ 0} & \textbf{.68$\pm$ 0} & \textbf{.68$\pm$ 0} & \textbf{.68$\pm$ 0} & \textbf{.68$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & .32 & .32 & .37 & .4 & .51 & .51 & .51 & .52 & .52 & .52 & 1 \\
 & B & .17 & .21 & .22 & .23 & .28 & .31 & .31 & .3 & .3 & .3 & 1 \\
 & C & .32 & .3 & .29 & .32 & .48 & .5 & .5 & .48 & .48 & .48 & \textbf{1} \\
 & D & \textbf{.37$\pm$ .05} & \textbf{.36$\pm$ .05} & \textbf{.41$\pm$ .05} & \textbf{.45$\pm$ .06} & \textbf{.57$\pm$ .07} & \textbf{.58$\pm$ .06} & \textbf{.58$\pm$ .06} & \textbf{.58$\pm$ .06} & \textbf{.58$\pm$ .06} & \textbf{.58$\pm$ .06} & 1$\pm$ .01 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{satellite}}
 & A & .3 & .3 & .3 & .37 & .44 & .44 & .46 & .46 & .46 & .46 & 1 \\
 & B & .16 & .16 & .16 & .19 & .26 & .26 & .34 & .34 & .34 & .34 & 1 \\
 & C & .28 & .28 & .29 & .37 & .45 & .45 & .43 & .43 & .43 & .43 & \textbf{1} \\
 & D & \textbf{.42$\pm$ .05} & \textbf{.42$\pm$ .05} & \textbf{.41$\pm$ .05} & \textbf{.43$\pm$ .05} & \textbf{.56$\pm$ .06} & \textbf{.56$\pm$ .06} & \textbf{.58$\pm$ .04} & \textbf{.59$\pm$ .04} & \textbf{.59$\pm$ .04} & \textbf{.59$\pm$ .04} & 1$\pm$ .16 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & .16 & .15 & .16 & .17 & .21 & .21 & .21 & .26 & .26 & .26 & 1 \\
 & B & .15 & .15 & .17 & .16 & .24 & .3 & .35 & \textbf{.38} & .4 & .4 & 1 \\
 & C & .14 & .14 & .14 & .13 & .13 & .13 & .16 & .16 & .18 & .18 & \textbf{1} \\
 & D & \textbf{.23$\pm$ .04} & \textbf{.26$\pm$ .04} & \textbf{.29$\pm$ .04} & \textbf{.33$\pm$ .05} & \textbf{.36$\pm$ .04} & \textbf{.37$\pm$ .04} & \textbf{.38$\pm$ .03} & \textbf{.38$\pm$ .03} & \textbf{.41$\pm$ .03} & \textbf{.41$\pm$ .03} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & .24 & .24 & .26 & .26 & \textbf{.48} & \textbf{.48} & \textbf{.51} & \textbf{.51} & \textbf{.51} & \textbf{.51} & 1 \\
 & B & .15 & .15 & .16 & .21 & .27 & .27 & .3 & .34 & .34 & .34 & 1 \\
 & C & \textbf{.32} & \textbf{.32} & \textbf{.32} & \textbf{.32} & .45 & .45 & .48 & .48 & .48 & .48 & \textbf{1} \\
 & D & .28$\pm$ .05 & .28$\pm$ .05 & .27$\pm$ .04 & .3$\pm$ .04 & .47$\pm$ .04 & .47$\pm$ .04 & .48$\pm$ .04 & \textbf{.51$\pm$ .05} & \textbf{.51$\pm$ .05} & \textbf{.51$\pm$ .05} & \textbf{1$\pm$ 0} \\
\hline
\end{tabular}
}
\end{table}

==> tables/missingObs/evaluationTable_missingObs_30.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (RG09, LP, PLR, standardDeviationPerformance) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{4}{*}{\rotatebox[origin=c]{90}{average}}
 & A & .28 & .32 & .36 & .4 & .45 & .48 & .51 & .55 & .59 & .6 & 1 \\
 & B & .18 & .21 & .26 & .3 & .36 & .39 & .43 & .47 & .5 & .51 & 1 \\
 & C & .25 & .28 & .31 & .36 & .39 & .42 & .46 & .5 & .56 & .58 & \textbf{1} \\
 & D & \textbf{.34$\pm$ .01} & \textbf{.4$\pm$ .01} & \textbf{.45$\pm$ .01} & \textbf{.51$\pm$ .01} & \textbf{.55$\pm$ .01} & \textbf{.56$\pm$ .01} & \textbf{.61$\pm$ .01} & \textbf{.65$\pm$ .01} & \textbf{.71$\pm$ .01} & \textbf{.72$\pm$ .01} & 1$\pm$ .01 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{blocks-world}}
 & A & .07 & .08 & .09 & .13 & .17 & .16 & .22 & .25 & .29 & .29 & 1 \\
 & B & .05 & .08 & .1 & .13 & .12 & .14 & .23 & .26 & .33 & .33 & 1 \\
 & C & .08 & .1 & .1 & .11 & .11 & .1 & .12 & .12 & .12 & .13 & \textbf{1} \\
 & D & \textbf{.13$\pm$ 0} & \textbf{.14$\pm$ 0} & \textbf{.15$\pm$ 0} & \textbf{.17$\pm$ 0} & \textbf{.24$\pm$ 0} & \textbf{.23$\pm$ 0} & \textbf{.28$\pm$ 0} & \textbf{.3$\pm$ 0} & \textbf{.36$\pm$ 0} & \textbf{.37$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{campus}}
 & A & .77 & .77 & .77 & .77 & .77 & .77 & .77 & .77 & .77 & .77 & 1 \\
 & B & .5 & .5 & .5 & .5 & .5 & .5 & .5 & .5 & .5 & .5 & 1 \\
 & C & .8 & .8 & .8 & .8 & .8 & .8 & .8 & .8 & .8 & .8 & \textbf{1} \\
 & D & \textbf{.87$\pm$ 0} & \textbf{.87$\pm$ 0} & \textbf{.87$\pm$ 0} & \textbf{.87$\pm$ 0} & \textbf{.87$\pm$ 0} & \textbf{.87$\pm$ 0} & \textbf{.87$\pm$ 0} & \textbf{.87$\pm$ 0} & \textbf{.87$\pm$ 0} & \textbf{.87$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{depots}}
 & A & \textbf{.16} & \textbf{.19} & .22 & .22 & .23 & .3 & .37 & .4 & .46 & .47 & 1 \\
 & B & .13 & .16 & .15 & .19 & .26 & .26 & .33 & .33 & .37 & .41 & 1 \\
 & C & .11 & .11 & .14 & .18 & .14 & .14 & .27 & .32 & .46 & .5 & \textbf{1} \\
 & D & .1$\pm$ .03 & .17$\pm$ .05 & \textbf{.27$\pm$ .05} & \textbf{.44$\pm$ .03} & \textbf{.41$\pm$ .03} & \textbf{.42$\pm$ .03} & \textbf{.5$\pm$ .05} & \textbf{.57$\pm$ .04} & \textbf{.69$\pm$ .04} & \textbf{.73$\pm$ .04} & 1$\pm$ .04 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & A & .2 & .18 & .21 & .23 & .27 & .26 & .27 & .33 & .41 & .41 & 1 \\
 & B & .14 & .14 & .14 & .22 & .29 & .28 & .35 & .42 & .43 & .42 & 1 \\
 & C & .18 & .21 & .25 & .25 & .25 & .25 & .34 & .38 & .43 & .43 & \textbf{1} \\
 & D & \textbf{.29$\pm$ .03} & \textbf{.35$\pm$ .04} & \textbf{.4$\pm$ .05} & \textbf{.38$\pm$ .05} & \textbf{.43$\pm$ .05} & \textbf{.43$\pm$ .05} & \textbf{.47$\pm$ .05} & \textbf{.56$\pm$ .05} & \textbf{.66$\pm$ .05} & \textbf{.66$\pm$ .05} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{dwr}}
 & A & .19 & .2 & .18 & .21 & .24 & .19 & .19 & .23 & .24 & .27 & 1 \\
 & B & .17 & .2 & .16 & .14 & .19 & .19 & .21 & .27 & .39 & .46 & 1 \\
 & C & .25 & .21 & .2 & .16 & .21 & .25 & \textbf{.29} & .3 & .41 & .45 & \textbf{1} \\
 & D & \textbf{.27$\pm$ .03} & \textbf{.31$\pm$ .03} & \textbf{.24$\pm$ .04} & \textbf{.29$\pm$ .04} & \textbf{.25$\pm$ .04} & \textbf{.28$\pm$ .04} & .26$\pm$ .03 & \textbf{.42$\pm$ .05} & \textbf{.51$\pm$ .03} & \textbf{.52$\pm$ .03} & 1$\pm$ .03 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & .29 & .31 & .35 & .38 & \textbf{.42} & .44 & .51 & .58 & .64 & .67 & 1 \\
 & B & .14 & .14 & .2 & .27 & .36 & .39 & .41 & .46 & .51 & .54 & 1 \\
 & C & .18 & .16 & .16 & .24 & .3 & .32 & .43 & .55 & .61 & .69 & \textbf{1} \\
 & D & \textbf{.3$\pm$ .01} & \textbf{.32$\pm$ .02} & \textbf{.37$\pm$ .02} & \textbf{.41$\pm$ .02} & \textbf{.42$\pm$ .01} & \textbf{.46$\pm$ .01} & \textbf{.56$\pm$ .02} & \textbf{.59$\pm$ .01} & \textbf{.66$\pm$ .01} & \textbf{.7$\pm$ 0} & 1$\pm$ .01 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{ferry}}
 & A & .26 & .32 & .43 & .51 & .58 & .67 & .67 & .75 & .81 & .81 & 1 \\
 & B & .14 & .17 & .25 & .31 & .42 & .51 & .53 & .52 & .6 & .6 & 1 \\
 & C & .2 & .25 & .32 & .52 & .58 & .64 & .64 & .71 & .82 & .82 & \textbf{1} \\
 & D & \textbf{.37$\pm$ 0} & \textbf{.48$\pm$ 0} & \textbf{.57$\pm$ 0} & \textbf{.64$\pm$ 0} & \textbf{.69$\pm$ 0} & \textbf{.8$\pm$ 0} & \textbf{.83$\pm$ 0} & \textbf{.89$\pm$ 0} & \textbf{.91$\pm$ 0} & \textbf{.91$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{intrusion-detection}}
 & A & .18 & .22 & .29 & .38 & .44 & .51 & .51 & \textbf{.57} & \textbf{.57} & \textbf{.57} & 1 \\
 & B & .07 & .1 & .14 & .16 & .19 & .27 & .29 & .45 & .45 & .45 & 1 \\
 & C & \textbf{.24} & .26 & .31 & .39 & .37 & .42 & .45 & .51 & .51 & .51 & \textbf{1} \\
 & D & .22$\pm$ 0 & \textbf{.27$\pm$ 0} & \textbf{.34$\pm$ 0} & \textbf{.45$\pm$ 0} & \textbf{.47$\pm$ 0} & \textbf{.56$\pm$ 0} & \textbf{.56$\pm$ 0} & \textbf{.57$\pm$ 0} & \textbf{.57$\pm$ 0} & \textbf{.57$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{kitchen}}
 & A & .53 & .53 & .53 & .53 & .61 & .61 & .61 & .61 & .61 & .61 & \textbf{1} \\
 & B & .27 & .27 & .44 & .44 & .46 & .46 & .46 & .46 & .46 & .46 & 1 \\
 & C & .27 & .27 & .31 & .31 & .4 & .4 & .4 & .44 & .44 & .44 & 1 \\
 & D & \textbf{.63$\pm$ 0} & \textbf{.63$\pm$ 0} & \textbf{.63$\pm$ 0} & \textbf{.63$\pm$ 0} & \textbf{.67$\pm$ 0} & \textbf{.67$\pm$ 0} & \textbf{.67$\pm$ 0} & \textbf{.67$\pm$ 0} & \textbf{.67$\pm$ 0} & \textbf{.67$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{logistics}}
 & A & .21 & .31 & .36 & .45 & .5 & \textbf{.54} & .63 & .64 & .7 & .68 & 1 \\
 & B & .14 & .19 & .25 & .29 & .37 & .39 & .47 & .5 & .49 & .53 & 1 \\
 & C & .16 & .23 & .25 & .31 & .39 & .41 & .46 & .51 & .6 & .63 & \textbf{1} \\
 & D & \textbf{.23$\pm$ .03} & \textbf{.33$\pm$ .03} & \textbf{.39$\pm$ .03} & \textbf{.46$\pm$ .03} & \textbf{.53$\pm$ .02} & \textbf{.54$\pm$ .03} & \textbf{.64$\pm$ .02} & \textbf{.68$\pm$ .01} & \textbf{.72$\pm$ 0} & \textbf{.72$\pm$ 0} & 1$\pm$ .01 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & .28 & .36 & .37 & .48 & .51 & .61 & .63 & .65 & .77 & .79 & 1 \\
 & B & .2 & .36 & .34 & .4 & .49 & .57 & .55 & .64 & .66 & .66 & 1 \\
 & C & .21 & .43 & .46 & .43 & .36 & .43 & .57 & .55 & .64 & .68 & \textbf{1} \\
 & D & \textbf{.45$\pm$ 0} & \textbf{.6$\pm$ 0} & \textbf{.68$\pm$ 0} & \textbf{.8$\pm$ 0} & \textbf{.83$\pm$ 0} & \textbf{.83$\pm$ 0} & \textbf{.93$\pm$ 0} & \textbf{.98$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & .36 & .47 & .6 & .7 & .72 & .73 & .76 & .82 & .82 & .82 & 1 \\
 & B & .2 & .24 & .38 & .39 & .37 & .46 & .54 & .61 & .63 & .59 & 1 \\
 & C & .33 & .46 & .48 & .57 & .68 & .68 & .71 & .75 & .75 & .79 & \textbf{1} \\
 & D & \textbf{.44$\pm$ .05} & \textbf{.54$\pm$ .04} & \textbf{.68$\pm$ .04} & \textbf{.74$\pm$ .04} & \textbf{.78$\pm$ .03} & \textbf{.78$\pm$ .03} & \textbf{.83$\pm$ .03} & \textbf{.92$\pm$ .03} & \textbf{.92$\pm$ .03} & \textbf{.92$\pm$ .03} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{satellite}}
 & A & .32 & .34 & .34 & .4 & .45 & .47 & .53 & .6 & .66 & .66 & 1 \\
 & B & .16 & .21 & .24 & .3 & .46 & .47 & .57 & .63 & .63 & .63 & 1 \\
 & C & .3 & .29 & .32 & .42 & .57 & .57 & .53 & .56 & .63 & .63 & \textbf{1} \\
 & D & \textbf{.39$\pm$ .05} & \textbf{.44$\pm$ .03} & \textbf{.51$\pm$ .04} & \textbf{.59$\pm$ .04} & \textbf{.66$\pm$ .03} & \textbf{.66$\pm$ .03} & \textbf{.68$\pm$ .04} & \textbf{.75$\pm$ .04} & \textbf{.78$\pm$ .03} & \textbf{.78$\pm$ .03} & 1$\pm$ .11 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & .17 & .2 & .25 & .31 & .4 & .42 & .49 & .57 & .61 & .62 & 1 \\
 & B & .18 & \textbf{.25} & .27 & .34 & .47 & \textbf{.54} & .51 & \textbf{.59} & .63 & .65 & 1 \\
 & C & .13 & .11 & .16 & .2 & .27 & .34 & .38 & .41 & .5 & .54 & \textbf{1} \\
 & D & \textbf{.19$\pm$ .04} & \textbf{.25$\pm$ .04} & \textbf{.34$\pm$ .04} & \textbf{.35$\pm$ .03} & \textbf{.49$\pm$ .03} & .48$\pm$ .04 & \textbf{.55$\pm$ .03} & .56$\pm$ .05 & \textbf{.67$\pm$ .03} & \textbf{.71$\pm$ .04} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & .25 & .29 & \textbf{.36} & .36 & .4 & .46 & .47 & .49 & .52 & .5 & 1 \\
 & B & .19 & .21 & .33 & .4 & .39 & .43 & .45 & .45 & .46 & .46 & 1 \\
 & C & \textbf{.29} & .32 & .34 & \textbf{.5} & \textbf{.46} & \textbf{.54} & \textbf{.54} & \textbf{.54} & \textbf{.68} & \textbf{.68} & \textbf{1} \\
 & D & .27$\pm$ .03 & \textbf{.37$\pm$ .03} & .34$\pm$ .03 & .41$\pm$ .04 & .45$\pm$ .05 & .46$\pm$ .05 & .49$\pm$ .04 & .49$\pm$ .03 & .61$\pm$ .02 & .61$\pm$ .02 & \textbf{1$\pm$ 0} \\
\hline
\end{tabular}
}
\end{table}

==> tables/missingObs/evaluationTable_missingObs_50.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (RG09, LP, PLR, standardDeviationPerformance) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{4}{*}{\rotatebox[origin=c]{90}{average}}
 & A & .28 & .35 & .4 & .44 & .5 & .53 & .55 & .6 & .65 & .68 & 1 \\
 & B & .2 & .27 & .35 & .4 & .49 & .52 & .58 & .62 & .67 & .71 & 1 \\
 & C & .24 & .31 & .35 & .4 & .46 & .49 & .53 & .57 & .63 & .66 & \textbf{1} \\
 & D & \textbf{.34$\pm$ .01} & \textbf{.43$\pm$ 0} & \textbf{.47$\pm$ .01} & \textbf{.52$\pm$ .01} & \textbf{.58$\pm$ 0} & \textbf{.62$\pm$ .01} & \textbf{.64$\pm$ 0} & \textbf{.69$\pm$ 0} & \textbf{.74$\pm$ 0} & \textbf{.77$\pm$ 0} & 1$\pm$ .01 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{blocks-world}}
 & A & .08 & .1 & .11 & .13 & .17 & .22 & .29 & \textbf{.38} & \textbf{.44} & \textbf{.54} & 1 \\
 & B & .06 & .08 & .11 & .12 & .15 & .19 & .26 & .3 & .42 & .51 & 1 \\
 & C & .11 & .1 & .1 & .09 & .09 & .09 & .1 & .12 & .11 & .14 & \textbf{1} \\
 & D & \textbf{.12$\pm$ 0} & \textbf{.19$\pm$ 0} & \textbf{.21$\pm$ 0} & \textbf{.22$\pm$ 0} & \textbf{.23$\pm$ 0} & \textbf{.33$\pm$ 0} & \textbf{.32$\pm$ 0} & .36$\pm$ 0 & .4$\pm$ 0 & .5$\pm$ 0 & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{campus}}
 & A & .7 & .7 & .7 & .7 & .7 & .7 & .7 & .7 & .7 & .7 & 1 \\
 & B & .5 & .5 & .57 & .72 & .85 & .85 & .92 & .92 & .92 & .92 & 1 \\
 & C & \textbf{.93} & \textbf{.93} & \textbf{.93} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & D & .73$\pm$ 0 & .73$\pm$ 0 & .73$\pm$ 0 & .77$\pm$ 0 & .87$\pm$ 0 & .87$\pm$ 0 & .9$\pm$ 0 & .9$\pm$ 0 & .9$\pm$ 0 & .9$\pm$ 0 & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{depots}}
 & A & .16 & .16 & .18 & .21 & .25 & .27 & .29 & .38 & .45 & .54 & 1 \\
 & B & .11 & .12 & .12 & .16 & .26 & .31 & .4 & .51 & .66 & .71 & 1 \\
 & C & .09 & .09 & .13 & .16 & .27 & .29 & .28 & .43 & .5 & .57 & \textbf{1} \\
 & D & \textbf{.17$\pm$ .03} & \textbf{.21$\pm$ .02} & \textbf{.2$\pm$ .02} & \textbf{.29$\pm$ .02} & \textbf{.4$\pm$ .03} & \textbf{.51$\pm$ .03} & \textbf{.61$\pm$ .03} & \textbf{.72$\pm$ .02} & \textbf{.81$\pm$ .02} & \textbf{.86$\pm$ .02} & 1$\pm$ .02 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & A & .18 & .21 & .23 & .27 & .34 & .4 & .45 & .53 & .6 & .62 & 1 \\
 & B & .16 & .23 & .27 & .36 & .49 & .52 & .61 & .61 & .68 & .69 & 1 \\
 & C & .2 & .3 & \textbf{.36} & .36 & \textbf{.54} & \textbf{.59} & \textbf{.63} & .57 & .64 & .64 & \textbf{1} \\
 & D & \textbf{.21$\pm$ .02} & \textbf{.31$\pm$ .04} & .35$\pm$ .03 & \textbf{.37$\pm$ .04} & .47$\pm$ .04 & .46$\pm$ .04 & .53$\pm$ .04 & \textbf{.66$\pm$ .03} & \textbf{.7$\pm$ .02} & \textbf{.79$\pm$ .01} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{dwr}}
 & A & .2 & .22 & .26 & .28 & .27 & .25 & .2 & .23 & .27 & .28 & 1 \\
 & B & .16 & .21 & .27 & .29 & .28 & .3 & \textbf{.42} & \textbf{.51} & \textbf{.54} & \textbf{.68} & 1 \\
 & C & .21 & .21 & .23 & .27 & \textbf{.3} & \textbf{.32} & .29 & .32 & .43 & .5 & \textbf{1} \\
 & D & \textbf{.23$\pm$ .03} & \textbf{.32$\pm$ .03} & \textbf{.29$\pm$ .02} & \textbf{.3$\pm$ .03} & .26$\pm$ .03 & .31$\pm$ .03 & .33$\pm$ .03 & .39$\pm$ .02 & .46$\pm$ .02 & .57$\pm$ .02 & 1$\pm$ .01 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & \textbf{.21} & \textbf{.32} & \textbf{.37} & .38 & .45 & .49 & .54 & \textbf{.61} & \textbf{.71} & \textbf{.76} & 1 \\
 & B & .14 & .19 & .25 & .31 & .38 & .42 & .45 & .52 & .58 & .64 & 1 \\
 & C & .16 & .24 & .24 & .26 & .33 & .35 & .41 & .47 & .67 & \textbf{.76} & \textbf{1} \\
 & D & .2$\pm$ .01 & .3$\pm$ .01 & .36$\pm$ .01 & \textbf{.42$\pm$ .01} & \textbf{.51$\pm$ .01} & \textbf{.56$\pm$ .01} & \textbf{.6$\pm$ .01} & \textbf{.61$\pm$ .01} & .69$\pm$ .01 & .69$\pm$ .01 & 1$\pm$ .01 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{ferry}}
 & A & .24 & .35 & .48 & .55 & .73 & .73 & .77 & .79 & .85 & .85 & 1 \\
 & B & .16 & .32 & .41 & .47 & .65 & .68 & .75 & .77 & .83 & .84 & 1 \\
 & C & .29 & .29 & .45 & .64 & .66 & .68 & .77 & .79 & .82 & .86 & \textbf{1} \\
 & D & \textbf{.32$\pm$ 0} & \textbf{.45$\pm$ .01} & \textbf{.6$\pm$ 0} & \textbf{.68$\pm$ 0} & \textbf{.85$\pm$ 0} & \textbf{.85$\pm$ 0} & \textbf{.85$\pm$ 0} & \textbf{.86$\pm$ 0} & \textbf{.92$\pm$ 0} & \textbf{.92$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{intrusion-detection}}
 & A & \textbf{.18} & \textbf{.31} & \textbf{.34} & \textbf{.36} & .44 & .46 & .48 & .52 & .54 & .54 & 1 \\
 & B & .09 & .16 & .21 & .25 & .28 & .32 & .38 & .42 & .45 & .45 & 1 \\
 & C & .04 & .2 & .29 & .26 & .33 & .39 & .38 & .43 & .51 & .51 & \textbf{1} \\
 & D & \textbf{.18$\pm$ 0} & .28$\pm$ 0 & .31$\pm$ 0 & .34$\pm$ 0 & \textbf{.46$\pm$ 0} & \textbf{.5$\pm$ 0} & \textbf{.51$\pm$ 0} & \textbf{.54$\pm$ 0} & \textbf{.55$\pm$ 0} & \textbf{.55$\pm$ 0} & \textbf{1$\pm$ 0} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{kitchen}}
 & A & .54 & .68 & .68 & \textbf{.63} & .68 & .68 & \textbf{.64} & \textbf{.64} & \textbf{.64} & \textbf{.64} & \textbf{1} \\
 & B & .42 & .51 & .52 & .54 & .63 & .63 & \textbf{.64} & .59 & .59 & .59 & 1 \\
 & C & .24 & .24 & .29 & .27 & .29 & .38 & .4 & .4 & .4 & .4 & 1 \\
 & D & \textbf{.73$\pm$ 0} & \textbf{.73$\pm$ 0} & \textbf{.73$\pm$ 0} & .62$\pm$ 0 & \textbf{.69$\pm$ 0} & \textbf{.69$\pm$ 0} & .63$\pm$ 0 & .63$\pm$ 0 & .63$\pm$ 0 & .63$\pm$ 0 & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{logistics}}
 & A & .25 & .36 & \textbf{.43} & .52 & .61 & .65 & .69 & .7 & .77 & .77 & 1 \\
 & B & .15 & .28 & .38 & .43 & .47 & .52 & .59 & .63 & .69 & .7 & 1 \\
 & C & .18 & .22 & .19 & .31 & .39 & .54 & .62 & .72 & .77 & \textbf{.8} & \textbf{1} \\
 & D & \textbf{.3$\pm$ .03} & \textbf{.41$\pm$ .03} & .42$\pm$ .02 & \textbf{.57$\pm$ .02} & \textbf{.64$\pm$ .02} & \textbf{.67$\pm$ .02} & \textbf{.71$\pm$ .01} & \textbf{.76$\pm$ .01} & \textbf{.8$\pm$ .01} & \textbf{.8$\pm$ .01} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & .29 & .36 & .43 & .54 & .62 & .66 & .71 & .79 & .88 & .88 & 1 \\
 & B & .24 & .35 & .52 & .58 & .64 & .66 & .74 & .78 & .79 & .81 & 1 \\
 & C & .3 & .59 & .5 & .54 & .57 & .57 & .71 & .79 & .91 & .95 & \textbf{1} \\
 & D & \textbf{.49$\pm$ 0} & \textbf{.68$\pm$ 0} & \textbf{.73$\pm$ 0} & \textbf{.85$\pm$ 0} & \textbf{.87$\pm$ 0} & \textbf{.9$\pm$ 0} & \textbf{.91$\pm$ 0} & \textbf{.93$\pm$ 0} & \textbf{.98$\pm$ 0} & \textbf{.98$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & .4 & .49 & .61 & .65 & \textbf{.75} & \textbf{.78} & .8 & .85 & .89 & .89 & 1 \\
 & B & .26 & .35 & .46 & .54 & .66 & .66 & .71 & .72 & .8 & .81 & 1 \\
 & C & .39 & .43 & .63 & .66 & .71 & .71 & .75 & .82 & .86 & .86 & \textbf{1} \\
 & D & \textbf{.42$\pm$ .03} & \textbf{.59$\pm$ .04} & \textbf{.75$\pm$ .02} & \textbf{.75$\pm$ .02} & \textbf{.75$\pm$ .02} & \textbf{.78$\pm$ .02} & \textbf{.82$\pm$ .01} & \textbf{.93$\pm$ 0} & \textbf{.93$\pm$ 0} & \textbf{.93$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{satellite}}
 & A & .34 & .37 & .38 & .5 & .52 & .57 & .6 & .66 & .73 & .73 & 1 \\
 & B & .2 & .24 & .34 & .43 & .52 & .6 & .67 & .68 & .74 & .75 & 1 \\
 & C & .25 & .27 & .33 & .47 & .53 & .51 & .53 & .58 & .66 & .66 & \textbf{1} \\
 & D & \textbf{.46$\pm$ .03} & \textbf{.5$\pm$ .03} & \textbf{.56$\pm$ .04} & \textbf{.66$\pm$ .03} & \textbf{.68$\pm$ .03} & \textbf{.71$\pm$ .03} & \textbf{.71$\pm$ .03} & \textbf{.8$\pm$ .02} & \textbf{.83$\pm$ .03} & \textbf{.83$\pm$ .03} & 1$\pm$ .1 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & \textbf{.17} & .2 & .36 & \textbf{.42} & .47 & .47 & .46 & .5 & .62 & .7 & 1 \\
 & B & .15 & \textbf{.27} & \textbf{.41} & .4 & \textbf{.53} & \textbf{.53} & \textbf{.57} & \textbf{.59} & \textbf{.64} & \textbf{.71} & 1 \\
 & C & .07 & .14 & .14 & .2 & .25 & .29 & .39 & .32 & .36 & .5 & \textbf{1} \\
 & D & .1$\pm$ .03 & .25$\pm$ .03 & .33$\pm$ .01 & .4$\pm$ .02 & .42$\pm$ .03 & .42$\pm$ .03 & .44$\pm$ .03 & .49$\pm$ .02 & .57$\pm$ .02 & .61$\pm$ .03 & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & .21 & .36 & .41 & .45 & .53 & .57 & .63 & .66 & .73 & .77 & 1 \\
 & B & .16 & .28 & .34 & .39 & .49 & .54 & .61 & .68 & .79 & .82 & 1 \\
 & C & .21 & \textbf{.46} & \textbf{.5} & \textbf{.54} & .57 & \textbf{.68} & .71 & .75 & .82 & .82 & \textbf{1} \\
 & D & \textbf{.35$\pm$ .05} & \textbf{.46$\pm$ .03} & .45$\pm$ .03 & .52$\pm$ .02 & \textbf{.6$\pm$ .03} & \textbf{.68$\pm$ .03} & \textbf{.79$\pm$ .02} & \textbf{.83$\pm$ .02} & \textbf{.93$\pm$ .02} & \textbf{.93$\pm$ .02} & \textbf{1$\pm$ 0} \\
\hline
\end{tabular}
}
\end{table}

==> tables/missingObs/evaluationTable_missingObs_70.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (RG09, LP, PLR, standardDeviationPerformance) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{4}{*}{\rotatebox[origin=c]{90}{average}}
 & A & .3 & .37 & .45 & .51 & .58 & .62 & .64 & .68 & .71 & .75 & 1 \\
 & B & .21 & .28 & .37 & .43 & .53 & .55 & .63 & .66 & .73 & .77 & 1 \\
 & C & .28 & .33 & .41 & .44 & .51 & .58 & .63 & .66 & .72 & .78 & \textbf{1} \\
 & D & \textbf{.36$\pm$ .01} & \textbf{.45$\pm$ .01} & \textbf{.51$\pm$ .01} & \textbf{.59$\pm$ .01} & \textbf{.65$\pm$ .01} & \textbf{.69$\pm$ .01} & \textbf{.73$\pm$ .01} & \textbf{.76$\pm$ 0} & \textbf{.81$\pm$ .01} & \textbf{.83$\pm$ 0} & 1$\pm$ .01 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{blocks-world}}
 & A & .05 & .1 & .09 & .11 & .15 & .19 & .26 & .3 & \textbf{.45} & .51 & 1 \\
 & B & .06 & .08 & .09 & .1 & .14 & .19 & .25 & .28 & \textbf{.45} & \textbf{.53} & 1 \\
 & C & .08 & .08 & .08 & .07 & .07 & .08 & .11 & .12 & .14 & .18 & \textbf{1} \\
 & D & \textbf{.09$\pm$ 0} & \textbf{.15$\pm$ 0} & \textbf{.11$\pm$ 0} & \textbf{.14$\pm$ 0} & \textbf{.18$\pm$ 0} & \textbf{.22$\pm$ 0} & \textbf{.29$\pm$ 0} & \textbf{.32$\pm$ 0} & \textbf{.45$\pm$ 0} & .52$\pm$ 0 & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{campus}}
 & A & .77 & .77 & .77 & .8 & .8 & .8 & .8 & .8 & .8 & .8 & 1 \\
 & B & .5 & .5 & .63 & .8 & .87 & .87 & .93 & .93 & .93 & .93 & 1 \\
 & C & \textbf{1} & \textbf{1} & \textbf{.93} & \textbf{.93} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & D & .73$\pm$ 0 & .73$\pm$ 0 & .67$\pm$ 0 & .9$\pm$ 0 & .97$\pm$ 0 & .97$\pm$ 0 & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{depots}}
 & A & \textbf{.16} & \textbf{.22} & \textbf{.27} & .29 & .41 & .53 & .55 & .61 & .58 & .73 & 1 \\
 & B & .11 & .09 & .1 & .18 & .29 & .35 & .42 & .54 & .76 & .75 & 1 \\
 & C & .09 & .14 & .18 & .25 & .21 & .21 & .43 & .53 & .58 & .76 & \textbf{1} \\
 & D & .15$\pm$ .02 & .2$\pm$ .03 & .2$\pm$ .04 & \textbf{.31$\pm$ .04} & \textbf{.5$\pm$ .03} & \textbf{.66$\pm$ .04} & \textbf{.73$\pm$ .04} & \textbf{.85$\pm$ .03} & \textbf{.95$\pm$ .02} & \textbf{.96$\pm$ 0} & 1$\pm$ .02 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & A & .19 & .24 & .33 & .42 & .46 & .51 & .58 & .66 & .64 & .64 & 1 \\
 & B & .16 & .22 & .31 & .42 & .55 & .55 & .66 & .64 & .69 & .74 & 1 \\
 & C & .32 & \textbf{.43} & \textbf{.5} & .5 & \textbf{.66} & \textbf{.75} & .71 & .71 & .76 & .79 & \textbf{1} \\
 & D & \textbf{.34$\pm$ .05} & .42$\pm$ .05 & \textbf{.5$\pm$ .04} & \textbf{.54$\pm$ .05} & .57$\pm$ .05 & .66$\pm$ .04 & \textbf{.79$\pm$ .04} & \textbf{.77$\pm$ .04} & \textbf{.81$\pm$ .04} & \textbf{.85$\pm$ .04} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{dwr}}
 & A & .23 & .27 & .3 & .33 & .3 & .34 & .25 & .32 & .33 & .39 & 1 \\
 & B & .18 & .28 & .29 & .32 & .32 & .35 & \textbf{.49} & \textbf{.6} & .62 & .76 & 1 \\
 & C & .2 & .13 & .2 & .27 & .3 & .36 & .43 & .52 & .66 & \textbf{.8} & \textbf{1} \\
 & D & \textbf{.28$\pm$ .04} & \textbf{.4$\pm$ .05} & \textbf{.44$\pm$ .03} & \textbf{.4$\pm$ .04} & \textbf{.39$\pm$ .04} & \textbf{.39$\pm$ .05} & \textbf{.49$\pm$ .04} & .56$\pm$ .04 & \textbf{.74$\pm$ .02} & .77$\pm$ .03 & 1$\pm$ .01 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & .26 & .32 & \textbf{.37} & .39 & .45 & .51 & .51 & .51 & .65 & .74 & 1 \\
 & B & .15 & .21 & .28 & .32 & .39 & .4 & .46 & .53 & .6 & .67 & 1 \\
 & C & .2 & .23 & .33 & .34 & .4 & .44 & .45 & .45 & .6 & \textbf{.77} & \textbf{1} \\
 & D & \textbf{.27$\pm$ .02} & \textbf{.35$\pm$ .02} & \textbf{.37$\pm$ .02} & \textbf{.44$\pm$ .02} & \textbf{.5$\pm$ .03} & \textbf{.54$\pm$ .02} & \textbf{.54$\pm$ .01} & \textbf{.64$\pm$ .02} & \textbf{.69$\pm$ .01} & .71$\pm$ .01 & 1$\pm$ .01 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{ferry}}
 & A & .28 & .5 & .6 & .71 & .84 & .84 & .91 & .92 & .9 & .92 & 1 \\
 & B & .17 & .35 & .43 & .51 & .74 & .75 & .86 & .89 & .91 & .93 & 1 \\
 & C & .32 & .3 & .6 & .68 & .82 & .83 & .93 & .96 & .96 & .96 & \textbf{1} \\
 & D & \textbf{.41$\pm$ 0} & \textbf{.62$\pm$ .01} & \textbf{.78$\pm$ .02} & \textbf{.87$\pm$ 0} & \textbf{.95$\pm$ 0} & \textbf{.95$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{intrusion-detection}}
 & A & \textbf{.18} & \textbf{.26} & \textbf{.32} & \textbf{.39} & \textbf{.43} & \textbf{.5} & \textbf{.53} & \textbf{.55} & \textbf{.55} & \textbf{.55} & 1 \\
 & B & .11 & .17 & .25 & .31 & .3 & .33 & .36 & .47 & .53 & .53 & 1 \\
 & C & .17 & .22 & .22 & .12 & .27 & .36 & .4 & .43 & .54 & .54 & \textbf{1} \\
 & D & .14$\pm$ 0 & .23$\pm$ 0 & .25$\pm$ 0 & .35$\pm$ 0 & .38$\pm$ 0 & .49$\pm$ 0 & .52$\pm$ 0 & \textbf{.55$\pm$ 0} & \textbf{.55$\pm$ 0} & \textbf{.55$\pm$ 0} & \textbf{1$\pm$ 0} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{kitchen}}
 & A & .63 & .68 & .76 & .72 & .77 & .77 & .77 & \textbf{.76} & \textbf{.76} & \textbf{.76} & \textbf{1} \\
 & B & .51 & .51 & .53 & .54 & .71 & .71 & .74 & .66 & .66 & .66 & 1 \\
 & C & .31 & .31 & .33 & .33 & .42 & .47 & .47 & .47 & .47 & .47 & 1 \\
 & D & \textbf{.83$\pm$ 0} & \textbf{.83$\pm$ 0} & \textbf{.83$\pm$ 0} & \textbf{.8$\pm$ 0} & \textbf{.83$\pm$ 0} & \textbf{.83$\pm$ 0} & \textbf{.8$\pm$ 0} & .72$\pm$ 0 & .72$\pm$ 0 & .72$\pm$ 0 & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{logistics}}
 & A & .31 & .44 & .52 & .55 & .59 & .63 & .67 & .69 & .74 & .81 & 1 \\
 & B & .18 & .33 & .42 & .43 & .49 & .56 & .61 & .62 & .67 & .69 & 1 \\
 & C & .24 & .3 & .35 & .34 & .46 & .61 & .66 & \textbf{.74} & \textbf{.82} & \textbf{.85} & \textbf{1} \\
 & D & \textbf{.36$\pm$ .03} & \textbf{.46$\pm$ .04} & \textbf{.54$\pm$ .03} & \textbf{.6$\pm$ .03} & \textbf{.68$\pm$ .03} & \textbf{.69$\pm$ .02} & \textbf{.71$\pm$ .02} & .73$\pm$ .02 & .81$\pm$ .01 & .84$\pm$ .01 & \textbf{1$\pm$ 0} \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & .31 & .44 & .57 & .71 & .81 & .85 & .88 & .91 & .96 & \textbf{1} & 1 \\
 & B & .26 & .39 & .55 & .62 & .65 & .7 & .81 & .86 & .82 & .84 & 1 \\
 & C & .32 & .46 & .64 & .61 & .75 & .88 & .89 & .91 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & D & \textbf{.63$\pm$ 0} & \textbf{.75$\pm$ 0} & \textbf{.83$\pm$ 0} & \textbf{.85$\pm$ 0} & \textbf{.92$\pm$ 0} & \textbf{.92$\pm$ 0} & \textbf{.93$\pm$ 0} & \textbf{.93$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & \textbf{.4} & .55 & .7 & \textbf{.88} & .91 & .92 & .92 & .96 & .98 & .98 & 1 \\
 & B & .27 & .31 & .57 & .64 & .71 & .74 & .81 & .8 & .91 & .91 & 1 \\
 & C & .32 & .52 & .7 & .84 & .88 & .93 & .93 & .98 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & D & .35$\pm$ .04 & \textbf{.61$\pm$ .03} & \textbf{.75$\pm$ .03} & .86$\pm$ .01 & \textbf{.94$\pm$ .02} & \textbf{.94$\pm$ .02} & \textbf{.94$\pm$ .02} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{satellite}}
 & A & .33 & .33 & .42 & .45 & .53 & .61 & .67 & .74 & .77 & .78 & 1 \\
 & B & .22 & .26 & .33 & .41 & .57 & .64 & .75 & .75 & .85 & .85 & 1 \\
 & C & .2 & .2 & .36 & .43 & .51 & .58 & .69 & .73 & .89 & .89 & \textbf{1} \\
 & D & \textbf{.46$\pm$ .06} & \textbf{.44$\pm$ .06} & \textbf{.52$\pm$ .07} & \textbf{.61$\pm$ .06} & \textbf{.69$\pm$ .05} & \textbf{.77$\pm$ .04} & \textbf{.82$\pm$ .03} & \textbf{.9$\pm$ .02} & \textbf{.92$\pm$ .03} & \textbf{.92$\pm$ .03} & 1$\pm$ .09 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & \textbf{.14} & .21 & .35 & \textbf{.48} & .56 & \textbf{.56} & .55 & \textbf{.66} & \textbf{.69} & \textbf{.78} & 1 \\
 & B & \textbf{.14} & \textbf{.32} & \textbf{.46} & .44 & \textbf{.58} & .54 & \textbf{.62} & .61 & .64 & .74 & 1 \\
 & C & \textbf{.14} & .2 & .25 & .34 & .41 & .52 & .55 & .55 & .59 & .73 & \textbf{1} \\
 & D & .09$\pm$ .03 & .18$\pm$ .04 & .3$\pm$ .04 & .46$\pm$ .03 & .47$\pm$ .03 & .54$\pm$ .03 & .53$\pm$ .04 & .54$\pm$ .04 & .61$\pm$ .03 & .68$\pm$ .03 & 1$\pm$ 0 \\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & .24 & .26 & .36 & .48 & .72 & .73 & .82 & .87 & .89 & .93 & 1 \\
 & B & .16 & .25 & .35 & .42 & .57 & .62 & .69 & .76 & .93 & \textbf{.96} & 1 \\
 & C & .29 & \textbf{.38} & .48 & .48 & .54 & .61 & .75 & .82 & .82 & .93 & \textbf{1} \\
 & D & \textbf{.33$\pm$ .05} & .35$\pm$ .05 & \textbf{.57$\pm$ .06} & \textbf{.64$\pm$ .04} & \textbf{.8$\pm$ .03} & \textbf{.8$\pm$ .03} & \textbf{.9$\pm$ .03} & \textbf{.96$\pm$ 0} & \textbf{.96$\pm$ 0} & \textbf{.96$\pm$ 0} & \textbf{1$\pm$ 0} \\
\hline
\end{tabular}
}
\end{table}

==> tables/missingObs/evaluationTable_missingObs_average.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (PLR-wGraph, RG09, LPBased, VRL-10-woActions) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Precision (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{4}{*}{\rotatebox[origin=c]{90}{10\%}}
 & A & .3 & .3 & .31 & .34 & .4 & .4 & .41 & .42 & .42 & .42 & \textbf{1.9} \\
 & B & .28 & .28 & .3 & .32 & .38 & .38 & .39 & .41 & .42 & .42 & 4.5\\
 & C & .17 & .17 & .18 & .19 & .23 & .24 & .27 & .29 & .3 & .3 & 6.0\\
 & D & \textbf{.3} & \textbf{.32} & \textbf{.33} & \textbf{.36} & \textbf{.43} & \textbf{.44} & \textbf{.45} & \textbf{.47} & \textbf{.48} & \textbf{.48} & 2.7\\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{30\%}}
 & A & .29 & .32 & .36 & .4 & .44 & .46 & .52 & .56 & .61 & .62 & \textbf{1.6} \\
 & B & .28 & .32 & .36 & .4 & .45 & .48 & .51 & .55 & .59 & .6 & 3.2\\
 & C & .18 & .21 & .26 & .3 & .36 & .39 & .43 & .47 & .5 & .51 & 3.9\\
 & D & \textbf{.31} & \textbf{.36} & \textbf{.41} & \textbf{.46} & \textbf{.51} & \textbf{.53} & \textbf{.58} & \textbf{.62} & \textbf{.64} & \textbf{.65} & 2.0\\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{50\%}}
 & A & .28 & .35 & .39 & .46 & .51 & .54 & .56 & .59 & .66 & .7 & \textbf{1.6} \\
 & B & .28 & .35 & .4 & .44 & .5 & .53 & .55 & .6 & .65 & .68 & 2.8\\
 & C & .2 & .27 & .35 & .4 & .49 & .52 & .58 & .62 & .67 & .71 & 3.0\\
 & D & \textbf{.29} & \textbf{.38} & \textbf{.44} & \textbf{.5} & \textbf{.57} & \textbf{.6} & \textbf{.61} & \textbf{.66} & \textbf{.7} & \textbf{.73} & 1.8\\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{70\%}}
 & A & .31 & .36 & .45 & .5 & .57 & .61 & .65 & .69 & .75 & \textbf{.82} & \textbf{1.5} \\
 & B & .3 & .37 & .45 & .51 & .58 & .62 & .64 & .68 & .71 & .75 & 2.5\\
 & C & .21 & .28 & .37 & .43 & .53 & .55 & .63 & .66 & .73 & .77 & 2.7\\
 & D & \textbf{.32} & \textbf{.4} & \textbf{.47} & \textbf{.53} & \textbf{.6} & \textbf{.64} & \textbf{.69} & \textbf{.73} & \textbf{.77} & .8 & 1.6\\
\hline
\end{tabular}
}
\end{table}

==> tables/noisyObs/evaluationTable_noisyObs_25.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (PLR, RG09, VS) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Precision (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{3}{*}{\rotatebox[origin=c]{90}{average}}
 & A & .36 & .36 & .41 & .42 & .41 & .41 & .41 & .43 & .43 & .43 & \textbf{1.3} \\
 & B & .37 & .37 & .41 & .42 & .45 & .45 & .45 & .45 & .45 & .45 & 3.2\\
 & C & \textbf{.39} & \textbf{.4} & \textbf{.44} & \textbf{.47} & \textbf{.47} & \textbf{.48} & \textbf{.49} & \textbf{.51} & \textbf{.51} & \textbf{.51} & 1.8\\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{campus}}
 & A & \textbf{.76} & .76 & \textbf{.83} & \textbf{.86} & \textbf{.86} & \textbf{.86} & \textbf{.85} & \textbf{.81} & \textbf{.81} & \textbf{.81} & \textbf{1.0} \\
 & B & .72 & .72 & .73 & .74 & .74 & .74 & .74 & .74 & .74 & .74 & 1.3\\
 & C & \textbf{.76} & \textbf{.77} & .78 & .8 & .76 & .76 & .74 & .71 & .71 & .71 & 1.3\\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & .15 & .15 & .15 & .17 & .18 & .18 & .19 & .23 & .23 & .23 & \textbf{1.6} \\
 & B & \textbf{.19} & .19 & .18 & .22 & .24 & .24 & .23 & .22 & .22 & .22 & 6.4\\
 & C & .17 & \textbf{.2} & \textbf{.25} & \textbf{.33} & \textbf{.45} & \textbf{.47} & \textbf{.59} & \textbf{.65} & \textbf{.65} & \textbf{.65} & 2.0\\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{intrusion-detection}}
 & A & \textbf{.15} & \textbf{.15} & \textbf{.25} & \textbf{.25} & .26 & .26 & .25 & .33 & .33 & .33 & \textbf{1.1} \\
 & B & \textbf{.15} & \textbf{.15} & \textbf{.25} & \textbf{.25} & \textbf{.31} & \textbf{.31} & \textbf{.32} & \textbf{.34} & \textbf{.34} & \textbf{.34} & 3.3\\
 & C & \textbf{.15} & \textbf{.15} & .24 & .23 & .27 & .27 & .24 & .28 & .28 & .28 & 2.5\\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{kitchen}}
 & A & .38 & .38 & .4 & .4 & .34 & .34 & .34 & .36 & .36 & .36 & \textbf{1.4} \\
 & B & .41 & .41 & .49 & .49 & \textbf{.5} & \textbf{.5} & \textbf{.5} & \textbf{.5} & \textbf{.5} & \textbf{.5} & 1.7\\
 & C & \textbf{.49} & \textbf{.49} & \textbf{.5} & \textbf{.5} & .41 & .41 & .41 & .41 & .41 & .41 & \textbf{1.4} \\
\hline
\end{tabular}
}
\end{table}

==> tables/noisyObs/evaluationTable_noisyObs_50.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (PLR, RG09, VS) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Precision (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{3}{*}{\rotatebox[origin=c]{90}{average}}
 & A & .36 & .41 & .45 & .45 & .51 & .53 & .55 & .63 & .67 & .68 & \textbf{1.2} \\
 & B & .39 & .44 & .47 & .48 & .51 & .52 & .53 & .54 & .56 & .56 & 2.8\\
 & C & \textbf{.41} & \textbf{.47} & \textbf{.49} & \textbf{.52} & \textbf{.57} & \textbf{.59} & \textbf{.61} & \textbf{.67} & \textbf{.72} & \textbf{.72} & 1.6\\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{campus}}
 & A & .83 & \textbf{.89} & \textbf{.92} & \textbf{.95} & \textbf{.97} & \textbf{.95} & \textbf{.94} & \textbf{.91} & \textbf{.91} & \textbf{.91} & \textbf{1.0} \\
 & B & .77 & .76 & .76 & .77 & .77 & .77 & .77 & .76 & .77 & .77 & 1.3\\
 & C & \textbf{.86} & .85 & .87 & .88 & .89 & .86 & .84 & .83 & .81 & .81 & 1.2\\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & .14 & .13 & .13 & .14 & .18 & .2 & .25 & .4 & .51 & .53 & \textbf{1.5} \\
 & B & \textbf{.24} & .27 & .28 & .31 & .27 & .24 & .19 & .19 & .18 & .18 & 6.3\\
 & C & .22 & \textbf{.33} & \textbf{.36} & \textbf{.44} & \textbf{.5} & \textbf{.52} & \textbf{.54} & \textbf{.67} & \textbf{.8} & \textbf{.81} & 1.9\\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{intrusion-detection}}
 & A & .13 & .22 & .35 & .39 & .52 & .6 & .6 & .72 & .83 & .83 & \textbf{1.1} \\
 & B & .19 & .26 & \textbf{.38} & \textbf{.44} & \textbf{.57} & \textbf{.67} & \textbf{.71} & \textbf{.8} & \textbf{.87} & \textbf{.87} & 2.3\\
 & C & \textbf{.2} & \textbf{.27} & .36 & .38 & .5 & .58 & .62 & .73 & .81 & .81 & 2.0\\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{kitchen}}
 & A & .34 & .41 & .39 & .33 & .37 & .37 & .43 & \textbf{.49} & .44 & .44 & \textbf{1.2} \\
 & B & \textbf{.37} & \textbf{.48} & \textbf{.45} & \textbf{.42} & \textbf{.41} & \textbf{.41} & \textbf{.44} & .43 & .43 & .43 & 1.5\\
 & C & .35 & .43 & .37 & .36 & \textbf{.41} & \textbf{.41} & \textbf{.44} & .45 & \textbf{.45} & \textbf{.45} & \textbf{1.2} \\
\hline
\end{tabular}
}
\end{table}

==> tables/noisyObs/evaluationTable_noisyObs_average.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (PLR, RG09, VS) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Precision (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{3}{*}{\rotatebox[origin=c]{90}{25\%}}
 & A & .36 & .36 & .41 & .42 & .41 & .41 & .41 & .43 & .43 & .43 & \textbf{1.3} \\
 & B & .37 & .37 & .41 & .42 & .45 & .45 & .45 & .45 & .45 & .45 & 3.2\\
 & C & \textbf{.39} & \textbf{.4} & \textbf{.44} & \textbf{.47} & \textbf{.47} & \textbf{.48} & \textbf{.49} & \textbf{.51} & \textbf{.51} & \textbf{.51} & 1.8\\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{50\%}}
 & A & .36 & .41 & .45 & .45 & .51 & .53 & .55 & .63 & .67 & .68 & \textbf{1.2} \\
 & B & .39 & .44 & .47 & .48 & .51 & .52 & .53 & .54 & .56 & .56 & 2.8\\
 & C & \textbf{.41} & \textbf{.47} & \textbf{.49} & \textbf{.52} & \textbf{.57} & \textbf{.59} & \textbf{.61} & \textbf{.67} & \textbf{.72} & \textbf{.72} & 1.6\\
\hline
\end{tabular}
}
\end{table}

==> tables/pmTest.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MS, RG09, LPBased, PLR, standardDeviationPerformance) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{5}{*}{\rotatebox[origin=c]{90}{average}}
 & A & .35 & .43 & .49 & .57 & .63 & .67 & .73 & .77 & .79 & .81 & 1 \\
 & B & .32 & .43 & .5 & .59 & .65 & .69 & .75 & .78 & .82 & .86 & 1 \\
 & C & .23 & .34 & .42 & .51 & .59 & .64 & .7 & .74 & .81 & .86 & 1 \\
 & D & .3 & .35 & .43 & .51 & .59 & .66 & .7 & .76 & .83 & .9 & \textbf{1} \\
 & E & \textbf{.38$\pm$ .01} & \textbf{.49$\pm$ .01} & \textbf{.59$\pm$ .01} & \textbf{.66$\pm$ .01} & \textbf{.73$\pm$ .01} & \textbf{.77$\pm$ .01} & \textbf{.83$\pm$ 0} & \textbf{.87$\pm$ 0} & \textbf{.91$\pm$ 0} & \textbf{.94$\pm$ 0} & 1$\pm$ .01 \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{blocks-world}}
 & A & .1 & .13 & .14 & .24 & .29 & .36 & .41 & .47 & .54 & .55 & 1 \\
 & B & .08 & .22 & .23 & .29 & .38 & .42 & .53 & .63 & \textbf{.81} & \textbf{.9} & 1 \\
 & C & .06 & .13 & .15 & .2 & .33 & .38 & .46 & .52 & .76 & .81 & 1 \\
 & D & .09 & .09 & .1 & .1 & .09 & .09 & .09 & .07 & .21 & .27 & \textbf{1} \\
 & E & \textbf{.13$\pm$ 0} & \textbf{.31$\pm$ 0} & \textbf{.24$\pm$ 0} & \textbf{.32$\pm$ 0} & \textbf{.42$\pm$ 0} & \textbf{.47$\pm$ 0} & \textbf{.57$\pm$ 0} & \textbf{.66$\pm$ 0} & .8$\pm$ 0 & \textbf{.9$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{campus}}
 & A & .73 & .73 & .73 & .53 & .57 & .43 & .57 & .63 & .6 & .6 & 1 \\
 & B & .73 & .8 & .8 & .83 & .83 & .83 & .83 & .8 & .8 & .8 & 1 \\
 & C & .5 & .87 & .87 & .97 & .97 & .97 & .97 & .97 & .97 & .97 & 1 \\
 & D & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & E & .67$\pm$ 0 & .87$\pm$ 0 & .87$\pm$ 0 & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{depots}}
 & A & \textbf{.21} & .16 & .16 & .22 & .38 & .49 & .48 & .54 & .59 & .59 & 1 \\
 & B & .16 & \textbf{.29} & \textbf{.28} & \textbf{.32} & .45 & .62 & .59 & .6 & .61 & .78 & 1 \\
 & C & .09 & .16 & .17 & .27 & .34 & .44 & .57 & .69 & .75 & .89 & 1 \\
 & D & .18 & .14 & .2 & .2 & .23 & .3 & .5 & .64 & .61 & .82 & \textbf{1} \\
 & E & .19$\pm$ .03 & .18$\pm$ .04 & \textbf{.28$\pm$ .05} & .3$\pm$ .03 & \textbf{.55$\pm$ .05} & \textbf{.68$\pm$ .04} & \textbf{.84$\pm$ .03} & \textbf{.9$\pm$ .02} & \textbf{.99$\pm$ .01} & \textbf{1$\pm$ 0} & 1$\pm$ .02 \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & A & .29 & \textbf{.37} & .5 & \textbf{.63} & \textbf{.73} & \textbf{.84} & \textbf{.92} & \textbf{.91} & \textbf{.91} & \textbf{.96} & 1 \\
 & B & .22 & .27 & .35 & .46 & .52 & .6 & .75 & .77 & .81 & .81 & 1 \\
 & C & .2 & .26 & .37 & .5 & .58 & .68 & .67 & .68 & .76 & .8 & 1 \\
 & D & .25 & .23 & .39 & .52 & .61 & .75 & .8 & .8 & .82 & .92 & \textbf{1} \\
 & E & \textbf{.32$\pm$ .04} & .35$\pm$ .05 & \textbf{.58$\pm$ .06} & .61$\pm$ .06 & .56$\pm$ .05 & .63$\pm$ .04 & .79$\pm$ .04 & .86$\pm$ .03 & .88$\pm$ .02 & .88$\pm$ .02 & 1$\pm$ 0 \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{dwr}}
 & A & .13 & .23 & .2 & .34 & .34 & .39 & .43 & .47 & .46 & .55 & 1 \\
 & B & .25 & .33 & .32 & .26 & .2 & .22 & .3 & .27 & .31 & .41 & 1 \\
 & C & .19 & .18 & .24 & .29 & .28 & .33 & .51 & .51 & .65 & .81 & 1 \\
 & D & .23 & .16 & .27 & \textbf{.45} & \textbf{.5} & \textbf{.54} & .52 & \textbf{.63} & \textbf{.79} & \textbf{1} & \textbf{1} \\
 & E & \textbf{.31$\pm$ .04} & \textbf{.49$\pm$ .06} & \textbf{.47$\pm$ .04} & .44$\pm$ .04 & .36$\pm$ .04 & .44$\pm$ .06 & \textbf{.61$\pm$ .04} & .61$\pm$ .04 & .73$\pm$ .03 & .87$\pm$ .04 & 1$\pm$ .01 \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & .29 & .32 & .44 & \textbf{.52} & .56 & .63 & \textbf{.71} & .76 & .83 & .94 & 1 \\
 & B & \textbf{.32} & \textbf{.34} & .45 & .48 & .57 & .63 & .69 & \textbf{.78} & .85 & \textbf{1} & 1 \\
 & C & .13 & .24 & .28 & .35 & .39 & .47 & .5 & .57 & .7 & .78 & 1 \\
 & D & .2 & .22 & .36 & .42 & .42 & .5 & .58 & .59 & .72 & \textbf{1} & \textbf{1} \\
 & E & .28$\pm$ 0 & .33$\pm$ .01 & \textbf{.46$\pm$ .03} & \textbf{.52$\pm$ .02} & \textbf{.67$\pm$ .02} & \textbf{.67$\pm$ .02} & .69$\pm$ .01 & \textbf{.78$\pm$ .01} & \textbf{.88$\pm$ .02} & .93$\pm$ 0 & \textbf{1$\pm$ .01} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{ferry}}
 & A & .38 & \textbf{.7} & \textbf{.8} & .83 & .89 & .95 & .93 & .96 & .96 & .96 & 1 \\
 & B & .28 & .58 & .73 & .8 & .89 & .91 & .95 & .96 & .96 & .96 & 1 \\
 & C & .19 & .34 & .54 & .75 & .85 & .88 & .91 & .91 & .93 & .96 & 1 \\
 & D & .25 & .38 & .64 & .73 & .84 & .89 & .96 & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & E & \textbf{.41$\pm$ 0} & .65$\pm$ .01 & .75$\pm$ .01 & \textbf{.87$\pm$ 0} & \textbf{.98$\pm$ 0} & \textbf{.98$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{intrusion-detection}}
 & A & \textbf{.26} & \textbf{.45} & .59 & \textbf{.8} & \textbf{.83} & \textbf{.83} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & 1 \\
 & B & \textbf{.26} & \textbf{.45} & .59 & \textbf{.8} & \textbf{.83} & \textbf{.83} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & 1 \\
 & C & .18 & .24 & .35 & .38 & .66 & .67 & .72 & .78 & .94 & .96 & 1 \\
 & D & .16 & .33 & .34 & .62 & .64 & .77 & .81 & .92 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & E & .22$\pm$ 0 & .4$\pm$ 0 & \textbf{.65$\pm$ 0} & .77$\pm$ 0 & .81$\pm$ 0 & .81$\pm$ 0 & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{kitchen}}
 & A & .7 & \textbf{.77} & \textbf{.87} & \textbf{.87} & .67 & .67 & .8 & .9 & \textbf{.9} & \textbf{.9} & \textbf{1} \\
 & B & .66 & .73 & .77 & .83 & .83 & .83 & .83 & \textbf{.93} & .8 & .8 & 1 \\
 & C & .51 & .54 & .58 & .73 & .77 & .77 & .7 & .76 & .67 & .67 & 1 \\
 & D & .33 & .33 & .24 & .16 & .33 & .33 & .33 & .53 & .53 & .53 & 1 \\
 & E & \textbf{.77$\pm$ 0} & \textbf{.77$\pm$ 0} & \textbf{.87$\pm$ 0} & \textbf{.87$\pm$ 0} & \textbf{.87$\pm$ 0} & \textbf{.87$\pm$ 0} & \textbf{.87$\pm$ 0} & .87$\pm$ 0 & .77$\pm$ 0 & .77$\pm$ 0 & \textbf{1$\pm$ 0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{logistics}}
 & A & .35 & .41 & .47 & .6 & .7 & .73 & .76 & \textbf{.89} & \textbf{.97} & \textbf{1} & 1 \\
 & B & .34 & .47 & .58 & \textbf{.69} & .72 & .77 & .8 & .82 & .93 & \textbf{1} & 1 \\
 & C & .16 & .35 & .41 & .48 & .5 & .53 & .68 & .68 & .69 & .74 & 1 \\
 & D & .23 & .39 & .42 & .51 & .58 & .76 & \textbf{.83} & \textbf{.89} & \textbf{.97} & \textbf{1} & \textbf{1} \\
 & E & \textbf{.42$\pm$ .03} & \textbf{.5$\pm$ .03} & \textbf{.59$\pm$ .03} & \textbf{.69$\pm$ .03} & \textbf{.77$\pm$ .02} & \textbf{.81$\pm$ .01} & \textbf{.83$\pm$ .01} & \textbf{.89$\pm$ 0} & \textbf{.97$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ .01} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & .41 & .65 & .73 & \textbf{.84} & .88 & .86 & .89 & \textbf{.96} & \textbf{1} & \textbf{1} & 1 \\
 & B & .32 & .49 & .59 & .74 & .82 & .87 & .9 & .95 & \textbf{1} & \textbf{1} & 1 \\
 & C & .24 & .43 & .58 & .57 & .76 & .8 & .82 & .86 & .95 & .93 & 1 \\
 & D & .34 & .54 & .64 & .71 & .77 & .86 & .89 & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & E & \textbf{.61$\pm$ 0} & \textbf{.77$\pm$ 0} & \textbf{.8$\pm$ 0} & .83$\pm$ 0 & \textbf{.9$\pm$ 0} & \textbf{.92$\pm$ 0} & \textbf{.93$\pm$ 0} & \textbf{.96$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & .46 & \textbf{.6} & .69 & .89 & .89 & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & 1 \\
 & B & .43 & \textbf{.6} & .74 & \textbf{.91} & \textbf{.92} & .93 & .93 & .96 & .98 & .98 & 1 \\
 & C & .31 & .48 & .64 & .67 & .7 & .74 & .81 & .84 & .91 & .93 & 1 \\
 & D & \textbf{.48} & .52 & \textbf{.8} & .82 & .86 & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & E & .47$\pm$ .05 & .58$\pm$ .04 & .78$\pm$ .01 & .85$\pm$ .03 & .89$\pm$ 0 & \textbf{.96$\pm$ 0} & \textbf{.96$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{satellite}}
 & A & .35 & .31 & .36 & .43 & .59 & .66 & .74 & .81 & .81 & .81 & 1 \\
 & B & .35 & .35 & .42 & .54 & .64 & .62 & .67 & .71 & .74 & .77 & 1 \\
 & C & .26 & .29 & .38 & .52 & .52 & .62 & .72 & .71 & .72 & .75 & 1 \\
 & D & .34 & .24 & .29 & .6 & \textbf{.77} & .8 & .82 & .91 & \textbf{.95} & \textbf{.96} & \textbf{1} \\
 & E & \textbf{.48$\pm$ .03} & \textbf{.47$\pm$ .05} & \textbf{.58$\pm$ .06} & \textbf{.68$\pm$ .03} & .76$\pm$ .04 & \textbf{.81$\pm$ .03} & \textbf{.88$\pm$ .03} & \textbf{.94$\pm$ .02} & .94$\pm$ .02 & \textbf{.96$\pm$ .01} & 1$\pm$ .07 \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & \textbf{.28} & \textbf{.3} & .16 & .14 & .27 & .3 & .34 & .25 & .29 & .3 & 1 \\
 & B & .15 & .22 & .32 & .45 & \textbf{.58} & .6 & .61 & \textbf{.68} & .73 & .8 & 1 \\
 & C & .16 & .25 & \textbf{.36} & \textbf{.5} & .57 & \textbf{.63} & \textbf{.68} & .64 & .83 & .87 & 1 \\
 & D & .13 & .21 & .25 & .32 & .5 & .57 & .57 & .5 & \textbf{.86} & \textbf{.96} & \textbf{1} \\
 & E & .08$\pm$ .03 & .24$\pm$ .05 & .34$\pm$ .03 & .46$\pm$ .05 & .55$\pm$ .04 & .52$\pm$ .03 & .56$\pm$ .03 & .61$\pm$ .03 & .68$\pm$ .03 & .79$\pm$ .01 & \textbf{1$\pm$ 0} \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & .32 & .36 & .57 & \textbf{.68} & \textbf{.82} & \textbf{.95} & \textbf{.96} & .98 & \textbf{1} & \textbf{1} & 1 \\
 & B & .28 & .29 & .38 & .48 & .59 & .73 & .83 & .89 & .93 & .96 & 1 \\
 & C & .22 & .3 & .42 & .52 & .6 & .65 & .85 & .92 & .95 & \textbf{1} & 1 \\
 & D & .3 & .41 & .45 & .48 & .73 & .82 & .89 & .96 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & E & \textbf{.41$\pm$ .04} & \textbf{.47$\pm$ .04} & \textbf{.58$\pm$ .05} & .64$\pm$ .04 & .78$\pm$ .04 & \textbf{.95$\pm$ .02} & .95$\pm$ .02 & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} \\
\hline
\end{tabular}
}
\end{table}

==> tables/rules/depots_precision.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MS, RG09, LPBased, PLR-rhw, balanced-svr, VSAPN) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{6}{*}{\rotatebox[origin=c]{90}{average}}
 & A & .31 & .39 & .47 & .59 & .66 & .73 & .76 & .81 & .84 & .88 & 1.6\\
 & B & .29 & .39 & .46 & .54 & .6 & .67 & .72 & .76 & .8 & .87 & 2.3\\
 & C & .19 & .3 & .39 & .46 & .52 & .58 & .68 & .72 & .79 & .86 & 2.5\\
 & D & .28 & .33 & .44 & .51 & .59 & .69 & .75 & .81 & .86 & .97 & 1.1\\
 & E & .28 & .36 & .48 & .54 & .59 & .65 & .72 & .76 & .83 & .94 & \textbf{1.0} \\
 & F & \textbf{.38} & \textbf{.45} & \textbf{.56} & \textbf{.6} & \textbf{.69} & \textbf{.75} & \textbf{.84} & \textbf{.89} & \textbf{.95} & \textbf{.97} & 1.1\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{depots}}
 & A & \textbf{.21} & .16 & .16 & .22 & .38 & .49 & .48 & .54 & .59 & .59 & 1.8\\
 & B & .16 & \textbf{.29} & .28 & .32 & .45 & .62 & .59 & .6 & .61 & .78 & 2.6\\
 & C & .09 & .16 & .17 & .27 & .34 & .44 & .57 & .69 & .75 & .89 & 2.4\\
 & D & .18 & .14 & .2 & .2 & .23 & .3 & .5 & .64 & .61 & .82 & 1.2\\
 & E & .14 & .14 & .29 & \textbf{.34} & .46 & \textbf{.71} & .71 & .86 & .93 & \textbf{1.0} & \textbf{1.0} \\
 & F & \textbf{.21} & .14 & \textbf{.32} & .29 & \textbf{.54} & .68 & \textbf{.86} & \textbf{.89} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & A & .29 & \textbf{.37} & \textbf{.5} & \textbf{.63} & \textbf{.73} & \textbf{.84} & \textbf{.92} & \textbf{.91} & \textbf{.91} & \textbf{.96} & 1.4\\
 & B & .22 & .27 & .35 & .46 & .52 & .6 & .75 & .77 & .81 & .81 & 2.9\\
 & C & .2 & .26 & .37 & .5 & .58 & .68 & .67 & .68 & .76 & .8 & 2.3\\
 & D & .25 & .23 & .39 & .52 & .61 & .75 & .8 & .8 & .82 & .92 & 1.1\\
 & E & .25 & .25 & .43 & .46 & .46 & .43 & .57 & .57 & .64 & .64 & \textbf{1.0} \\
 & F & \textbf{.32} & .36 & \textbf{.5} & .57 & .57 & .57 & .79 & .89 & .89 & .93 & \textbf{1.0} \\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{dwr}}
 & A & .13 & .23 & .2 & .34 & .34 & .39 & .43 & .47 & .46 & .55 & 2.0\\
 & B & .25 & .33 & .32 & .26 & .2 & .22 & .3 & .27 & .31 & .41 & 2.7\\
 & C & .19 & .18 & .24 & .29 & .28 & .33 & .51 & .51 & .65 & .81 & 2.0\\
 & D & .23 & .16 & .27 & \textbf{.45} & \textbf{.5} & \textbf{.54} & .52 & .63 & .79 & \textbf{1.0} & 1.1\\
 & E & .21 & .34 & .3 & .38 & .39 & .43 & \textbf{.68} & \textbf{.75} & .82 & \textbf{1.0} & \textbf{1.0} \\
 & F & \textbf{.36} & \textbf{.39} & \textbf{.46} & .39 & .43 & .5 & \textbf{.68} & .68 & \textbf{.86} & .89 & \textbf{1.0} \\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & .29 & .32 & .44 & \textbf{.52} & .56 & .63 & .71 & .76 & .83 & .94 & 2.4\\
 & B & \textbf{.32} & .34 & \textbf{.45} & .48 & .57 & .63 & .69 & .78 & .85 & \textbf{1.0} & 3.0\\
 & C & .13 & .24 & .28 & .35 & .39 & .47 & .5 & .57 & .7 & .78 & 3.3\\
 & D & .2 & .22 & .36 & .42 & .42 & .5 & .58 & .59 & .72 & \textbf{1.0} & \textbf{1.0} \\
 & E & .25 & .24 & .35 & .21 & .2 & .2 & .2 & .21 & .37 & .9 & \textbf{1.0} \\
 & F & .3 & \textbf{.35} & .41 & \textbf{.52} & \textbf{.58} & \textbf{.65} & \textbf{.72} & \textbf{.81} & \textbf{.88} & .93 & \textbf{1.0} \\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{logistics}}
 & A & .35 & .41 & .47 & .6 & .7 & .73 & .76 & \textbf{.89} & \textbf{.97} & \textbf{1.0} & 1.5\\
 & B & .34 & .47 & .58 & .69 & .72 & .77 & .8 & .82 & .93 & \textbf{1.0} & 1.9\\
 & C & .16 & .35 & .41 & .48 & .5 & .53 & .68 & .68 & .69 & .74 & 3.7\\
 & D & .23 & .39 & .42 & .51 & .58 & .76 & \textbf{.83} & \textbf{.89} & \textbf{.97} & \textbf{1.0} & 1.2\\
 & E & \textbf{.46} & \textbf{.53} & \textbf{.59} & .69 & .69 & .75 & .81 & .88 & \textbf{.97} & \textbf{1.0} & \textbf{1.0} \\
 & F & .41 & .51 & \textbf{.59} & \textbf{.71} & \textbf{.8} & \textbf{.82} & .82 & \textbf{.89} & \textbf{.97} & \textbf{1.0} & 1.2\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & .41 & .65 & .73 & \textbf{.84} & .88 & .86 & .89 & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.3\\
 & B & .32 & .49 & .59 & .74 & .82 & .87 & .9 & .95 & \textbf{1.0} & \textbf{1.0} & 1.7\\
 & C & .24 & .43 & .58 & .57 & .76 & .8 & .82 & .86 & .95 & .93 & 2.0\\
 & D & .34 & .54 & .64 & .71 & .77 & .86 & .89 & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & E & .39 & .5 & .54 & .64 & .79 & .82 & .86 & .86 & .93 & \textbf{1.0} & \textbf{1.0} \\
 & F & \textbf{.61} & \textbf{.77} & \textbf{.8} & .83 & \textbf{.9} & \textbf{.92} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & 1.2\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & .46 & .6 & .69 & .89 & .89 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.2\\
 & B & .43 & .6 & .74 & \textbf{.91} & \textbf{.92} & .93 & .93 & .96 & .98 & .98 & 1.5\\
 & C & .31 & .48 & .64 & .67 & .7 & .74 & .81 & .84 & .91 & .93 & 2.0\\
 & D & \textbf{.48} & .52 & .8 & .82 & .86 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.1\\
 & E & .36 & .5 & .79 & .82 & .82 & .93 & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & F & .46 & \textbf{.64} & \textbf{.82} & .86 & .89 & \textbf{.96} & \textbf{.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & .32 & .36 & \textbf{.57} & .68 & .82 & .95 & .96 & .98 & \textbf{1.0} & \textbf{1.0} & 1.2\\
 & B & .28 & .29 & .38 & .48 & .59 & .73 & .83 & .89 & .93 & .96 & 1.8\\
 & C & .22 & .3 & .42 & .52 & .6 & .65 & .85 & .92 & .95 & \textbf{1.0} & 2.4\\
 & D & .3 & .41 & .45 & .48 & .73 & .82 & .89 & .96 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
 & E & .18 & .36 & \textbf{.57} & \textbf{.75} & \textbf{.93} & \textbf{.96} & \textbf{1.0} & .96 & .96 & \textbf{1.0} & \textbf{1.0} \\
 & F & \textbf{.39} & \textbf{.46} & \textbf{.57} & .64 & .82 & .93 & .93 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} \\
\hline
\end{tabular}
}
\end{table}

==> tables/sap_inspiration_session/precision.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (MS, PLR-rhw, standardDeviationPerformance) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Precision (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{3}{*}{\rotatebox[origin=c]{90}{average}}
 & GRP & .35 & .43 & .49 & .57 & .63 & .67 & .73 & .77 & .79 & .81 & 1 \\
 & LBR & .28 & .32 & .41 & .5 & .57 & .64 & .68 & .72 & .8 & .86 & \textbf{1} \\
 & FPV & \textbf{.38$\pm$ .01} & \textbf{.49$\pm$ .01} & \textbf{.59$\pm$ .01} & \textbf{.66$\pm$ .01} & \textbf{.73$\pm$ .01} & \textbf{.77$\pm$ .01} & \textbf{.83$\pm$ 0} & \textbf{.87$\pm$ 0} & \textbf{.91$\pm$ 0} & \textbf{.94$\pm$ 0} & \textbf{1$\pm$ .01} \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{blocks-world}}
 & A & .1 & .13 & .14 & .24 & .29 & .36 & .41 & .47 & .54 & .55 & 1 \\
 & B & .09 & .09 & .1 & .1 & .09 & .09 & .09 & .07 & .21 & .27 & \textbf{1} \\
 & C & \textbf{.13$\pm$ 0} & \textbf{.31$\pm$ 0} & \textbf{.24$\pm$ 0} & \textbf{.32$\pm$ 0} & \textbf{.42$\pm$ 0} & \textbf{.47$\pm$ 0} & \textbf{.57$\pm$ 0} & \textbf{.66$\pm$ 0} & \textbf{.8$\pm$ 0} & \textbf{.9$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{campus}}
 & A & .73 & .73 & .73 & .53 & .57 & .43 & .57 & .63 & .6 & .6 & 1 \\
 & B & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & C & .67$\pm$ 0 & .87$\pm$ 0 & .87$\pm$ 0 & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{depots}}
 & A & \textbf{.21} & .16 & .16 & .22 & .38 & .49 & .48 & .54 & .59 & .59 & 1 \\
 & B & .18 & .14 & .2 & .2 & .23 & .3 & .5 & .64 & .61 & .82 & \textbf{1} \\
 & C & .19$\pm$ .03 & \textbf{.18$\pm$ .04} & \textbf{.28$\pm$ .05} & \textbf{.3$\pm$ .03} & \textbf{.55$\pm$ .05} & \textbf{.68$\pm$ .04} & \textbf{.84$\pm$ .03} & \textbf{.9$\pm$ .02} & \textbf{.99$\pm$ .01} & \textbf{1$\pm$ 0} & 1$\pm$ .02 \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & A & .29 & \textbf{.37} & .5 & \textbf{.63} & \textbf{.73} & \textbf{.84} & \textbf{.92} & \textbf{.91} & \textbf{.91} & \textbf{.96} & 1 \\
 & B & .25 & .23 & .39 & .52 & .61 & .75 & .8 & .8 & .82 & .92 & \textbf{1} \\
 & C & \textbf{.32$\pm$ .04} & .35$\pm$ .05 & \textbf{.58$\pm$ .06} & .61$\pm$ .06 & .56$\pm$ .05 & .63$\pm$ .04 & .79$\pm$ .04 & .86$\pm$ .03 & .88$\pm$ .02 & .88$\pm$ .02 & 1$\pm$ 0 \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{dwr}}
 & A & .13 & .23 & .2 & .34 & .34 & .39 & .43 & .47 & .46 & .55 & 1 \\
 & B & .23 & .16 & .27 & \textbf{.45} & \textbf{.5} & \textbf{.54} & .52 & \textbf{.63} & \textbf{.79} & \textbf{1} & \textbf{1} \\
 & C & \textbf{.31$\pm$ .04} & \textbf{.49$\pm$ .06} & \textbf{.47$\pm$ .04} & .44$\pm$ .04 & .36$\pm$ .04 & .44$\pm$ .06 & \textbf{.61$\pm$ .04} & .61$\pm$ .04 & .73$\pm$ .03 & .87$\pm$ .04 & 1$\pm$ .01 \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & \textbf{.29} & .32 & .44 & \textbf{.52} & .56 & .63 & \textbf{.71} & .76 & .83 & .94 & 1 \\
 & B & .2 & .22 & .36 & .42 & .42 & .5 & .58 & .59 & .72 & \textbf{1} & \textbf{1} \\
 & C & .28$\pm$ 0 & \textbf{.33$\pm$ .01} & \textbf{.46$\pm$ .03} & \textbf{.52$\pm$ .02} & \textbf{.67$\pm$ .02} & \textbf{.67$\pm$ .02} & .69$\pm$ .01 & \textbf{.78$\pm$ .01} & \textbf{.88$\pm$ .02} & .93$\pm$ 0 & \textbf{1$\pm$ .01} \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{ferry}}
 & A & .38 & \textbf{.7} & \textbf{.8} & .83 & .89 & .95 & .93 & .96 & .96 & .96 & 1 \\
 & B & .25 & .38 & .64 & .73 & .84 & .89 & .96 & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & C & \textbf{.41$\pm$ 0} & .65$\pm$ .01 & .75$\pm$ .01 & \textbf{.87$\pm$ 0} & \textbf{.98$\pm$ 0} & \textbf{.98$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{intrusion-detection}}
 & A & \textbf{.26} & \textbf{.45} & .59 & \textbf{.8} & \textbf{.83} & \textbf{.83} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & 1 \\
 & B & .16 & .33 & .34 & .62 & .64 & .77 & .81 & .92 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & C & .22$\pm$ 0 & .4$\pm$ 0 & \textbf{.65$\pm$ 0} & .77$\pm$ 0 & .81$\pm$ 0 & .81$\pm$ 0 & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} \\
\hline
\multirow{2}{*}{\rotatebox[origin=c]{90}{kitchen}}
 & A & .7 & \textbf{.77} & \textbf{.87} & \textbf{.87} & .67 & .67 & .8 & \textbf{.9} & \textbf{.9} & \textbf{.9} & \textbf{1} \\
 & C & \textbf{.77$\pm$ 0} & \textbf{.77$\pm$ 0} & \textbf{.87$\pm$ 0} & \textbf{.87$\pm$ 0} & \textbf{.87$\pm$ 0} & \textbf{.87$\pm$ 0} & \textbf{.87$\pm$ 0} & .87$\pm$ 0 & .77$\pm$ 0 & .77$\pm$ 0 & \textbf{1$\pm$ 0} \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{logistics}}
 & A & .35 & .41 & .47 & .6 & .7 & .73 & .76 & \textbf{.89} & \textbf{.97} & \textbf{1} & 1 \\
 & B & .23 & .39 & .42 & .51 & .58 & .76 & \textbf{.83} & \textbf{.89} & \textbf{.97} & \textbf{1} & \textbf{1} \\
 & C & \textbf{.42$\pm$ .03} & \textbf{.5$\pm$ .03} & \textbf{.59$\pm$ .03} & \textbf{.69$\pm$ .03} & \textbf{.77$\pm$ .02} & \textbf{.81$\pm$ .01} & \textbf{.83$\pm$ .01} & \textbf{.89$\pm$ 0} & \textbf{.97$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ .01} \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & .41 & .65 & .73 & \textbf{.84} & .88 & .86 & .89 & \textbf{.96} & \textbf{1} & \textbf{1} & 1 \\
 & B & .34 & .54 & .64 & .71 & .77 & .86 & .89 & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & C & \textbf{.61$\pm$ 0} & \textbf{.77$\pm$ 0} & \textbf{.8$\pm$ 0} & .83$\pm$ 0 & \textbf{.9$\pm$ 0} & \textbf{.92$\pm$ 0} & \textbf{.93$\pm$ 0} & \textbf{.96$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & .46 & \textbf{.6} & .69 & \textbf{.89} & \textbf{.89} & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & 1 \\
 & B & \textbf{.48} & .52 & \textbf{.8} & .82 & .86 & \textbf{.96} & \textbf{.96} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
 & C & .47$\pm$ .05 & .58$\pm$ .04 & .78$\pm$ .01 & .85$\pm$ .03 & \textbf{.89$\pm$ 0} & \textbf{.96$\pm$ 0} & \textbf{.96$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & 1$\pm$ 0 \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{satellite}}
 & A & .35 & .31 & .36 & .43 & .59 & .66 & .74 & .81 & .81 & .81 & 1 \\
 & B & .34 & .24 & .29 & .6 & \textbf{.77} & .8 & .82 & .91 & \textbf{.95} & \textbf{.96} & \textbf{1} \\
 & C & \textbf{.48$\pm$ .03} & \textbf{.47$\pm$ .05} & \textbf{.58$\pm$ .06} & \textbf{.68$\pm$ .03} & .76$\pm$ .04 & \textbf{.81$\pm$ .03} & \textbf{.88$\pm$ .03} & \textbf{.94$\pm$ .02} & .94$\pm$ .02 & \textbf{.96$\pm$ .01} & 1$\pm$ .07 \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & \textbf{.28} & \textbf{.3} & .16 & .14 & .27 & .3 & .34 & .25 & .29 & .3 & 1 \\
 & B & .13 & .21 & .25 & .32 & .5 & \textbf{.57} & \textbf{.57} & .5 & \textbf{.86} & \textbf{.96} & \textbf{1} \\
 & C & .08$\pm$ .03 & .24$\pm$ .05 & \textbf{.34$\pm$ .03} & \textbf{.46$\pm$ .05} & \textbf{.55$\pm$ .04} & .52$\pm$ .03 & .56$\pm$ .03 & \textbf{.61$\pm$ .03} & .68$\pm$ .03 & .79$\pm$ .01 & \textbf{1$\pm$ 0} \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & .32 & .36 & .57 & \textbf{.68} & \textbf{.82} & \textbf{.95} & \textbf{.96} & .98 & \textbf{1} & \textbf{1} & 1 \\
 & B & .3 & .41 & .45 & .48 & .73 & .82 & .89 & .96 & \textbf{1} & \textbf{1} & \textbf{1} \\
 & C & \textbf{.41$\pm$ .04} & \textbf{.47$\pm$ .04} & \textbf{.58$\pm$ .05} & .64$\pm$ .04 & .78$\pm$ .04 & \textbf{.95$\pm$ .02} & .95$\pm$ .02 & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} & \textbf{1$\pm$ 0} \\
\hline
\end{tabular}
}
\end{table}

==> tables/sap_inspiration_session/time.tex <==
\begin{table}
\caption{Comparison of average computation times \textbf{in seconds} among all evaluated methods when applied to all evaluated benchmark domains. The average computation time is reported for different sizes of the observation sequence (i.e., $|\mathbf{O}|)$ and set of possible goals (i.e., $|G|$).}
\label{tab:computationTimeTable}
\centering
\resizebox*{0.75\columnwidth}{!}{
\begin{tabular}{ll|lllll}
\multicolumn{1}{c}{$|G|$}		 & \multicolumn{1}{c|}{}		 & \multicolumn{5}{c}{\textbf{$|\mathbf{O}|$}}\\
			 & 			 & 5 		 & 10 		 & 25		 & 50 		 & 100\\ \hline 
\multirow{5}{*}{5}
 & GRP & 47 & 87 & 208 & 409 & 811\\
 & LBR & 1.4 & 1.4 & 1.4 & 1.4 & 1.4\\
 & FPV & \textbf{.37} & \textbf{.37} & \textbf{.37} & \textbf{.37} & \textbf{.37}\\
\hline
\multirow{5}{*}{10}
 & GRP & 94 & 174 & 416 & 818 & 1622\\
 & LBR & 2.8 & 2.8 & 2.8 & 2.9 & 2.9\\
 & FPV & \textbf{.74} & \textbf{.74} & \textbf{.74} & \textbf{.74} & \textbf{.74}\\
\hline
\multirow{5}{*}{20}
 & GRP & 188 & 348 & 832 & 1636 & 3244\\
 & LBR & 5.7 & 5.7 & 5.7 & 5.7 & 5.7 \\
 & FPV & \textbf{1.48} & \textbf{1.48} & \textbf{1.48} & \textbf{1.48} & \textbf{1.48} \\
\hline
\end{tabular}
}
\end{table}
